Continuous Optimization for Decoding Errors

Error-correcting codes are one of the most fundamental objects in pseudorandomness, with applications in communication, complexity theory, and beyond. Codes are useful because of their ability to support decoding, which is the task of recovering a codeword from its noisy copy. List decoding is a relaxation where the decoder is allowed to output a list of codewords, and has seen tremendous progress over the last 25 years. In this thesis, we prove new algorithmic and combinatorial results about list decoding. We describe a list decoding framework that reduces the task of efficient decoding to proving distance in certain restricted proof systems. We then instantiate this framework for Tanner codes of Sipser and Spielman [IEEE Trans. Inf. Theory 1996] and Alon-Edmonds-Luby (AEL) distance amplification [FOCS 1995] of unique decodable base codes to get the first polynomial time list decoding algorithms for these codes. We also show extensions to the quantum version of AEL distance amplification to get polynomial-time list decodable quantum LDPC codes. We next give an alternate viewpoint of the above framework based on abstract regularity lemmas. We show how to efficiently implement the regularity lemma for the case of Ta-Shma's explicit codes near the Gilbert-Varshamov bound [STOC 2017]. This leads to a near-linear time algorithm for unique decoding of Ta-Shma's code. We also give new combinatorial results that improve known list sizes beyond the Johnson bound. Firstly, we adapt the AEL amplification to construct a new family of explicit codes that can be combinatorially list decoded to the optimal error correction radius. This is the first example of such a code that does not use significant algebraic ingredients. Secondly, we present list size improvements for Folded Reed-Solomon codes, improving the state of the art list size for explicit list decoding capacity achieving codes.

==> framework/prelims.tex <==
\label{sec:prelims}
%
% For a graph $G=(V,E)$, we define $N(v)$ to be the set of edges incident on the vertex $v$.
%
For a bipartite graph $G=(L,R,E)$ where $L$ is the set of left vertices, and $R$ is the set of right
vertices, we index the left set by $\li$ and the right set by $\ri$. For a vertex $\li \in L$, 
we denote the set of edges incident to it by $N_L(\li)$ (left neighborhood), and the set of edges
incident to  $\ri\in R$ is denoted by $N_R(\ri)$(right neighborhood). 
%
We use $\li \sim \ri$ to denote that the vertex $\li \in L$ is adjacent to the vertex $\ri \in R$, that is, $(\li,\ri)\in E$. 

Fix an arbitrary ordering of the edges. Then there are bijections between the sets $E$, $L \times
[d]$, and $R \times [d]$, 
given by taking $(\li,i)$ to be the $i^{th}$ edge incident on $\li$, and similarly for $R \times [d]$.
%
% each edge $e\in E$ can be uniquely mapped to a unique pair
% $(\li,i)\in L \times [d]$, where $\li$ is the left endpoint of $e$ and $e$ is the $i^{th}$ edge
% incident on $\li$ under the aforementioned ordering. Likewise, each edge $e\in E$ can be uniquely
% mapped to a pair $(\ri,j) \in R\times [d]$ where $\ri$ is the right endpoint of $e$ and $e$ is the
% $j^{th}$ edge incident on $\ri$ under the same fixed ordering. 
Henceforth, we will implicitly assume such an ordering of the edges is fixed, and use the resulting bijections.
% , which allows us to talk about $i^{th}$ edge incident on $\li$ and $j^{th}$ edge incident on $\ri$.
%

%\snote{TODO: Verify the above paragraph in detail, and maybe write it better.}

\begin{definition}
	Let $[q]$ be a finite alphabet and let $f,g\in [q]^n$. Then the (fractional) distance
        between $f,g$ is defined as \[ \dis(f,g) = \Ex{i\in [n]}{ \indi{f_i \neq g_i}} \mper \]
\end{definition}

\begin{definition}[Code, distance and rate]
	A code $\calC$ of block length $n$, distance $\delta$ and rate $\rho$ over the alphabet size $q$ is a set $\calC \subseteq [q]^n$ with the following properties
	\begin{enumerate}[(i)]
		\item $\rho = \frac{\log_{q} |\calC|}{n}$
		\item $\delta = \min_{h_1,h_2\in \calC} \dis(h_1,h_2)$
	\end{enumerate}
	Such codes are succinctly represented as $[n,\delta,\rho]_q$.
	We say $\calC$ is a linear code if $[q]$ can be identified with a finite field and $\calC$ is a linear subspace of $[q]^n$.
\end{definition}

% Sometimes, we will view $\calC$ as a bijection $\calC: [|\calC|] \rightarrow [q]^n$, or $\calC: [q^{\rho \cdot n}] \rightarrow [q]^n$.

\begin{definition}[List of codewords]
	For any $g\in [q]^n$, the list of codewords in $\calC$ that are at a distance less than
        $\delta$ from $g$ is denoted by $\calL(g,\delta)$. That is $\calL(g,\delta) = \inbraces{h\in \calC \suchthat \dis(h,g) < \delta }$.
\end{definition}

\subsection{Expander graphs}
%
\begin{definition}[$(n,d,\lambda)$-expander]
A $d$-regular bipartite graph $G(L,R,E)$ with $|L|=|R|=n$ is said to be an $(n,d,\lambda)$-expander if
\[
	\sigma_2(A_G) \leq \lambda \cdot d
\]
where $A_G$ is the $L\times R$ biadjacency matrix, and $\sigma_2(A_G)$ is its second largest singular value.
\end{definition}

Infinite families of $(n,d,\lambda)$-expanders, with growing $n$ as $d$ and $\lambda$ are constant, can be derived based on double covers of Ramanujan graphs of \cite{LPS88} as long as $\lambda \geq \frac{2\sqrt{d-1}}{d}$.

\begin{lemma}[Expander Mixing Lemma]
	Given an $(n,d,\lambda)$-expander $G=(L,R,E)$ and functions $f: L \rightarrow \R$ and $g: R \rightarrow \R$, the following well known property is a simple consequence of definition of $(n,d,\lambda)$-expanders:
	\ifnum\confversion=1
	\small
	\[
		\abs{\Ex{\li \sim \ri}{ f(\li) \cdot g(\ri)} - \Ex{\li}{f(\li)} \Ex{\ri}{g(\ri)}}
                \leq \lambda \cdot \norm{f}_2 
                \norm{g}_2
	\]
	\normalsize
	\else
	\[
		\abs{\Ex{\li \sim \ri}{ f(\li) \cdot g(\ri)} - \Ex{\li}{f(\li)} \cdot \Ex{\ri}{g(\ri)}}
                \leq \lambda \cdot \inparen{\Ex{\li}{f^2(\li)}}^{1/2} \cdot
                \inparen{\Ex{\ri}{g^2(\ri)}}^{1/2} \mper
	\]
	\fi
\end{lemma}

\subsection{Graph based codes}
%
\paragraph{Expander codes.}
We recap the construction from~\cite{Zemor01}, building on ideas from \cite{Tanner81, SS96},
which constructs an infinite family of good codes starting from any good (inner) linear code over a
small fixed block length of rate larger than $1/2$. The code $\calC_0$ is also referred to as the
base code for $\calC^{Tan}$.
\begin{definition}
	Given an inner linear code $\calC_0$ on alphabet $[q]$ and block length $d$, and a $d$-regular graph $G(V,E)$, we define the Tanner code $\TanC$ as
	\[
		\TanC = \{ h: E\rightarrow [q] \suchthat h|_{N(v)} \in \calC_0, \forall v \in V\}
	\]
	where $h|_S$ for $S\subseteq E$ denotes the restriction of $h$ to the set of coordinates indexed by $S$.
	In this work, we will only use Tanner codes defined on bipartite graphs. 
\end{definition}
By using an infinite family of graphs with constant degree $d$, we get an infinite family of codes based on an inner code of block length $d$.

\begin{theorem}[\cite{SS96}, \cite{Zemor01}]
	Let the distance and rate of the inner code $\calC_0$ be $\delta_0$ and $\rho_0$ respectively, and those of associated $\TanC$ be $\delta$ and $\rho$. If $G$ is an $(n,d,\lambda)$-expander, then $\delta \geq \delta_0\cdot (\delta_0-\lambda)$ and $\rho\geq 2\rho_0-1$.
\end{theorem}
%
The codes above were shown to be linear time decodable up to their unique decoding radius (for the designed distance) in \cite{Zemor01} and \cite{SkaRoth03}.
%
\paragraph{Alon-Edmonds-Luby distance amplification}\label{sec:AEL_prelims}

The following distance amplification scheme was introduced in \cite{ABNNR92}, \cite{AEL95} and used by \cite{GI05} to design linear time unique decodable near-MDS codes.

\begin{definition}[Concatenated codes]
	Fix an $(n,d,\lambda)$-expander $G(L,R,E)$. Let $\calC_{1}$ be an $[n,\delta_{1},r_{1}]_{q_1}$ code and let $\calC_{0}$ be a $[d,\delta_{0},r_{0}]_{q_0}$ code with $q_1 = |\calC_0|$. 
	
	We define the concatenation of $f\in [q_1]^L$ with $\calC_{0}: [q_1]\rightarrow [q_0]^d$ as $f^*: E \rightarrow [q_0]$, defined as
	\[
		f^{*}_{\calC_{0}}(e) ~=~ \calC_{0}(f(\li))(j)
	\]
	where $\li$ is the left endpoint of edge $e$ and $e$ is the $j^{th}$ edge incident on $\li$.
	The concatenated code $\calC^{*}_{\calC_{0}}(\calC_1)$ of block length $n\cdot d$ and alphabet $[q_0]$ is defined to be,
	\[
		\calC^{*}_{\calC_{0}}(\calC_{1}) ~=~ \{ f^{*}_{\calC_{0}} \suchthat f \in \calC_{1}\}
	\]
	When clear from context, we will omit $\calC_{0},\calC_1$ in the above notation to call the concatenated code $\calC^*$.
\end{definition}

\begin{claim}
	$\dis(f^{*}_{\calC_{0}},g^{*}_{\calC_{0}}) ~\geq~ \delta_{0}\cdot \dis(f,g)$, which also
        implies $\Delta(\calC^{*}_{\calC_{0}}(\calC_{1})) \geq \delta_{0} \cdot \delta_{1}$.
\end{claim}


% \begin{corollary}
% 		The distance of the concatenated code $\calC^{*}_{\calC_{0}}(\calC_{1})$ is at least $ \delta_{0} \cdot \delta_{1}$.
% \end{corollary}

\begin{definition}[AEL Codes]
	Fix an $(n,d,\lambda)$-expander $G(L,R,E)$. Let $\calC_{1}$ be an $[n,\delta_{1},r_{1}]_{q_1}$ code and let $\calC_{0}$ be a $[d,\delta_{0},r_{0}]_{q_0}$ code with $q_1 = |\calC_0|$. 
%
We define the AEL-encoding $f^{AEL}_{\calC_{0}}: R \rightarrow [q_0]^d$ as
	\[
		f^{AEL}_{\calC_{0}} (\ri) ~=~ \left( f^{*}_{\calC_{0}}(e_1),f^{*}_{\calC_{0}}(e_2),\cdots,f^{*}_{\calC_{0}}(e_d) \right)
	\]
	where $e_1,e_2,\cdots,e_d$ are the $d$ edges incident on $\ri$.
	The AEL code $\calC^{AEL}_{\calC_{0}}(\calC_{1}) \subseteq [q_0^d]^{n}$ is defined as 
	\[
		\calC^{AEL}_{\calC_{0}}(\calC_{1}) ~=~ \{ f^{AEL}_{\calC_{0}} \suchthat f \in \calC_{1}\}
	\]
	When clear from context, we will omit $\calC_{0},\calC_1$ in the above notation to call the AEL code $\AELC$.
\end{definition}
%
Alon, Edmonds and Luby, proved the following result, which shows that the construction can be used
to amplify the distance to $\delta_0$, by choosing $\lambda$ sufficiently small.
%
\begin{theorem}[\cite{AEL95}]\label{thm:ael_distance}
	$\dis(f^{AEL}_{\calC_{0}},g^{AEL}_{\calC_{0}}) ~\geq~ \delta_{0}-
        \frac{\lambda}{\dis(f,g)}$, which also implies $\Delta(\calC^{AEL}_{\calC_{0}}(\calC_{1}))
        ~\geq~ \delta_{0} - \frac{\lambda}{\delta_{1}}$.
\end{theorem}

% By choosing $\delta_{0}$ large and $\lambda$ small enough, we can amplify the distance between strings via this encoding.

% \begin{corollary}
% 	The distance of AEL code $\calC^{AEL}_{\calC_{0}}(\calC_{1})$ is at least $\delta_{0} - \frac{\lambda}{\delta_{1}}$.
% \end{corollary}

A codeword $f$ of $\AELC$ technically belongs to the space $[q_0^d]^R$. However, in this paper, we choose to identify codewords of $\AELC$ as belonging to $[q_0]^E$. It is clear that the two spaces are in bijection with each other and in fact, one can just \emph{fold} or \emph{unfold} the symbols to move from one space to the other. Choosing $f$ to be in $[q_0]^E$ allows us to talk about $f$ viewed from left vertex set $L$ or right vertex set $R$ simply by changing the distance functions. Let $f,g \in \AELC$, then we define the following three distance functions:
%
\begin{align*}
	\dis^L(f,g) &\defeq \Ex{\li\in L}{ \indi{ f_{N_L(\li)} \neq g_{N_L(\li)}}} \\
	\dis(f,g) &\defeq \Ex{e\in E}{\indi{ f_e \neq g_e}} = \Ex{\li \in L}{\dis(f_{N_L(\li)},g_{N_L(\li)})} = \Ex{\ri \in R}{\dis(f_{N_R(\ri)},g_{N_R(\ri)})}\\
	\dis^R(f,g) &\defeq \Ex{\ri\in R}{ \indi{ f_{N_R(\ri)} \neq g_{N_R(\ri)}}} 
\end{align*}

\cref{thm:ael_distance} can then be stated in a simpler form as
\begin{theorem}[Restatement of \cref{thm:ael_distance}]
	$\dis^R(f,g) \geq \delta_0 - \frac{\lambda}{\dis^L(f,g)}$.
\end{theorem}
\subsection{Sum-of-Squares hierarchy}
%
The sum-of-squares hierarchy of semidefinite programs (SDPs) provides a family of increasingly
powerful convex relaxations for several optimization problems. 
%
Each ``level" $t$ of the hierarchy is parametrized by a set of constraints corresponding to
polynomials of degree at most $t$ in the optimization variables. While the relaxations in the
hierarchy can be viewed as  semidefinite programs of size $n^{O(t)}$ \cite{BS14, Laurent09}, 
it is often convenient to view the solution as a linear operator, called the ``pseudoexpectation" operator.
%
% It is well-known that such constrained pseudoexpectation operators of SoS-degree $t$ can be described as solutions to semidefinite programs of size $n^{O(t)}$ \cite{BS14, Laurent09}. This hierarchy of semidefinite programs for increasing $t$ is known as the SoS hierarchy.


%
%
\vspace{-5 pt}
%
\paragraph{Pseudoexpectations}
%
Let $t$ be an positive even integer and fix an alphabet $[q]$. An SoS solution of degree $t$, or a pseudoexpectation of SoS-degree $t$, over the variables $\zee = \{Z_{i,j}\}_{i\in[m],j\in[q]}$ is represented by a linear operator $ \tildeEx{\cdot}: \R[\zee]^{\leq t} \rightarrow \R$ such that:
%
\vspace{-5 pt}
%
\begin{enumerate}[(i)]
    \item $\tildeEx{1} = 1$.
    \item $\tildeEx{p^2} \geq 0$ if $p$ is a polynomial in $\zee = \{Z_{i,j}\}_{i\in [m],j\in [q]}$ of degree $\leq t/2$.
\end{enumerate}
%
\vspace{-5 pt}
%
 Note that linearity implies $\tildeEx{p_1} + \tildeEx{p_2} = \tildeEx{p_1+p_2}$ and $\tildeEx{c\cdot
  p_1} = c \cdot \tildeEx{p_1}$ for $c\in \R$, for $p_1, p_2 \in \R[\zee]^{\leq t}$.
%
This also allows for a succinct representation of $\tildeEx{\cdot}$ using any basis for $\R[\zee]^{\leq t}$.
%

The set of all pseudoexpectations should be seen as a relaxation for the set of all possible
(distributions over) assignments to $m$ variables in alphabet $[q]$.
%
%
Indeed, any assignment $f: [m] \rightarrow [q]$, can be seen as a pseudoexpectation 
which assigns the value $1$ to a
monomial consistent with $f$ and $0$ otherwise. This can be extended via linearity to all
polynomials, and then by convexity of the constraints to all distributions over assignments.
%
However, the reverse is not true when $t < m$, and there can be degree-$t$ pseudoexpectations which do
not correspond to any genuine distribution.

It is possible to optimize over the set of degree-$t$ pseudoexpectations in time $m^{O(t)}$ via SDPs
(under certain conditions on the bit-complexity of solutions~\cite{OD16, RW17:sos}).
%
We next define what it means for pseudoexpectations to satisfy some problem-specific constraints.

% Indeed, any assignment $f: [m] \rightarrow [q]$ has a corresponding pseudoexpectation described below.

% Let $z^{(f)}_{i,j} = \indi{f(i) = j}$, where $\indi{\cdot}$ is the $0/1$ indicator function. Then the pseudoexpectation corresponding to assignment $f$ is given by
% \begin{align*}
% 	\PExp^{(f)}[{p(\zee)}] = p\inparen{\inbraces{z^f_{i,j}}_{i\in[m],j\in[q]}}
% \end{align*}

% for every polynomial $p$ of degree at most $t$.

% As can be verified easily, the set of pseudoexpectations is convex, and so we can also extend this correspondence to distributions over assignments in a natural way. If $\PExp^{(\calD)}[{\cdot}]$ is the pseudoexpectation corresponding to a distribution $\calD$ over assignments, it holds that
% \[
% 	\PExp^{(\calD)}[{p(\zee)}] = \Ex{f\sim \calD}{p\inparen{\inbraces{z^f_{i,j}}_{i\in[m],j\in[q]}}}
% \]
% which explains the term pseudo-expectation.

% However, pseudoexpectations only exist for low-degree polynomials, and there can be pseudoexpectation operators that do not correspond to any genuine distribution over assignments. The main reason for working with pseudoexpectations instead of genuine distributions is that the set of SoS-degree $t$ can be optimized over in time $m^{O(t)}$ via SDPs.

% As a relaxation, pseudoexpectations are used in efficient algorithm design when coupled with
% suitable rounding algorithms. 
% %
% For such applications (including ours), it is important to look at relaxations that satisfy certain problem-specific constraints. We define next what it means for pseudoexpectations to satisfy constraints.

% \paragraph{Constrained Pseudoexpectations}
% %

\begin{definition}[Constrained Pseudoexpectations]\label{def:constraints_on_sos}
%	 
Let $\calS = \inbraces{f_1 = 0, \ldots, f_m = 0, g_1 \geq 0, \ldots, g_r \geq 0}$ be a system of
polynomial constraints, with each polynomial in $\calS$ of degree at most $t$. We say $\tildeEx{\cdot}$ is a pseudoexpectation operator respecting $\calS$, if in addition to the above conditions, it also satisfies
	%
	\begin{enumerate}
	\item $\tildeEx{p \cdot f_i} = 0$,  $\forall i \in [m]$ and $\forall p$ such that $\deg(p \cdot f_i) \leq t$.
	\item $\tildeEx{p^2 \cdot \prod_{i \in S} g_i} \geq 0$, $\forall S \subseteq [r]$ and $\forall p$ such that $\deg(p^2 \cdot \prod_{i \in S} g_i) \leq t$.
	\end{enumerate}
\end{definition}
%
%
\paragraph{Local constraints and local functions.}
%
Any constraint that involves at most $k$ variables from $\zee$, with $k\leq t$, can be written as a degree-$k$ polynomial, and such constraints may be enforced into the SoS solution.
%
% \paragraph{Canonical usage}
%
In particular, we will always consider the following canonical constraints on the variables $\zee$.
\ifnum\confversion=1
\begin{align*}
&Z_{i,j}^2 = Z_{i,j},\ \forall i\in[m],j\in[q] \\
\text{and} \quad &\sum_j Z_{i,j} = 1,\ \forall i\in[m] \mper
\end{align*}
\else
\[
Z_{i,j}^2 = Z_{i,j},\ \forall i\in[m],j\in[q] 
\quad \text{and} \quad 
\sum_j Z_{i,j} = 1,\ \forall i\in[m] \mper
\]
\fi
% As shown in the previous section, an assignment $f:[m]\rightarrow [q]$ is encoded using $m$ characteristic vectors, and so we wish to impose the following local constraints on the variables $\zee$:
%
% \begin{enumerate}[(i)]
% 	\item $Z_{i,j}^2 = Z_{i,j},\ \forall i\in[m],j\in[q]$.
% 	\item $\sum_j Z_{i,j} = 1,\ \forall i\in[m]$.
% \end{enumerate}
%
% These constraints are enforced as described in \cref{def:constraints_on_sos}, and we will henceforth not explicitly mention it. \snote{See Madhur's comment.}
%
We will also consider additional constraints and corresponding polynomials, defined by ``local" functions. For any $f\in [q]^m$ and $M\sub [m]$, we use $f_M$ to denote the restriction $f|_M$, and $f_i$ to denote $f_{\{i\}}$ for convenience.
%
\begin{definition}[$k$-local function]
	A function $\mu: [q]^m \rightarrow \R$ is called $k$-local if there is a set $M\subseteq [m]$ of size $k$ such that $\mu(f)$ only depends on $\inbraces{f(i)}_{i\in M}$, or equivalently, $\mu(f)$ only depends on $f|_M$.
	
	If $\mu$ is $k$-local, we abuse notation to also use $\mu: [q]^M \rightarrow \R$ with $\mu(\alpha) = \mu(f)$ for any $f$ such that $f|_M=\alpha$. It will be clear from the input to the function $\mu$ whether we are using $\mu$ as a function on $[q]^m$ or $[q]^M$.
\end{definition}

Let $\mu:[q]^m\rightarrow \R$ be a $k$-local function that depends on coordinates $M\subseteq [m]$ with $|M|=k$. Then $\mu$ can be written as a degree-$k$ polynomial $p_{\mu}$ in $\zee$:
\[
	p_{\mu}(\zee) = \sum_{\alpha \in [q]^M} \inparen{\mu(\alpha) \cdot\prod_{i\in M} Z_{i,\alpha_i}}
\]

% To see how $p_{\mu}$ is related to the $k$-local function $\mu$, observe that $p_{\mu}\inparen{\zee = \inbraces{z^{(f)}_{i,j}}} = \mu(f)$.

With some abuse of notation, we let $\mu(\zee)$ denote $p_{\mu}(\zee)$. We will use such $k$-local
functions inside $\tildeEx{\cdot}$ freely without worrying about their polynomial
representation. For example, $\tildeEx{ \indi{\zee_{i} \neq j}}$ denotes $\tildeEx{ 1- Z_{i,j}}$. 
%
% $\tildeEx{\cdot}$ operator applied to the polynomial corresponding to the $1$-local function $\mu: [q]^m \rightarrow \R$ which is defined as: $\mu(f)$ is $1$ if $f_i = 0$ and $\mu(f) = 0$ otherwise.
% %
The notion of $k$-local functions can also be extended from real valued functions to vector valued functions in a straightforward way.

\begin{definition}[vector-valued local functions]
A function $\mu: [q]^m \rightarrow \R^N$ is $k$-local if the $N$ real valued functions corresponding to the $N$ coordinates are all $k$-local. Note that these different coordinate functions may depend on different sets of variables, as long as the number is at most $k$ for each of the functions.
\end{definition}
%
\vspace{-5 pt}
%
\paragraph{Local distribution view of SoS}

It will be convenient to use a shorthand for the function $\indi{\zee_S = \alpha}$, and we will use $\zee_{S,\alpha}$. Likewise, we use $\zee_{i,j}$ as a shorthand for the function $\indi{\zee_i = j}$. That is, henceforth,
\ifnum\confversion=1
\begin{align*}
	&\tildeEx{\zee_{S,\alpha}} = \tildeEx{\indi{\zee_S = \alpha}} = \tildeEx{ \prod_{s\in S}
                                    Z_{s,\alpha_s}}  \\
	\text{and } \quad & \tildeEx{\zee_{i,j}} = \tildeEx{\indi{\zee_i = j}} = \tildeEx{ Z_{i,j}}.
\end{align*}
\else
\begin{align*}
	\tildeEx{\zee_{S,\alpha}} ~=~ \tildeEx{\indi{\zee_S = \alpha}} = \tildeEx{ \prod_{s\in S}
                                    Z_{s,\alpha_s}} 
\qquad \text{and} \qquad
	\tildeEx{\zee_{i,j}} ~=~ \tildeEx{\indi{\zee_i = j}} = \tildeEx{ Z_{i,j}}
\end{align*}
\fi

% Note that for any degree-$t$ pseudoexpectation operator $\tildeEx{\cdot}$ with $t\geq 2$,
% \[
% 	\sum_{j\in [q]} \tildeEx{\zee_{i,j}} = \sum_{j} \tildeEx{Z_{i,j}} = \tildeEx{\sum_j Z_{i,j}}= 1
% \qquad \text{and} \qquad
% 	\tildeEx{\zee_{i,j}} = \tildeEx{Z_{i,j}} = \tildeEx{Z_{i,j}^2} \geq 0
% \]
% Thus, the real values $\inbraces{\tildeEx{\zee_{i,j}}}_{j\in [q]}$ define a distribution over $[q]$
% , which we will sometimes call local distribution for $\zee_i$. 

% In fact, this argument can be extended to define local distributions for $\zee_S$ for $|S|\leq
% t/2$. Let $S \subseteq [m]$ be such that $|S|=k\leq t/2$,
Note that for any $S \subseteq [m]$ with $\abs{S} = k \leq t/2$,
\ifnum\confversion=1
\begin{gather*}
	\sum_{ \alpha \in [q]^{k}} \tildeEx{\zee_{S,\alpha}} = 
% \sum_{ \alpha \in [q]^{k}} \tildeEx{ \prod_{s\in S} Z_{s,\alpha_s}} 
 \tildeEx{ \prod_{s\in S} \inparen{ \sum_{j\in [q]} Z_{s,j}} } = 1
\\
	\tildeEx{\zee_{S,\alpha}} = \tildeEx{ \prod_{s\in S} Z_{s,\alpha_s}} = \tildeEx{ \prod_{s\in
            S} Z^2_{s,\alpha_s}} \geq 0 \mper
\end{gather*}
\else
\[
	\sum_{ \alpha \in [q]^{k}} \tildeEx{\zee_{S,\alpha}} = 
% \sum_{ \alpha \in [q]^{k}} \tildeEx{ \prod_{s\in S} Z_{s,\alpha_s}} 
 \tildeEx{ \prod_{s\in S} \inparen{ \sum_{j\in [q]} Z_{s,j}} } = 1
\qquad \text{and} \qquad
	\tildeEx{\zee_{S,\alpha}} = \tildeEx{ \prod_{s\in S} Z_{s,\alpha_s}} = \tildeEx{ \prod_{s\in
            S} Z^2_{s,\alpha_s}} \geq 0 \mper
\]
\fi
Thus, the values $\inbraces{\tildeEx{\zee_{S, \alpha}}}_{\alpha\in [q]^S}$ define a distribution
over $[q]^k$, referred to as the local  distribution for $\zee_S$.

% which we think of as the local distribution for $\zee_S$.
%
% Given a distribution $\calD$ over assignments in $[q]^m$, the local distribution induced by $\PExp^{(\calD)}[\cdot]$ on $\zee_S$ is precisely the marginal distribution induced by $\calD$ for the set $S$. In this view, degree-$t$ pseudoexpectations give us consistent marginal distributions over sets of size at most $t/2$ that may not correspond to any global distribution, and allow us to optimize over this set in time $m^{\calO(t)}$.
%
Let $\mu: [q]^m \rightarrow\R$ be a $k$-local function for $k\leq t/2$, depending on $M \subseteq
[m]$. Then, $\tildeEx{\mu(\zee)}$ can be seen as the expected value of the function $\mu$ under the
local distribution for $M$, since
%
\ifnum\confversion=1
\begin{align*}
	\tildeEx{\mu(\zee)} 
~=~& \tildeEx{\sum_{\alpha\in [q]^M} \inparen{\mu(\alpha) \cdot\prod_{i\in M} Z_{i,\alpha_i}}}\\
~=~& \sum_{\alpha\in [q]^M} \mu(\alpha) \cdot \tildeEx{\prod_{i\in M} Z_{i,\alpha_i}}\\
~=~& \sum_{\alpha\in [q]^M} \mu(\alpha) \cdot \tildeEx{\zee_{M,\alpha}} \mper
\end{align*}
\else
\begin{align*}
	\tildeEx{\mu(\zee)} 
~=~ \tildeEx{\sum_{\alpha\in [q]^M} \inparen{\mu(\alpha) \cdot\prod_{i\in M} Z_{i,\alpha_i}}}
~=~ \sum_{\alpha\in [q]^M} \mu(\alpha) \cdot \tildeEx{\prod_{i\in M} Z_{i,\alpha_i}}
~=~ \sum_{\alpha\in [q]^M} \mu(\alpha) \cdot \tildeEx{\zee_{M,\alpha}} \mper
\end{align*}
\fi
%

\begin{claim}
	Let $\tildeEx{\cdot}$ be a degree-$t$ pseudoexpectation. For $k \leq t/2$, let $\mu_1,\mu_2$
        be two $k$-local functions on $[q]^m$, depending on the same set of coordinates $M$, and
        $\mu_1(\alpha) \leq \mu_2(\alpha) ~~\forall \alpha \in [q]^M$. Then $\tildeEx{\mu_1(\zee)} \leq \tildeEx{\mu_2(\zee)}$.
%
 % Suppose that for any $\alpha\in [q]^M$, $\mu_1(\alpha) \leq \mu_2(\alpha)$. Then
 %        \[
 %        	\tildeEx{\mu_1(\zee)} \leq \tildeEx{\mu_2(\zee)}
 %        \]
\end{claim}

\begin{proof}
Let $\calD_M$ be the local distribution induced by $\tildeEx{\cdot}$ for $\zee_M$. Then
$\tildeEx{\mu_1(\zee)} = \Ex{\alpha \sim \calD_M}{\mu_1(\alpha)}$, and $\tildeEx{\mu_2(\zee)} =
\Ex{\alpha\sim \calD_M}{\mu_2(\alpha)}$, which implies $\tildeEx{\mu_1(\zee)} \leq \tildeEx{\mu_2(\zee)}$.
%
% Since $\mu_1(\alpha) \leq \mu_2(\alpha)$ for every $\alpha\in [q]^M$, 
% \[
% 	\Ex{\alpha \sim \calD_M}{\mu_1(\alpha)} \leq \Ex{\alpha\sim \calD_M}{\mu_2(\alpha)}
% \]
% and so,
% \[
% 	\tildeEx{\mu_1(\zee)} \leq \tildeEx{\mu_2(\zee)}
% \]
\end{proof}
%
The previous claim allows us to replace any local function inside $\tildeEx{\cdot}$ by another local function that dominates it. We will make extensive use of this fact.
%
%
\vspace{-5 pt}
\paragraph{Covariance for SoS solutions}
Given two sets $S,T \sub [m]$ with $|S|,|T|\leq k/4$, we can define the covariance between indicator random variables of $\zee_S$ and $\zee_T$ taking values $\alpha$ and $\beta$ respectively, according to the local distribution over $S \cup T$. This is formalized in the next definition.
\begin{definition}
Let $\tildeEx{\cdot}$ be a pseudodistribution operator of SoS-degree-$t$, and $S,T$ are two sets of
size at most $t/4$, and $\alpha\in [q]^S$, $\beta\in [q]^T$, we define the pseudo-covariance and
pseudo-variance,
%
\ifnum\confversion=1
\small
\begin{gather*}
\tildecov(\zee_{S,\alpha},\zee_{T,\beta}) 
= \tildeEx{ \zee_{S,\alpha} \cdot \zee_{T,\beta} } - \tildeEx{\zee_{S,\alpha}} \tildeEx{\zee_{T,\beta}} \\	
\tildeVar{\zee_{S,\alpha}} ~=~ \tildecov(\zee_{S,\alpha},\zee_{S,\alpha})
\end{gather*}
\normalsize
\else
\begin{align*}
\tildecov(\zee_{S,\alpha},\zee_{T,\beta}) 
~=~ \tildeEx{ \zee_{S,\alpha} \cdot \zee_{T,\beta} } - \tildeEx{\zee_{S,\alpha}} \tildeEx{\zee_{T,\beta}}
\qquad \text{and} \qquad		
\tildeVar{\zee_{S,\alpha}} ~=~ \tildecov(\zee_{S,\alpha},\zee_{S,\alpha})
\end{align*}
\fi
%
The above definition is extended to pseudo-covariance and pseudo-variance for pairs of sets $S,T$, 
as the sum of absolute value of pseudo-covariance for all pairs $\alpha,\beta$ :
%
\ifnum\confversion=1
\begin{gather*}
\tildecov(\zee_S,\zee_T) 
~=~ \sum_{\alpha\in [q]^S \atop \beta\in [q]^T} \abs{ \tildecov(\zee_{S,\alpha},\zee_{T,\beta}) } \\
\tildeVar{\zee_S} ~=~ \sum_{\alpha\in [q]^S} \abs{ \tildeVar{\zee_{S,\alpha} } }
\end{gather*}
\else
\[
\tildecov(\zee_S,\zee_T) 
~=~ \sum_{\substack{\alpha\in [q]^S \\ \beta\in [q]^T}} \abs{ \tildecov(\zee_{S,\alpha},\zee_{T,\beta}) }
\qquad \text{and} \qquad		
\tildeVar{\zee_S} ~=~ \sum_{\alpha\in [q]^S} \abs{ \tildeVar{\zee_{S,\alpha} } }
\]
\fi
%
\end{definition}

% These definitions can be extended to pseudocovariances and pseudo-variances for pairs of sets $S,T$ with $|S|,|T|\leq t/4$ as the sum of absolute value of pseudocovariance for all pairs $\alpha,\beta$.
% \begin{definition}
% Let $\tildeEx{\cdot}$ be a pseudodistribution operator of SoS-degree-$t$, and $S,T$ are two sets of size at most $t/4$, we define the pseudo-covariance between $\zee_S$ and $\zee_T$ as,
% 	\begin{align*}
% 		\tildecov(\zee_S,\zee_T) = \sum_{\alpha\in [q]^S,\beta\in [q]^T} \abs{ \tildecov(\zee_{S,\alpha},\zee_{T,\beta}) }
% 	\end{align*}
% We also define the analogous pseudovariance as,
% 	\begin{align*}
% 		\tildeVar{\zee_S} = \sum_{\alpha\in [q]^S} \abs{ \tildeVar{\zee_{S,\alpha} } }
% 	\end{align*}
% \end{definition}
%
We will need the fact that $\tildeVar{\zee_S}$ is bounded above by 1, since,
%
\ifnum\confversion=1
\begin{align*}
\tildeVar{\zee_S} 
&~=~ \sum_{\alpha} \abs{\tildeVar{\zee_{S,\alpha}}} \\
&~=~ \sum_{\alpha}\inparen{
          \tildeEx{\zee_{S,\alpha}^2} - \tildeEx{\zee_{S,\alpha}}^2} \\
&~\leq~ \sum_{\alpha} \tildeEx{\zee_{S,\alpha}^2} \\
&~=~ \sum_{\alpha} \tildeEx{\zee_{S,\alpha}} 
~=~ 1
\end{align*}
\else
\[
\tildeVar{\zee_S} 
~=~ \sum_{\alpha} \abs{\tildeVar{\zee_{S,\alpha}}} 
~=~ \sum_{\alpha}\inparen{
          \tildeEx{\zee_{S,\alpha}^2} - \tildeEx{\zee_{S,\alpha}}^2} 
~\leq~ \sum_{\alpha} \tildeEx{\zee_{S,\alpha}^2} 
~=~ \sum_{\alpha} \tildeEx{\zee_{S,\alpha}} 
~=~ 1
\]
\fi

% \begin{claim}\quad	$\tildeVar{\zee_S} \leq 1$.
% \end{claim}
% %
% \begin{proof}
% \begin{align*}
% 	\tildeVar{\zee_S} &= \sum_{\alpha} \abs{\tildeVar{\zee_{S,\alpha}}} = \sum_{\alpha}\inparen{ \tildeEx{\zee_{S,\alpha}^2} - \tildeEx{\zee_{S,\alpha}}^2} \leq \sum_{\alpha} \tildeEx{\zee_{S,\alpha}^2} = \sum_{\alpha} \tildeEx{\zee_{S,\alpha}} = 1
% \end{align*}
% \end{proof}
%
\vspace{-5 pt}
\paragraph{Conditioning SoS solutions.}
%
We will also make use of conditioned pseudoexpectation operators, which may be defined in a way
similar to usual conditioning for true expectation operators, as long as the event we condition on
is local. 
%
The conditioned SoS solution is of a smaller degree, but continues to respect the constraints that original solution respects.

\begin{definition} Let $F \subseteq [q]^m$ be subset (to be thought of as an event) such that $\one_F:[q]^m \rightarrow \{0,1\}$ is a $k$-local function. Then for every $t>2k$, we can condition a pseudoexpectation operator of SoS-degree $t$ on $F$ to obtain a new conditioned pseudoexpectation operator $\condPE{\cdot}{E}$ of SoS-degree $t-2k$, as long as $\tildeEx{\one^2_F(\zee)}>0$. The conditioned SoS solution is given by
\[
	\condPE{ p(\zee)}{F(\zee) } \defeq \frac{\tildeEx{p(\zee) \cdot \one^2_{F}(\zee)}}{\tildeEx{\one^2_{F}(\zee)}}
\]
where $p$ is any polynomial of degree at most $t-2k$.
\end{definition}

We can also define pseudocovariances and pseudo-variances for the conditioned SoS solutions.
\begin{definition}
	Let $F\sub [q]^m$ be an event such that $\one_F$ is $k$-local, and let $\tildeEx{\cdot}$ be a pseudoexpectation operator of degree $t$, with $t>2k$. Let $S,T$ be two sets of size at most $\frac{t-2k}{2}$ each. Then the pseudocovariance between $\zee_{S,\alpha}$ and $\zee_{T,\beta}$ for the solution conditioned on event $F$ is defined as,
\ifnum\confversion=1
\begin{multline*}
\tildecov(\zee_{S,\alpha},\zee_{T,\beta} \vert F) = \\
\tildeEx{ \zee_{S,\alpha} \zee_{T,\beta} \vert F} - \tildeEx{\zee_{S,\alpha} \vert F} \tildeEx{\zee_{T,\beta} \vert F}
\end{multline*}
\else
\begin{align*}
\tildecov(\zee_{S,\alpha},\zee_{T,\beta} \vert F) 
~=~ \tildeEx{ \zee_{S,\alpha} \zee_{T,\beta} \vert F} - \tildeEx{\zee_{S,\alpha} \vert F} \tildeEx{\zee_{T,\beta} \vert F}
\end{align*}
\fi
\end{definition}

We also define the pseudocovariance between $\zee_{S,\alpha}$ and $\zee_{T,\beta}$ after
conditioning on a random assignment for some $\zee_V$ with $V\sub [m]$. 
%
Note that here the random assignment for $\zee_V$ is chosen according to the local distribution for
the set $V$.

\begin{definition}[Pseudocovariance for conditioned pseudoexpectation operators]
\ifnum\confversion=1
\begin{multline*}
\tildecov(\zee_{S,\alpha},\zee_{T,\beta} \vert \zee_V) 
= \\ \sum_{\gamma \in [q]^V}   \tildecov(\zee_{S,\alpha},\zee_{T,\beta} \vert \zee_V = \gamma) \cdot \tildeEx{\zee_{V,\gamma}}
	\end{multline*}
\else
\begin{align*}
\tildecov(\zee_{S,\alpha},\zee_{T,\beta} \vert \zee_V) 
~=~ \sum_{\gamma \in [q]^V}   \tildecov(\zee_{S,\alpha},\zee_{T,\beta} \vert \zee_V = \gamma) \cdot \tildeEx{\zee_{V,\gamma}}
\end{align*}
\fi
\end{definition}

And we likewise define $\tildeVar{\zee_{S,\alpha} \vert \zee_V}$, $\tildecov(\zee_S, \zee_T \vert \zee_V)$ and $\tildeVar{\zee_S \vert \zee_V}$.

\subsection{SoS relaxations for codes}
%
For both Tanner codes and AEL codes, we will identify $[m]$ with $E$ so that the SoS solutions will be relaxations to the assignments to edges of a bipartite $(n,d,\lambda)$-expander.

\paragraph{Pseudocodewords for Tanner Codes}

Let $G(L,R,E)$ be the bipartite $(n,d,\lambda)$-expander on which the Tanner code is defined, and let $\calC_0\subseteq [q]^d$ be the inner code. The SoS variables will be $\zee = \{Z_{e,j}\}_{e\in E,j\in [q]}$. 

\begin{definition}[Tanner Pseudocodewords]
For $t\geq 2d$, we define a degree-$t$ Tanner pseuocodeword to be a degree-$t$ pseudoexpectation operator $\tildeEx{\cdot}$ on $\zee$ respecting the following constraints:
%
\ifnum\confversion=1
\begin{align*}
&\forall \li \in L, \quad \zee_{N_L(\li)} \in \calC_0 \\
\text{and } \quad &\forall \ri \in R,\quad \zee_{N_R(\ri)} \in\calC_0
\end{align*}
\else
\begin{align*}
\forall \li \in L, \quad \zee_{N_L(\li)} \in \calC_0 
\qquad \text{and} \qquad          
\forall \ri \in R,\quad \zee_{N_R(\ri)} \in\calC_0
\end{align*}
\fi
%
Again, since these constraints are $d$-local, it is sufficient to enforce that certain degree-$d$ polynomials are zero (respected by pseudoexpectation) to enforce these constraints. 
%
In particular, each parity check in the parity check matrix of $\calC_0$ will correspond to a monomial of size at most $d$ that we can enforce to be equal to 1.
\end{definition}

We can also define a generalization of distance between two codewords to include pseudocodewords.
%
\begin{definition}[Distance from a pseudocodeword]
%
The distance between a pseudocodeword $\tildeEx{\cdot}$ of SoS-degree $t\geq 2d$ and a codeword $h$ of $\TanC$ is defined as
\ifnum\confversion=1
\begin{align*}
\dis(\tildeEx{\cdot},h) 
~\defeq~& \Ex{e\in E}{\tildeEx{\indi{\zee_e \neq h_e}}} \\
~=~& \Ex{\li\in L}{\tildeEx{\dis(\zee_{N_L(\li)},  h_{N_L(\li)})}}
\end{align*}
\else
\[
\dis(\tildeEx{\cdot},h) 
~\defeq~ \Ex{e\in E}{\tildeEx{\indi{\zee_e \neq h_e}}} 
~=~ \Ex{\li\in L}{\tildeEx{\dis(\zee_{N_L(\li)},  h_{N_L(\li)})}}
\]
\fi
\end{definition}

\paragraph{Pseudocodewords for AEL}

Let $G(L,R,E)$ be the bipartite $(n,d,\lambda)$-expander on which the AEL code is defined, and let $\calC_0\subseteq [q_0]^d$ be the inner code. The SoS variables will be $\zee = \{Z_{e,j}\}_{e\in E,j\in [q_0]}$. 

\begin{definition}[AEL Pseudocodewords]
	For $t\geq 2d$, we define a degree-$t$ AEL pseuocodeword to be a degree-$t$ pseudoexpectation operator $\tildeEx{\cdot}$ on $\zee$ respecting the following constraints:
	\begin{align*}
		\forall \li \in L,\quad \zee_{N_L(\li)} \in \calC_0
	\end{align*}
\end{definition}

Next we define the distances between a pseudocodeword and a codeword of $\AELC$. 
\begin{definition}[Distance from a pseudocodeword]
	The left, middle and right distances between a pseudocodeword $\tildeEx{\cdot}$ of SoS-degree $t\geq 2d$ and a codeword $h \in \AELC$ are defined as
	\begin{align*}
		\dis^L(\tildeEx{\cdot},h) &\defeq \Ex{\li}{\tildeEx{\indi{\zee_{N_L(\li)} \neq h_{N_L(\li)}}}} \\
	\dis(\tildeEx{\cdot},h) &\defeq \Ex{e}{\tildeEx{\indi{\zee_e \neq h_e}}} \\
		\dis^R(\tildeEx{\cdot},h) &\defeq \Ex{\ri\in R}{\tildeEx{\indi{\zee_{N_R(\ri)}\neq  h_{N_R(\ri)}}}}
	\end{align*}
\end{definition}
%
%It will be convenient to look at AEL codewords as triplets $(h^L,h,h^R)$, where $h^L\in [q_0^d]^L$, $h\in [q_0]^E$ and $h^R=[q_0^d]^R$ which satisfy $h^L_{\li} = h_{N_L(\li)}$ and $h^R_{\ri} = h_{N_R(\ri)}$. These are shorthands for same object (from the left, middle or right), and knowing one of them is enough to deduce the other two. 
%We also define two additional distance functions to measure distances from left or middle:
%\ifnum\confversion=1
%\begin{align*}
%	
%\end{align*}
%\else
%\begin{align*}
%	\dis^L(\tildeEx{\cdot},h) = \Ex{\li}{\tildeEx{\indi{\zee_{N_L(\li)} \neq h_{N_L(\li)}}}} \qquad \text{and} \qquad \dis(\tildeEx{\cdot},h) = \Ex{e}{\tildeEx{\indi{\zee_e \neq h_e}}}
%\end{align*}
%\fi

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> intro/csp.tex <==
\subsection{Preliminaries}

\subsubsection{Simplicial Complexes}\label{subsec:complexes}

It will be convenient to work with hypergraphs satisfying a certain
downward-closed property (which is straightforward to obtain).

\begin{definition}
A {\deffont simplicial complex} $X$ with ground set $[n]$ is a
downward-closed collection of subsets of $[n]$, \ie for all sets $\ess
\in X$ and $\tee \subseteq \ess$, we also have $\tee \in X$. The sets
in $X$ are referred to as {\deffont faces} of $X$.
%
We use the notation $X(i)$ for the set of all faces of a simplicial
complex $X$ with cardinality $i$ and $X(\leq d)$ for the set of all
faces of cardinality at most $d$.~\footnote{Note that it is more
  common to associate a geometric representation to simplicial
  complexes, with faces of cardinality $i$ being referred to as faces
  of \emph{dimension} $i-1$ (and the collection being denoted by
  $X(i-1)$ instead of $X(i)$). However, we prefer to index faces by
  their cardinality to improve readability of related expressions.}
By convention, we take $X(0) := \set{\varnothing}$.

A simplicial complex $X(\leq d)$ is said to be a {\deffont pure
  simplicial complex} if every face of $X$ is contained in some face
of size $d$. Note that in a pure simplicial complex $X(\leq d)$, the
top slice $X(d)$ completely determines the complex.
\end{definition}

Simplicial complexes are equipped with the following probability
measures on their sets of faces.

\begin{definition}[Probability measures $(\Pi_1, \ldots, \Pi_d)$]
Let $X(\leq d)$ be a pure simplicial complex and let $\Pi_d$ be an arbitrary probability measure on
$X(d)$. We define a coupled array of random variables $(\ess^{(d)}, \ldots,
\ess^{(1)})$ as follows: sample $\ess^{(d)} \sim \Pi_d$ and (recursively) for
each $i \in [d]$, take $\ess^{(i-1)}$ to be a uniformly random subset of
$\ess^{(i)}$ of size $i-1$.
The distributions $\Pi_{d-1}, \ldots, \Pi_1$ are then defined to be the marginal
distributions of the random variables $\ess^{(d-1)}, \ldots, \ess^{(1)}$. We also define
the joint distribution of $(\ess^{(d)}, \ldots, \ess^{(1)})$ as $\Pi$.
Note that the choice of $\Pi_d$ determines each other distribution $\Pi_i$ on $X(i)$.
\end{definition}

In order to work with the HDX and expander walk instantiations in a
unified manner, we will use also use the notation $X(k)$ to indicate
the set of all length $k-1$ walks on a graph $G$. In this case, $X(k)$
is a set of $k$-tuples rather than subsets of size $k$.  This
distinction will be largely irrelevant, but we will use $W_G(k)$ when
referring specifically to walks rather than subsets.  The set of walks
$W_G(k)$ has a corresponding distribution $\Pi_k$ as well (see
\cref{def:walk_collection}).

%\subsubsection{Codes and Lifts}
%
\subsubsection{Codes}

We briefly recall some standard code terminology. Let $\Sigma$ be a
finite alphabet with $q \in \mathbb{N}$ symbols. We will be mostly
concerned with the case $\Sigma=\mathbb{F}_2$. Given $z,z' \in
\Sigma^n$, recall that the relative Hamming distance between $z$ and
$z'$ is \text{$\Delta(z,z') \coloneqq \abs{\set{i \mid z_i\ne
      z_i'}}/n$}. Any set $\Cc \subset \Sigma^n$ gives rise to a
$q$-ary code. The distance of $\Cc$ is defined as $\Delta(\Cc)
\coloneqq \min_{z\ne z'} \Delta(z,z')$ where $z,z' \in \Cc$. We say
that $\Cc$ is a linear code~\footnote{In this case, $q$ is required to
  be a prime power.}  if $\Sigma = \mathbb{F}_q$ and $\Cc$ is a linear
subspace of $\mathbb{F}_q^n$. The rate of $\Cc$ is
$\log_q(\abs{\Cc})/n$.

Instead of discussing the distance of a binary code, it will often be more natural to phrase results in terms of its bias.

\begin{definition}[Bias]
  The {\deffont bias} of a word~\footnote{Equivalently, the bias of $z \in \{\pm 1\}^n$ is $\bias(z) \coloneqq \abs{\E_{i \in [n]} z_i}$.}
  $z \in \F_2^n$ is $\bias(z) \coloneqq \abs{\E_{i \in [n]} (-1)^{z_i}}$. The bias of a code $\Cc$ is the
  maximum bias of any non-zero codeword in $\Cc$.
\end{definition}

\subsubsection{Lifts} \label{subsec:lifts}

Starting from a code $\Cc_1 \subset \Sigma^{X(1)}_1$, we amplify its
distance by considering a \textit{lifting} operation defined as
follows.

\begin{definition}[Lifting Function]
Let $g: \Sigma_1^k \to \Sigma_k$ and $X(k)$ be a collection of $k$-uniform hyperedges or walks of length $k-1$ on the set $X(1)$.
For $z \in \Sigma_1^{X(1)}$, we define $\lift_{X(k)}^g(z) = y$ such that $y_{\ess} = g(z\vert_{\ess})$ for all $\ess \in X(k)$, where $z\vert_{\ess}$ is the restriction of $z$ to the indices in $\ess$.

The lifting of a code $\mathcal C_1 \subseteq \Sigma_1^{X(1)}$ is
	$$\lift_{X(k)}^g(\mathcal C_1) = \{\lift_{X(k)}^g(z) \mid z \in \mathcal C_1\},$$
which we will also denote $\mathcal C_k$.
We will omit $g$ and $X(k)$ from the notation for lifts when they are clear from context.
\end{definition}

We will call liftings that amplify the distance of a code \emph{robust}.
\begin{definition}[Robust Lifting]\label{def:lift_rob}
  We say that $\lift_{X(k)}^g$ is $(\delta_0,\delta)$-robust
  if for every $z,z' \in \Sigma_1^{X(1)}$ we have
  $$
  \Delta(z,z') \ge \delta_0 \implies \Delta(\lift(z), \lift(z')) \ge \delta.
  $$
\end{definition}

For us the most important example of lifting is when the function $g$
is \text{$k$-XOR} and $\Sigma_1=\Sigma_k=\mathbb{F}_2$, which has been
extensively studied in connection with codes and
otherwise~\cite{Ta-Shma17, STV99, GNW95, ABNNR92}. In our language of
liftings, $k$-XOR corresponds to the \emph{direct sum lifting}.

\begin{definition}[Direct Sum Lifting]
 Let $\mathcal C_1 \subseteq \F_2^n$ be a base code on $X(1) = [n]$.
 The {\deffont direct sum lifting} of a word $z \in \F_2^n$ on a
 collection $X(k)$ is $\dsum_{X(k)}(z) = y$ such that $y_{\ess} = \sum_{i \in \ess} z_i$ 
 for all $\ess \in X(k)$.
\end{definition}

We will be interested in cases where the direct sum lifting reduces
the bias of the base code; in~\cite{Ta-Shma17}, structures with such a
property are called parity samplers, as they emulate the reduction in
bias that occurs by taking the parity of random samples.

\begin{definition}[Parity Sampler]
  Let $g \colon \mathbb{F}_2^k \to \mathbb{F}_2$. We say that
    $\lift_{X(k)}^g$ is an $(\epsilon_0, \epsilon)$-parity sampler if
  for all $z \in \F_2^{X(1)}$ with $\bias(z) \leq \epsilon_0$, we have
  $\bias(\lift(z)) \leq \epsilon$.
\end{definition}

\subsubsection{Constraint Satisfaction Problems (CSPs)}
%
A $k$-CSP instance $\Ins(H, \Pred, w)$ with alphabet size $q$
consists of a $k$-uniform hypergraph $H$, a set of constraints 
\[ \Pred= \set*{ \Pred_\aye \subseteq [q]^{\aye} : \aye \in H},\]
and a non-negative weight function $w \in \RR_+^H$ on the
constraints satisfying $\sum_{\aye \in H}w(a) = 1$.
% Here, each set $\Cc_{\aye}$ can be thought of
% as the set of satisfying assignments to the constraint on the variables in $\aye$.

We will think of the constraints as predicates that are satisfied by an assignment
$\assn$ if we have $\assn|_{\aye} \in \Pred_\aye$,
\ie~the restriction of $\assn$ on $\aye$ is contained in
$\Pred_\aye$. We write $\SAT_\Ins(\assn)$ for the (weighted) fraction
of the constraints satisfied by the assignment $\assn$, \ie
\[ 
\SAT_\Ins(\assn) 
~=~ \sum_{\aye \in H} w(\aye) \cdot \one[\assn|_\aye \in \Pred_\aye] 
~=~ \Ex{\aye \sim w}{\one[\assn|_\aye \in \Pred_\aye]}
\mper
\]
We denote by $\OPT(\Ins)$ the maximum of $\SAT_\Ins(\assn)$ over all
$\assn \in [q]^{V(H)}$.

A particularly important class of $k$-CSPs for our work will be
$k$-XOR: here the input consists of a $k$-uniform hypergraph $H$ with
weighting $w$, and a (right hand side) vector $r \in \FF_2^H$. The
constraint for each $\aye \in H$ requires
\[ \sum_{i \in \aye} \sigma(i) = r_\aye \pmod{2}.\]
In this case we will use the notation $\Ins(H, r, w)$ to refer to the
$k$-XOR instance. When the weighting $w$ is implicitly clear, we will
just omit it and write $\Ins(H, r)$. 

%
%
Any $k$-uniform hypergraph $H$ can be associated with a pure
simplicial complex in a canonical way by just setting $X_{\Ins} = \set*{\bee
  : \exists\ \aye \in H ~\text{and}~ \aye \supseteq \bee }$; notice that
$X_{\Ins}(k) = H$. 
%
We will refer to this complex as the {\deffont constraint complex} of the instance $\Ins$.
%
The probability distribution $\Pi_{k}$ on
$X_{\Ins}$ will be derived from the weight function $w$ of the
constraint:
\[ \Pi_{k}(\aye) = w(\aye) \quad\forall \aye \in X_{\Ins}(k) = H.\]

\subsection{Unique Decoding}

The main result here is that if the CSP corresponding to the direct sum can be approximated arbitrarily well, and the lifting is distance amplifying in a sufficiently strong sense, then we can unique decode from a certain radius. This radius may not be the true unique decoding radius of the lifted code, but it is possible to take the decoding radius arbitrarily close to 1/4 by assuming sufficiently strong parity sampling.
%
%\subsection{Unique Decoding on Parity Samplers}

Our approach to unique decoding for $\Cc_k$ is as follows.
Suppose a received word $\tilde y \in \F_2^{X(k)}$ is close to $y^\star \in \Cc_k$, which is the direct sum lifting of some $z^\star \in \Cc_1$ on $X(k)$.
We first find an approximate solution $z \in \F_2^n$ to the $k$-XOR instance $\Ins(X(k), \tilde y)$ with predicates
	\[ \sum_{i  \in \ess} z_{i}  = {\tilde y}_\ess \pmod 2 \]
for every $\ess \in X(k)$.
Note that $z$ being an approximate solution to $\Ins(X(k), \tilde y)$ is equivalent to its lifting $\dsum_{X(k)}(z)$ being close to $\tilde y$.
In \cref{lem:robust-approx-ud}, we show that if $\dsum_{X(k)}$ is a sufficiently strong parity sampler, either $z$ or its complement $\conj{z}$ will be close to $z^\star$.
Running the unique decoding algorithm for $\Cc_1$ on $z$ and $\conj{z}$ will recover $z^\star$, from which we can obtain $y^\star$ by applying the direct sum lifting.

\begin{lemma}\label{lem:robust-approx-ud}
    Let $0 < \beta  < 1/2$ and $0 < \epsilon < 1/4-\beta/2$. Suppose $\Cc_1$ is a
    linear code that is efficiently uniquely
    decodable within radius $1/4 - \mu_0$ for some $\mu_0 >
    0$, and $\Cc_k = \dsum_{X(k)}(\Cc_1)$ where $\dsum_{X(k)}$ is a
    $(1/2+2\mu_0, 2\beta)$-parity sampler. Let $\tilde
    y \in \FF_2^{X(k)}$ be a word that has distance strictly less than $(1/4 - \beta/2 - \epsilon)$
    from $\Cc_k$, and let $y^\star = \dsum_{X(k)}(z^\star) \in \Cc_k$ be the word closest to $\tilde y$.
    
    Then, for any $z \in \FF_2^n$ satisfying
        $$\Delta(\dsum_{X(k)}(z), \tilde y) < \frac{1}{4} - \frac{\beta}{2},$$
    we have either
    \[ \Delta(z^\star,z) \le \frac{1}{4} - \mu_0 ~~\textrm{ or
    }~~\Delta(z^\star,\conj{z}) \le \frac{1}{4} - \mu_0.\]
    In particular, either $z$ or $\conj{z}$ can be efficiently
    decoded in $\Cc_1$ to obtain $z^\star \in \Cc_1$.
\end{lemma}

\begin{remark}
    Since $\dsum_{X(k)}$ is a $(1/2 + 2\mu_0, 2\beta)$-parity sampler, the code
    $\Cc_k$ has distance $\Delta(\Cc_k) \ge 1/2 - \beta$. This implies that $z^\star \in \Cc_1$
    is unique, since its direct sum lifting $y^\star$ is within distance $\Delta(\Cc_k)/2$ of $\tilde y$.
\end{remark}

\begin{proof}
  Let $y = \dsum_{X(k)}(z)$. We have
  $$
  \Delta(y^\star, y) \leq \Delta(y^\star, \tilde y) + \Delta(y, \tilde y) < \frac 12 - \beta.
  $$
  By linearity of $\dsum_{X(k)}$, $\Delta(\dsum_{X_k}(z^\star-z),0) < 1/2-\beta$, so $\bias(\dsum_k(z^\star-z)) > 2\beta$.
  From the $(1/2+2\mu_0, 2\beta)$-parity sampling assumption, $\bias(z^\star-z) > 1/2 + 2\mu_0$.
  Translating back to distance, either $\Delta(z^\star, z) < 1/4 - \mu_0$ or $\Delta(z^\star, z) > 3/4 + \mu_0$,
  the latter being equivalent to $\Delta(z^\star, \conj{z}) < 1/4-\mu_0$.
\end{proof}

To complete the unique decoding algorithm, we need only describe how a
good enough approximate solution $z \in \mathbb{F}_2^n$ to a $k$-XOR
instance $\Ins(X(k), \tilde y)$ allows us to recover $z^{\star} \in \Cc_1$
provided $\tilde y$ is sufficiently close to $\Cc_k$. We will rely on the
following observation relating satisfiability and distance.
%
\begin{remark}
  $$
  \SAT_{\Ins(X(k), \tilde y)}(z) = 1 - \Delta(\dsum_{X(k)}(z), \tilde y).
  $$
\end{remark}

\begin{corollary}
  Suppose $\Cc_1$, $X(k)$, $z^{\star}$, $y^{\star}$ and $\tilde y$ are as in the
  assumptions of~\cref{lem:robust-approx-ud}. If $z \in \mathbb{F}_2^n$
  is such that
  $$
  \SAT_{\Ins(X(k), \tilde y)}(z) \ge \OPT_{\Ins(X(k), \tilde y)} - \epsilon,
  $$
  then unique decoding either $z$ or $\conj{z}$ gives $z^{\star} \in \Cc_1$.
  Furthermore, if such a $z$ can be found efficiently, so can $z^{\star}$.
\end{corollary}

\begin{proof}
  By the assumption on $z$, we have
  \begin{align*}
    1 - \Delta(\dsum_{X(k)}(z), \tilde y) &=\SAT_{\Ins(X(k), \tilde y)}(z)\\
                                         &\ge \OPT_{\Ins(X(k), \tilde y)} - \epsilon\\
                                         &\ge \SAT_{\Ins(X(k), \tilde y)}(z^{\star}) - \epsilon \\
                                         & = 1 - \Delta(y^\star, \tilde y) -\epsilon,
  \end{align*}
  implying $\Delta(\dsum_{X(k)}(z), \tilde y) \le \Delta(y^\star, \tilde y) + \epsilon$.
  Using the assumption that $\tilde y$ has distance strictly less than $(1/4 - \beta/2 - \epsilon)$
  from $\Cc_k$, we get that $\Delta(\dsum_{X(k)}(z), \tilde y) < 1/4 -\beta/2$, in which case
  we are under all the conditions required in \cref{lem:robust-approx-ud}.
\end{proof}

%\subsection{Concrete Instantiations}
%
%\subsection*{High Dimensional Expanders}
%If the collection $X(k)$ is part of a sufficiently expanding
%$\gamma$-HDX, we can use the following algorithm to approximately solve the $k$-XOR instance.
%
%\begin{theorem}[\cite{AJT19}]
%%
%Let $\Ins$ be an instance of \maxkcsp on $n$ variables taking values over an
%alphabet of size $q$, and let $\epsilon > 0$. Let the simplicial complex $X_{\Ins}$
%be a $\gamma$-HDX with $\gamma = \epsilon^{O(1)} \cdot (1/(kq))^{O(k)}$. 
%%
%Then there is an algorithm based on $(k/\epsilon)^{O(1)} \cdot q^{O(k)}$ levels of the
%    Sum-of-Squares hierarchy which produces an assignment satisfying at least an $(\OPT - \epsilon)$
%fraction of the constraints.
%\end{theorem}
%
%If $X$ is a HDX with the parameters to both satisfy this theorem and be a $(1/2 + 2 \mu_0, 2\beta)$ parity sampler, we can achieve efficient unique decodability of $\Cc_k = \dsum_{X(k)}(\Cc_1)$.
%
%\begin{corollary}\label{cor:cooked-ud-hdx}
%    Let $X(\le d)$ be a $d$-dimensional $\gamma$-HDX satisfying the premises of \cref{lemma:hdx_parity_samplers} that would guarantee that $X(k)$ is a 
%    $(1/2 + 2\mu_0, 2\beta)$-parity sampler, namely, for some $0 < \theta  < \frac{2}{1 + 4\mu_0} - 1$, we have
%    $k \ge \log_{(1 + \theta) \cdot (\frac{1}{2} + 2\mu_0) }(2\beta/3)$, $d \ge \max\set*{ \frac{3k^2}{2\beta},\frac{3}{\theta^2 (1/2 + 2\mu_0)^2\beta}}$, and $\gamma= O(1/d^2)$.
%
%    Then, assuming $\Cc_1$ is efficiently unique decodable within radius $1/4 - \mu_0$, one can uniquely decode $\Cc_k = \dsum_{X(k)}(\Cc_1)$
%    within distance $1/4 - \beta/2 - \epsilon$ in time $n^{(k/\epsilon)^{O(1)} \cdot 2^{O(k)}}, $\footnote{Here we are assuming that uniquely decoding $\Cc_1$ within
%    radius $1/4 - \mu_0$ takes time less than this.} where we have
%    \[ \epsilon = (\gamma \cdot (2k)^{O(k)})^{\frac{1}{O(1)}}. \]
%\end{corollary}
%
%\subsection*{Expander Walks}
%
%In \cref{sec:expander_walks}, we will show that the algorithmic results of
%\cite{AJT19} can be made to work when $X(k)$ is the set of walks of length $k$
%of a suitably strong expander (\cref{cor:cite-ahead-split},
%\cref{cor:alg-cooked-baked2}). In particular, we have the following.
%\begin{theorem}
%    Let $G = (V, E)$ be a graph with $\sigma_2(G) = \lambda$, and $k$
%    a given parameter. Let $\Ins$ be a $k$-CSP instance over an
%    alphabet of size $k$ whose constraint graph is the set of walks
%    in $G$ of length $k$. Let $\epsilon > 0$ be such that $\lambda =
%    O(\epsilon^2/(k^2 \cdot q^{2k}))$.
%
%    Then there exists an algorithm based on $O\parens*{\frac{q^{4k}
%    k^7}{\epsilon^5}}$-levels of the Sum-of-Squares hierarchy which
%    produces an assignment satisfying at least an $(\OPT
%    - \epsilon)$-fraction of the constraints.
%\end{theorem}
%Using this result, one can efficiently unique decode $\Cc_k = \dsum_{X(k)}(\Cc_1)$ when $X(k)$ is
%the set of walks of length $k$ on an expander strong enough to achieve the necessary parity sampling property.
\begin{corollary}\label{cor:cooked-ud-expander}
    Let $\Cc_1$ be a code that is efficiently unique decodable within radius
    $1/4 - \mu_0$ for some $\mu_0 > 0$. 
    Let $G$ be a graph satisfying $\sigma_2(G) =\lambda$, with $1/2 +
    \mu_0 + 2\lambda < 1$. Let $k \ge 2 \log_{1/2 + \mu_0 +
    2\lambda}(2\beta) + 1$, and define $X(k)$ to be the set of all walks in $G$ of
    length at most $k$---note that $\dsum_{X(k)}$ is a $(1/2 + 2\mu_0,
    2\beta)$-parity sampler by \cref{theo:expander_parity_sampler}.

    The code $\Cc_k = \dsum_{X(k)}(\Cc_1)$ can be efficiently decoded within radius
    $1/4 - \beta/2 - \epsilon$ in time $n^{O(2^{4k} \cdot k^7/\epsilon^5)}$, where we have
    \[ \epsilon = O(\lambda \cdot k^2 \cdot 2^k).\]
\end{corollary}
%
%\begin{remark}
%    In both \cref{cor:cooked-ud-hdx}
%    and \cref{cor:cooked-ud-expander}, when $\mu_0$ and $\beta$ are
%    constants, $k$ can be constant, which means
%    we can decode $\Cc_k$ from a radius arbitrarily close to $1/4 - \beta/2$ if
%    we have strong enough guarantees on the quality of the expansion
%    of the high-dimensional expander or the graph, respectively.
%
%    Notice, however, that the unique decodability radius of the code
%    $\Cc_k$ is potentially larger than
%    $1/4 - \beta/2$. Our choice of $(1/2 + 2\mu_0,
%    2\beta)$-parity sampling is needed to ensure that the approximate $k$-CSP
%    solutions lie within the unique decoding radius of $\Cc_1$. Since
%    the bias of the code $\Cc_1$ will generally be smaller than the parity sampling requirement of $1/2 + 2\mu_0$,
%    the bias of the code $\Cc_k$ will be smaller than
%    $2\beta$. In this case, the maximum distance at which our unique decoding algorithm works will be
%    smaller than $\Delta(\Cc_k)/2$.
%\end{remark}

\subsection{List Decoding}



\subsection{Unique Decoding Codes close to GV bound}

==> intro/dsum.tex <==
Before defining direct sum codes, let us define expander graphs formally.

\begin{definition}[Non-bipartite expander]
	Let $G=(V,E)$ be a $d$-regular graph, and let $A_G$ be the normalized adjacency matrix of $G$ so that its top eigenvalue is 1. The graph $G$ is called a $\lambda$-expander if $A_G$ has all the other eigenvalues bounded in absolute value by $\lambda$.
\end{definition}

The main properties of an expander graph that we will use are that they can be constructed explicitly for arbitrarily small values of $\lambda$ \cite{LPS88}, and that they satisfy the following expander mixing lemma:

\begin{lemma}[Expander Mixing Lemma (EML)]
Let $G=(V,E)$ be a $\lambda$-expander. Let $f,g : V\rightarrow \R$ be two functions on $V$. The expander mixing lemma says that the for an expander graph, the average of $f(u)g(v)$ is same whether $u$ and $v$ are chosen based on edges of an expander or $u$ and $v$ are chosen from all pairs in $V\times V$.
	\[
		\abs{\Ex{(u,v) \in E}{f(u)\cdot g(v)} - \Ex{u\in V}{f(u)}\cdot \Ex{v\in V}{g(v)}} \leq \lambda \cdot \Ex{u\in V}{f(u)^2}^{1/2} \cdot \Ex{v\in V}{g(v)^2}^{1/2}
	\]
\end{lemma}

This reduction in number of choices from $n^2$ to $nd$ upto $\lambda$ is what allows expanders to be used in many derandomization applications.

We will be also be heavily using bipartite expanders, which can be obtained as 2-covers of usual expanders, and also satisfy a corresponding expander mixing lemma.

\begin{definition}[Bipartite expander]
	Let $G=(L,R,E)$ be a $d$-regular bipartite graph, and let $A_G$ be the $L \times R$ normalized biadjacency matrix of $G$ so that its top singular value is 1. The graph $G$ is called a $\lambda$-expander if $A_G$ has all the other singular values bounded by $\lambda$.
\end{definition}

\begin{lemma}[Expander Mixing Lemma (EML) on bipartite graphs]
Let $G=(L,R,E)$ be a bipartite $\lambda$-expander. Let $f : L\rightarrow \R$ and $g:R\rightarrow \R$ be two functions on $L$ and $R$ respectively. The EML for bipartite graphs says that
	\[
		\abs{\Ex{(\li,\ri) \in E}{f(\li)\cdot g(\ri)} - \Ex{\li\in L}{f(\li)}\cdot \Ex{\ri\in R}{g(\ri)}} \leq \lambda \cdot \Ex{\li \in L}{f(\li)^2}^{1/2} \cdot \Ex{\ri\in R}{g(\ri)^2}^{1/2}
	\]
\end{lemma}

\vspace{\pspacing}
\subsection{Ta-Shma's breakthrough}
The Plotkin bound says that a code with blocklength $n$, alphabet size $q$ and distance at least $1-\frac{1}{q}$ can have only $\poly(n)$ many codewords, and in particular, the rate of such codes must be 0. For binary codes, this means that no good code have distance $1/2$. For the converse, the Gilbert-Varshamov (GV) bound says that there exist binary codes with distance $\frac{1-\eps}{2}$ and rate $\Omega(\eps^2)$. However, the GV bound shows the existence of such codes via the probabilistic method, and an explicit family of codes with similar parameters has remained elusive for over 70 years.

For many decades, the best rate-distance tradeoff achieved by an explicit binary code was rate $\Omega(\eps^3)$ for distance $\frac{1-\eps}{2}$. These codes are obtained by concatenating a large alphabet code near the Singleton bound with a constant-sized optimal binary code. In 2017, Ta-Shma \cite{TS17} gave a breakthrough construction of explicit linear codes of distance $\frac{1-\eps}{2}$ and rate $\eps^{2+o(1)}$, getting significantly closer to the existential Gilbert-Varshamov (GV) bound rate of $\Omega(\eps^2)$. This is also the state-of-the-art for explicit $\epsilon$-biased sets, a pseudorandomness primitive useful for derandomization. 

Ta-Shma's construction is a distance amplification scheme called \emph{parity sampling}, where the bias of any $\pm 1$ string of length $n$ improves when passed through a direct-sum operation based on an ordered hypergraph. Recall that the bias of a string $f\in \{-1,1\}^n$ is $\frac{\sum_{i=1}^n f_i}{n}$.

\begin{definition}[Direct-sum]
	Let $W \sub [n]^k$ be an ordered hypergraph. The direct sum operation $\dsum_W : \{-1,1\}^n \rightarrow \{-1,1\}^W$ is defined as,
	\[
		\dsum_W(f)(w)= \prod_{i\in w} f_i
	\]
	where $w\in W$.
\end{definition}

The definition of the direct sum operation can be extended from strings to codes by applying it codeword-by-codeword.

\begin{definition}[Parity Sampler]
	An ordered hypergraph $W\sub [n]^k$ is an $(\eps_0,\eps)$ parity sampler if for every string $f\in \{-1,1\}^n$ with bias $\leq \eps_0$, the bias of $\dsum_W(f)$ is $\leq \eps$.
\end{definition}

When $W = [n]^k$, parity sampling ensures that the bias $\eps_0$ of every string improves exponentially to $\eps_0^k$. Ta-Shma showed that picking $W$ to be an intricate but explicit sub-collection of all length-$k$ walks on an expander graph is pseudorandom enough to get a similar exponential boost. That is, this $W$ is an $(\eps_0,\approx \eps_0^k)$ parity sampler. However, the hypergraph used by Ta-Shma has size $|W| = \calO_{\eps_0,k}(n)$ instead of $|W| = n^k$.

\begin{theorem}[\cite{TS17}, informal]
	There is an explicit $(\eps_0, \approx \eps_0^k)$ parity sampler $W\sub [n]^k$, based on (subcollection of) length-$k$ walks on a Ramanujan expander graph, such that $|W| \approx n / (\eps_0^{k})^{2+o(1)}$.
\end{theorem}
A linear code is $\eps$-balanced if every non-zero codeword in it is $\eps$-biased, and every $\eps$-balanced code has distance at least $\frac{1-\eps}{2}$. Parity samplers can be used for distance amplification of binary codes. To do this, one starts with an explicit $\eps_0$-balanced code of suboptimal rate-distance tradeoff. Applying the direct-sum operation codeword by codeword yields a new code of blocklength $|W|$ and bias $\approx \eps_0^k$. The rate of the new code is worse by a factor of $n/|W|$, which for Ta-Shma's construction is $(\eps_0^k)^{2+o(1)}$. Taking $\eps \approx \eps_0^k$, this yields codes with distance $\frac{1-\eps}{2}$ and rate $\eps^{2+o(1)}$.
%For a string $f:[n] \rightarrow \{0,1\}$, the direct-sum according to a $k$-regular ordered hypergraph $W \sub [n]^k$ is given by $\dsum_W(f) : W \rightarrow \{0,1\}$ such that for any $e = (i_1,i_2,\cdots ,i_k)$
%\[
%	\dsum_W(f) (e) = f(i_1) \oplus f(i_2) \oplus \cdots \oplus f(i_k)
%\]
%By using $W$ to be a carefully chosen subcollection of all length $k-1$ walks on an expander graph so that $|W| = \calO(n/\eps^{2+o(1)})$, Ta-Shma's proof shows that it is possible to ensure that $\bias(f) \leq \eps_0 \implies \bias(\dsum_W(f))\leq \eps$.

\subsection{Constraint Satisfaction Problems on Expanders}

Constraint satisfaction problems (CSPs) are combinatorial optimization problems involving $n$ variables that take values from an alphabet $\Sigma$ with a prescribed set of constraints on these variables. The goal is to assign values to these variables from $\Sigma$ such that the number of constraints satisfied is maximized.  The fraction of constraints satisfied by the best possible assignment is called the \emph{value} of the CSP.

A CSP is called a $k$-CSP if every constraint involves $k$ variables. Often these constraints on $k$ variables appear as a shared common predicate like XOR, and in such a case, the CSP is called $k$-XOR. The constraints of a $2$-CSP form a graph on $n$ vertices, with an edge between two vertices if they appear together in a constraint. Likewise, a $k$-CSP induces a $k$-uniform hypergraph, and we say that the CSP is supported on the corresponding graph or hypergraph. It has long been known that 2-CSPs supported on a dense graph admit efficient approximation algorithms based on random sampling, regularity lemmas and convex hierarchies \cite{AKK95, FriezeK99, YZ14:dense}. These results were extended to include $2$-CSP instances supported on expanders using spectral/semidefinite programming based algorithms \cite{CMM06, AKKSTV08, Kolla11, BRS11}. Finally, Alev, Jeronimo and Tulsiani \cite{AJT19} extended these results to $k$-CSPs supported on High-Dimensional Expanders by using a notion of multilevel expansion they called \emph{splittability}. Their algorithm is based on the Sum-of-Squares (SoS) hierarchy of semidefinite programs.

\subsection{Decoding Direct Sum Codes}

In \cite{AJQST20}, we showed that algorithmic tractability of CSPs supported on splittable hypergraphs, together with their parity sampling properties, facilitates decoding for direct sum codes based on such hypergraphs. Moreover, we showed that the expander walks hypergraph also satisfies splittability in addition to high-dimensional expanders, and in the other direction, a high-dimensional expander is also a parity sampler. This allowed us to develop list decoding algorithms for direct sum codes based on high dimensional expanders and on expander walks. 

Moreover, through a known reduction from direct sum to direct product, we could also recover the results of \cite{DHKLNTS19} who showed a direct product based distance amplification scheme called ABNNR amplification can be list decoded if the direct product is supported on a high-dimensional expander. \cite{DHKLNTS19} used the expanding structure to set up a specific 2-CSP called Unique Games on expanders, which they then solved using a blackbox call to the CSP algorithms mentioned above. The work of \cite{DHKLNTS19} was tailored to high dimensional expanders, relying on a notion called double samplers, and did not deal with expander walks.

We next show how the CSP algorithms help with unique decoding using relatively simple ideas. Since direct sum is a distance amplification scheme, where one starts with a base code and construct a new code based on it, our algorithms are actually reductions to decoding problems in the base code. As we will see, these reductions can sometimes be quite favorable by reducing list decoding of the amplified code to only unique decoding of the base code.
\begin{theorem}[unique decoding direct sum]
	Let $\calC_0$ be an $\eps_0$-balanced binary code of blocklength $n$ that is decodable upto radius $\frac{1-\eps_0^{dec}}{2}$ in time $\calT_1(n)$, for some $\eps_0^{dec} \in [\eps_0,1)$. Suppose $W\sub [n]^k$ is an $(\eps_0^{dec},\eps)$ parity sampler, so that $\calC = \dsum_W(\calC_0)$ is $\eps$-balanced. 

	Suppose for some $\kappa \geq 0$, there is an algorithm that runs in time $\calT_2(n,k, \kappa)$ and given a $k$-XOR instance on $W$ with value $OPT$, outputs an assignment that satisfies $OPT-\kappa$ fraction of constraints.
	
	Then the code $\calC$ can be decoded upto radius $\frac{1-\eps - 2\kappa}{4}$ in time $\calT_1(n)+\calT_2(n,k,\kappa)$.
\end{theorem}
%
\begin{proof}
	Given $g\in \{-1,1\}^W$, the decoding task is to find a codeword $\dsum_W(h) \in \calC$ such that $\Delta(g,\dsum_W(h))\leq \frac{1-\eps-2\kappa}{4}$,  and we are promised such a codeword exists. Because of triangle inequality, the closest codeword to $g$ must be $\dsum_W(h)$. That is,
	\[
		h = \argmin_{f\in \calC_0} \Delta(g,\dsum_W(f)) = \argmax_{f\in \calC_0} \ip{g}{\dsum_W(f)}
	\]
	The optimization in the rightmost term is possibly intractable, but relaxing the constraint $f\in \calC_0$ allows us to view this optimization as a $k$-XOR instance on $W$. Moreover, we know that the optimal for this optimization is at least $\frac{1+\eps+2\kappa}{2}$. Then, this $k$-XOR solver returns $\dsum_W(h')$ such that $\ip{g}{\dsum_W(h')} \geq \frac{1+\eps+2\kappa}{2} - \kappa = \frac{1+\eps}{2}$. Note that $h'$ need not be in $\calC_0$. Rewriting in Hamming distance,
	\[
		\Delta(g,\dsum_W(h')) \leq \frac{1-\eps}{4}
	\]
	and by triangle inequality
	\begin{align*}
		\Delta(\dsum_W(h),\dsum_W(h')) \leq \Delta(\dsum_W(h),g) + \Delta(g,\dsum_W(h')) &\leq \frac{1-\eps-2\kappa}{4}+\frac{1-\eps}{4} \\
		&= \frac{1-\eps-\kappa}{2}
	\end{align*}
	By the contrapositive of $(\eps_0^{dec},\eps)$ parity sampling applied to strings $h$ and $h'$, we get that $\Delta(h,h') \leq \frac{1-\eps_0^{dec}}{2}$ or $\Delta(h,h') \geq \frac{1+\eps_0^{dec}}{2}$. Therefore, $h$ can be found using decoding calls in the base code $\calC_0$ from $h'$ and the string obtained by flipping every coordinate of $h'$.
\end{proof}

Note that the above reduction requires an $(\eps_0^{dec},\eps)$ parity sampler, which can be stronger than the distance amplification requirement of $(\eps_0,\eps)$ parity sampler.

The algorithm to list decode is significantly more involved, and involves modifying the CSP algorithm for $k$-XOR. We will only mention the key ingredients needed for list decoding, since full details are outside the scope of this proposal. As mentioned before, the $k$-XOR algorithm of \cite{AJT19} is based the Sum-of-Squares (SoS) hierarchy, which optimizes over \emph{pseudodistributions} of assignments. A pseudodistribution is a relaxation of the set of distributions which only needs to \emph{appear like a distribution} to certain low-degree tests. In exchange for this weaker property, pseudodistributions can be efficiently optimized over, via semidefinite programming. 

In the case of solving $k$-XOR, we ask for a pseudodistribution that maximizes the number of constraints satisfied, and then round it to an integral assignment. For list decoding, we first set a threshold for the number of constraints that need to be satisfied, and then among the pseudodistributions that satisfy this threshold, we pick the one that maximizes some entropic proxy. This ensures that the pseudodistribution is \emph{close to} every codeword in the list, and a random conditioning based rounding then allows the algorithm to recover every list codeword with some small but positive probability.
%
This leads to the following informal theorem for direct sum codes based on expander walks.

\begin{theorem}[\cite{AJQST20}]\label{thm:ajqst}
Let $\eps_0 <1/2$ be a constant and $\eps \in (0,\eps_0)$, and let $G$ be a $d$-regular $\gamma$-two-sided spectral expander graph on $n$ vertices with $\gamma \leq \eps^{\calO(1)}$.

For every $\eps_0$-balanced linear code $\calC_0 \sub \F_2^n$ that is unique decodable in time $\calT(n)$, there exists a direct sum encoding $\calC \sub \F_2^{W_G(k)}$ with $k = \calO(\log(1/\eps))$ that is $\eps$-balanced and satisfies the following:
\begin{itemize}
	\item If $g$ is $\frac{1-\sqrt{\eps}}{2}$-close to $\calC$, then we can compute the list of all codewords of $\calC$ that are $\frac{1-\sqrt{\eps}}{2}$-close to $g$ in time $n^{\eps^{-\calO(1)}}\cdot \calT(n)$.
	\item The rate of $\calC$ is $R = R_0/d^{k-1}$, where $R_0$ is the rate of $\calC_0$.
\end{itemize}
\end{theorem}
%In \cite{AJQST20}, we showed that choosing $W$ to be structured as opposed to random not only helps with the explicitness of the code, but also with algorithmic tractability of the decoding problem. In particular, the (multilevel) expansion properties that help with parity sampling also allow the algorithms developed by Alev, Jeronimo and Tulsiani \cite{AJT19} to solve $k$-XOR instances supported on it. Building on the ideas of Dinur et al \cite{DHKLNTS19}, who showed connections between list decoding direct product and constraint satisfaction problems (CSPs), we gave a polynomial time algorithm to list decode direct sum codes based on expander walks or High-Dimensional Expanders (HDXs).

\subsection{Decoding Direct Sum Codes near the GV bound}

In \cref{thm:ajqst}, the graph $G$ needs to be a very strong expander, with its second largest eigenvalue bounded by $\eps^{\calO(1)}$, because of the requirements imposed by the underlying SoS-based algorithms of \cite{AJT19}. In contrast, Ta-Shma was able to build an $(\eps_0,\eps)$ parity sampler using $\calO(\log(1/\eps))$ length walks on a $\gamma$-expander with $\gamma \approx \eps_0^2$. The extra strong expansion requirement in \cref{thm:ajqst} also means that the corresponding rate loss is much worse, and the best bound we can guarantee is that rate $R = R_0 \cdot \eps^{\calO(\log(1/\eps))}$. Therefore, while the codes in \cref{thm:ajqst} allow efficient list decoding upto radii arbitrarily close to 1/2, their rate is quasipolynomial in $\eps$, and nowhere close to the GV bound $\Omega(\eps^2)$.

It may be expected that since the expander used in \cref{thm:ajqst} is much stronger than needed for Ta-Shma's construction( $\gamma \leq \eps^{\calO(1)}$ instead of $\gamma \approx \eps_0^2$), that the true bias of the final code is also much better than just $\Omega(\eps)$. However, the way these parameters are coupled in the analysis of parity sampling does not allow us to take advantage of this stronger expansion. The source of the strong expansion requirement of $\gamma \leq \eps^{\calO(1)}$ can be broadly thought to be the strong quality of approximation we expect from the CSP solvers of \cite{AJT19}. Dense CSPs support arbitrarily good approximation, but for a sparse CSP to inherit them, their expansion quality should be correspondingly good. In fact, the algorithm of \cite{AJT19} suffers an approximation error of $\gamma^{\Omega(1)} \cdot 2^k$.

To list decode upto radius $\frac{1-\eps}{2}$, the approximation error must be $\calO(\eps)$. But if we aim for only the unique decoding task, while still using the list decoding framework of \cite{AJQST20}, it is possible to tolerate larger amounts of error, so that $\gamma^{\Omega(1)}\cdot 2^k$ can be taken to be a constant such as $0.1$. However, $\gamma$ still needs to be small enough to offset the $2^k$ term. 

In \cite{JQST20}, we exploit the fact that walks hypergraph can be seen as a cascaded structure to only deal with small $k$ at a time (independent of $\eps$), instead of $k \approx \log(1/\eps)$. We start with the observation that the set of all length-$k^2$ walks in a graph $G$ can be seen as the set of all length-$k$ walks over the graph $G'$, where $G'$ has length-$k$ walks of $G$ as vertices, and two vertices in $G'$ are connected with an edge iff the endpoints of the corresponding walks in $G$ are adjacent. This observation can be extended to obtain a cascade of codes $\calC_0, \calC_1, \cdots ,\calC_{\ell}$, where $\calC_{\ell} = \calC$ and $\ell = \log \log (1/\eps)$, such that every $\calC_i$ is obtained from $\calC_{i-1}$ via a direct sum operation. The key advantage is that the hypergraph used for this direct sum is $k$-uniform for a constant $k$. This allows us to take $\gamma = \Omega(1)$ instead of $\gamma = \eps^{\calO(1)}$.

With some more technical modifications, this allows us to develop algorithms to unique decode the direct sum construction of Ta-Shma with near-optimal parameters. The algorithm works by recursively reducing the list decodability of $\calC_i$ to that of $\calC_{i-1}$. This leads to the following theorem.

\begin{theorem}[\cite{JQST20}]
	For every $\eps>0$, there are explicit binary linear Ta-Shma codes $\calC_{n,\eps} \sub \F_2^n$ for infinitely many values $n\in \N$ such that
	\begin{enumerate}[(i)]
		\item $\calC_{n,\eps}$ is $\eps$-balanced,
		\item rate of $\calC_{n,\eps}$ is $\eps^{2+o(1)}$, and
		\item $\calC_{n,\eps}$ can be unique decoded in time $n^{\calO_{\eps}(1)}$.
	\end{enumerate}
\end{theorem}

In fact, our algorithm can list decode upto a radius $1/2 - 2^{-\Theta((\log_2(1/\eps))^{1/6})}$ that approaches 1/2 as $\eps \rightarrow 0$. Therefore, for small $\eps$, this algorithm can decode significantly beyond the unique decoding radius. However, note that the Johnson bound implies that Ta-Shma's code is combinatorially list decodable up to radius $\frac{1-\sqrt{\eps}}{2}$, which approaches $1/2$ with a much better dependence on $\eps$ as $\eps \rightarrow 0$. 

The works \cite{AJQST20, JQST20} were extended by \cite{RR23} who avoided the CSP viewpoint of decoding by directly working with the Sum-of-Squares relaxations underlying the CSP solver of \cite{AJT19}. This allowed them to efficiently decode Ta-Shma's code upto the Johnson bound, which is the best radius up to which we know that the list sizes are polynomial. \cite{RR23} showed that the parity sampling result of Ta-Shma can be extended to pseudodistributions obtained after some random conditioning. This allowed them to impose essentially the same constraint on expansion $\gamma$ for decoding as is needed for the distance amplification to work.

==> intro/proposed.tex <==
In this section, we propose some directions for future work related to the results described until now. We broadly focus on two goals: improvements in the capacity achieving codes of \cref{sec:beyond_johnson}, and faster algorithms to replace SoS.

\subsection{Codes beyond Johnson bound}

As described in \cref{sec:beyond_johnson}, we can construct new list decoding capacity achieving codes using just expander graphs. However, there are several interesting directions in which this result may be improved:
\begin{enumerate}
	\item The results we obtain are only combinatorial until now. It would be interesting to list decode up to capacity with efficient algorithms. In fact, one motivation for looking for such combinatorial constructions of capacity-achieving codes is to have truly linear time decoding algorithms that work up to the capacity.
	\item Secondly, the list size and alphabet size are both towers of height $\poly(1/\eps)$. The counting technique we use can also be used for bounding the size of an affine subspace, giving an upper bound that is a tower of height equal to dimension of the affine subspace. But for an affine subspace counting the number of affine combinations gives a much sharper bound that is singly exponential in the dimension. Following the intuition from affine subspace should allow us to get a list size of $(1/\eps)^{1/\eps}$.
	\item It would also be interesting to investigate extensions such as list-recovery, which are useful for constructing binary codes decodable up to the Zyablov bound (that is, best concatenation based rate-distance tradeoff).
\end{enumerate}

Another interesting direction, which was one of our original motivations, is to investigate \emph{general} ways of improving the list decoding radius of a code by interleaving. For interleaved RS codes, Parvaresh and Vardy \cite{PV05} showed that interleaving only related codewords $f(X)$ and $f(X)^d \mod E(X)$, for some irreducible polynomial $E(X)$, allows for constant list sizes beyond the Johnson bound. We may think of this as a pseudorandom relation between the two codewords being interleaved. Is there a similar combinatorial (pseudorandom) condition that can be extracted out of their proof that works for general codes?

Finally, interleaving or folding are operations closely related to direct product, and inherently lead to codes over large alphabets. Is it possible to replace the direct product by direct sum in some cases, and what implications could such a result have constructing binary codes achieving list decoding capacity?
%
\subsection{Faster algorithms}

We have seen that the SoS hierarchy based algorithms combined with the random conditioning based correlation rounding are a powerful tool for the task of list decoding. However, these algorithms run in time $n^{\poly(1/\eps)}$, which is hopelessly impractical. This is partially alleviated in the case of direct sum codes where we can do gentle list decoding in near-linear time. However, for list decoding of other classes of codes like Tanner codes and AEL amplified codes, as well as to get to the Johnson bound of Ta-Shma codes, we are stuck with the poor running times of SoS. We would like to pursue the following threads for faster algorithms:

%The running times for the SoS-based list decoders up to Johnson bound, though polynomial, are quite poor.
\begin{enumerate}
	\item There are multiple directions for possible improvements: SoS-degree reduction \cite{DV14, ST21}, faster continuous optimization \cite{GS12:faster}, spectral methods \cite{GI02, HSSS16} and regularity lemmas \cite{OGT15, JST21}. In particular, for Ta-Shma's code, can the regularity lemma based algorithm of \cite{JST21} be made to work up to the Johnson bound to match \cite{RR23}?
	\item The key step in the decoding algorithms that leads to poor running times is the correlation rounding for SoS. A concrete goal is whether the correlation rounding can be implemented via enumeration over some basis, potentially discovered via a regularity lemma, that avoids the need for higher moments. This enumeration could allow us to produce the non-convexity inherent in the set of low-correlation SoS solutions, just as the trivial exponential-time enumeration can produce fully non-convex integral solutions. This question is interesting even for the linear programming based Sherali-Adams hierarchy, as used in \cite{YZ14:dense, HST20, CLN22}.
	\item Finally, coming back to decoding, for most of the codes above, we know of efficient combinatorial unique decoders. Moreover, these unique decoders may even have a convex optimization style interpretation. For example, \Zemor's alternating decoder \cite{Zemor01} for Tanner codes may be seen as alternating projections applied to the sets satisfying left code constraints and right code constraints respectively. Further, even though the algorithm works only over expanders, the algorithm does not require an efficiently discoverable certificate of expansion. Is there a way to combine our entropy maximization intuition with these combinatorial decoders that does away with the need for SDPs? A recent work \cite{BBKS24} implements something similar in the learning setting, their combinatorial greedy algorithm only needs the Restricted Isometry Property to be true for some matrix for correctness, but does not need a certificate to use in the algorithm.
\end{enumerate}
%
%\subsection{Other less concrete problems}

%\input{less_concrete}

==> quantum/abstract.tex <==

\edits{Abstract needs to more work}

We show that Quantum Low-Density Parity Check (QLDPC) codes with efficient \emph{unique} decoding algorithms, when amplified using the expander-based distance amplification of Alon, Edmonds, and Luby [FOCS 1995], yield new QLDPC codes, which can be efficiently \emph{list decoded} up to the Johnson bound. Previous constructions of list decodable good distance quantum codes either required access to a classical side channel for list decoding LDPC codes,
or required stronger list decoding properties for the starting code, precluding the LDPC property for which constructions of list decodable codes were not previously available. 

Our results are based on convex relaxations obtained using the Sum-of-Squares hierarchy, which reduce the problem of list decoding the distance amplified codes to unique decoding the starting base codes. Combined with recent breakthrough constructions of good QLDPC codes with efficient unique decoding, this yields a construction of QLDPC codes with optimal rate-distance tradeoffs and efficient list decoding up to the Johnson bound. 

==> quantum/ael.tex <==
\section{Concatenated Codes and AEL Amplification}
%
\label{sec:ael}

In this section, we will formalize the quantum CSS generalizations of two operations on classical codes -- \textit{code concatenation} and AEL \textit{distance amplification} \cite{AEL95}. We define it purely in linear algebraic terms but the recent work~\cite{BGG22} also formalizes this using the stabilizer code framework. 

\subsection{Concatenation of CSS Codes}

To define a concatenation of CSS codes, one needs a pair of outer code and inner code that are compatible with respect to some parameters. Additionally in the quantum case, we need a pair of duality-preserving maps as defined in~\cref{lem:compl}.  


%Let $\cD = (\dx, \dz)$ be a $[[n, k_\out, \delta_{\out}n]]_{q^k}$ CSS code over the field $\F_{q^k}$. Let $\cC = (\cx, \cz)$ be a $[[d, k, \delta_{\inn}d]]_{q}$ CSS code over the field $\F_{q}$ and let $(\subs{\phi}{X} ,\subs{\phi}{X})$ be the maps obtained from~\cref{lem:compl}. % is the subspace obtained by applying the map $\phix$ to each coordinate of $\dx$. (resp., $\dz$).

 
%\paragraph{Complementary Bases} Let $\phix$  be a linear isomorphism of $\F_q$-vector spaces  $\phix: \F_{q^{k}} \to W_X$. Analogously, let $\phiz$ be an isomorphism to $W_Z$. We call them \textit{complementary} if, 
%    \begin{equation}
%    \mathsf{Tr}\, (xy) = \ip{\phix(x)}{\phiz(y)}_{\F_q^d}  \; \; \forall\, x,y \in \F_{q^k}
%    \end{equation}
\begin{definition}[Concatenated CSS Codes]
Given the following objects,	
\begin{itemize}
    \item \textbf{Outer Code} --- Let $\cD = (\dx, \dz)$ be a $[[n, k_{\out}, \delta_{\out}]]_{q^k}$ CSS code over the field $\F_{q^k}$.
    \item \textbf{Inner Code} --- Let $\cC = (\cx, \cz)$ be a $[[d, k, \delta_{\inn}]]_{q}$ CSS code over the field $\F_{q}$, such that $\cx = W_X \oplus \cz^{\perp}$ and $\cz = W_Z \oplus \cx^{\perp}$ respectively. 
    \item \textbf{Duality preserving maps} --- Let $(\phix,\phiz)$ be duality preserving maps as in~\cref{lem:compl} from $\F_{q^{k}}$ to $\subs{W}{X}$ and $\subs{W}{Z}$ respectively. Extend these maps to $\F_{q^k}^n$ by applying it to each coordinate.
\end{itemize}
\vspace{-5pt}
one defines the concatenated CSS Code, $\cE = \cD \circ_\varphi \cC$ as $(\ex, \ez)$ with
    \begin{align*}
        \ex &=\phix( \dx) + \mathbb{F}_{q_1}^n \otimes \cz^{\perp} \subseteq \F_q^{nd}\\
        \ez &= \phiz(\dz) + \mathbb{F}_{q_1}^n \otimes \cx^{\perp}\subseteq \F_q^{nd}
    \end{align*}
\end{definition}

We now give an explicit description of the dual spaces that will prove that the concatenation operation defines a CSS code and also be useful in proving the distance of the final code. 

% and denote the image of a subspace under these maps as $\phix(\dx)$ (respectively, $\phiz(\dz)$ )
%
%\begin{definition}[Concatenated CSS Codes]
%    Given a pair of CSS Codes $(\cx,\cz)$ and $(\dx,\dz)$ with respective parameters $[[d,k,\delta_\inn d]]_{q}$ and $[[n, k_{\out}, \delta_\out n]]_{q^k}$, we define the concatenated CSS Code, $\cE = \cD \circ_\varphi \cC$ as $(\ex, \ez)$ with
%    \begin{align*}
%        \ex &=\phix( \dx) + \mathbb{F}_{q_1}^n \otimes \cz^{\perp} \\
%        \ez &= \phiz(\dz) + \mathbb{F}_{q_1}^n \otimes \cx^{\perp}
%    \end{align*}
%     
%\end{definition} 
%\tnote{How to mention the condition for $\phi_X$??}
\begin{proposition}\label{prop:concat_dual}
    For the above definition of $(\ex, \ez)$, the dual spaces can be computed as follows,
    \begin{align*}
        \ex^{\perp} &= \phiz(\dx^{\perp}) + \mathbb{F}_{q}^n \otimes \cx^{\perp} \\
        \ez^{\perp} &= \phix(\dz^{\perp}) + \mathbb{F}_{q}^n \otimes \cz^{\perp}
    \end{align*}
    Therefore, $(\ex,\ez)$ is an $[[nd, k_{\out}\cdot k]]_q$ CSS code.
\end{proposition}
\begin{proof} We prove the first equation as the proofs are symmetric. Denote by $\mathcal{U}_X := \phiz(\dx^{\perp}) + \mathbb{F}_{q}^n \otimes \cx^{\perp}$. Notice that for a $\F_{q^k}$-subspace $U\subseteq \F_{q^k}^n$, we have $\dim(\phix(U))_{\F_q} = \dim(U)\cdot k$.  Thus, \[\dim(\mathcal{U}_X) = \dim(\dx^\perp)\,k + n\, \dim(\cx^\perp) = (n-k_{\out})\,k + n (d-k) = nd - k_{\out}k = \dim(\ex^\perp).\] 
Therefore, it suffices to show that $\mathcal{U}_X\subseteq \ex^\perp$. 
Let $u \in \mathcal{U}_X$ and $v \in \ex$ be any pair of vectors which, using the definition of the spaces, we express as,
\begin{align*}
 u ~&=~ (\phiz(u_1) + x_1,\,\cdots\,, \phiz(u_n) + x_n ) \in \mathcal{U}_X \quad \text{ where } x_i \in \cx^\perp\\   
 v ~&=~ (\phix(v_1) + z_1,\,\cdots\,, \phix(v_n) + z_n ) \in \ex \quad \;\; \,\text{ where } z_i \in \cz^\perp.
\end{align*}

Computing the inner product we get four kinds of terms,
\[
\ip{u}{v} = \sum_{i=1}^n \parens[\Big]{\ip{\phiz(u_i)}{\phix(v_i)} + \ip{\phiz(u_i)}{z_i} + \ip{x_i}{\phiz(v_i)} + \ip{x_i}{z_i} }  \]
Each of the last three terms is zero, as by definition, they belong to orthogonal spaces.
We are then left with the first term which can be calculated using the duality-preserving property of the maps.
\begin{align*}
   \ip{u}{v} ~&=~ \sum_{i=1}^n \ip{\phiz(u_i)}{\phix(v_i)} 
   ~=~ \sum_{i=1}^n \mathsf{Tr}\, (u_iv_i)
   ~=~ \mathsf{Tr}\, \left( \ip{u}{v} \right)  = 0 . 
\end{align*}
This proves that $\mathcal{U}_X = \ex^\perp$. Moreover, if $\dx = V_X \oplus \dz^\perp$, the proof implies that $\ex = \phi_X(V_X) \oplus \ez^\perp$.
%
   Thus, the dimension of the code is $\dim(\phi_X(V_X))_{\,\F_q} = \dim(V_X) \cdot k = k_{\out}\cdot k$. 
\end{proof}

\subsection{AEL Amplification and Folding CSS Codes}

Let $\cD$ be a CSS code in $\F_{q^k}^n$ and let $\cC$ be a a CSS code in $\F_q^d$, of dimension $k$. The AEL procedure amplifies the distance of the concatenated code $\cE = \cD \circ_{\varphi} \cC$ using a $d$-regular bipartite expander, $G = (L,R, E)$ where $\abs{L} = \abs{R} = n$. Note that the sizes of $L$ and $R$ match the blocklength of the outer code and the degree matches the blocklength of the inner code. 

Since, the concatenated code, $\cE$ is over $\F_q^{nd} \cong \F_q^E$, we can view the codewords, $z \in \ex$ (or $\ez$), as an assignment of $\F_q$-values to the edges. Denote by $z_\li \in \F_q^d$, the restriction of the vector $z$ to the neighborhood, $N(\li)$, of vertex $\li$. We will use similarly use $z_\ri$, to denote restrictions to the neighborhood of vertices in $R$.  We can now restate the definitions of the concatenated codes (and their duals) in a local manner, which will be required for a low-degree sum-of-squares proof.

\begin{definition}[Concatenated code]\label{def:concat}
	The concatenated code $\cE = \cD\circ_\varphi \cC$ and its duals can be explictly described as,
\begin{align*}
 	\ex ~&=~ \Set*{ x \mid x_{\li} =  \phix(u_\li) + z_\li, \text{ for a unique  } z_\li \in \cz^\perp \text{ and } u \in \parens{\dx}^L }\\[2.5pt]
 		\ex^\perp ~&=~ \Set*{ x \mid x_{\li} =  \phix(u_\li) + z_\li, \text{ for a unique  } z_\li \in \cx^\perp \text{ and } u \in \parens{\dx^\perp}^L }\\[2.5pt]
 		\ez ~&=~ \Set*{ x \mid x_{\li} =  \phix(u_\li) + z_\li, \text{ for a unique  } z_\li \in \cx^\perp \text{ and } v \in \parens{\dz}^L }\\[2.5pt]
 		\ez^\perp ~&=~ \Set*{ x \mid x_{\li} =  \phix(u_\li) + z_\li, \text{ for a unique  } z_\li \in \cz^\perp \text{ and } u \in \parens{\dx}^L }
 \end{align*}
 Uniqueness follows as $\mathrm{Im}(\phix) = \subs{W}{X}$ is disjoint from $\cz^\perp$ (and similirly for $\phiz$).
Thus, one can define local inversion maps $\unconx : x_\li = \phix(u_\li) + z_\li \mapsto u_\li \in \dx $, and   $\unconz : x_\li = \phiz(v_\li) + z_\li \mapsto v_\li \in \dz$.
 \end{definition}

The concatenated code $\cE$ is folded using the partitions induced by the neighborhoods of the right vertices. Explicitly, the folded code $\fold(\cE) =  (\fold(\ex), \fold(\ez))$ is given by,
 \begin{align*}
 	\fold(\ex) ~&=~ \Set*{\parens{\fold(z_{\ri_1}), \cdots , \fold(z_{\ri_n}) } \mid z \in \ex,\; \ri_i \in R} \subseteq \parens*{\F_{q}^d}^n  \\
 	\fold(\ez) ~&=~ \Set[\Big]{[\fold(z_{\ri_1}), \cdots , \fold(z_{\ri_n}) ] \mid z \in \ez,\; \ri_i \in R} \subseteq \parens*{\F_{q}^d}^n 
 	\end{align*} 
  	 
 The AEL procedure effectively is the three-step process --- (i) \textit{unfold} the $\F_{q^d}$-symbols of the outer code $\cD$ using the map $\varphi$ to an inner code $\cC$, (ii) shuffle the symbols via edges on a bipartite expander graph $G$, and (iii) collect $d$-symbols on the right vertices and fold them back to produce the final code, $\fold(\cE)$, which is a vector space CSS code with alphabet $\F_q^d$. 
 
 The key change is that the metric changes from the initial $\Delta_L(\cdot,
 \cdot)$ on the outer code $\cD$ to  $\Delta_R(\cdot,
 \cdot)$ on the folded code, $\fold(\cE)$. This change is crucial as this is where graph expansion comes in, and implies that the distance between codewords under the $\Delta_R$ metric is much larger than the initial distance under the $\Delta_L$ metric. We define these below as we will use this notation throughout the rest of the paper.  
%
 \begin{align*}
 	\Delta_L(z,h) ~&=~ \Ex{\ell\sim L}{\indi{ z_\li \neq h_{\li}}},  \\
 	\Delta_{L, \cz^\perp}(z,h) ~&=~ \Ex{\ell\sim L}{\indi{ z_\li \not\in h_{\li} + \cz^\perp }}, \\
 	\Delta_{R}(z,h) ~&=~\Ex{r\sim R}{\indi{ z_{r} \neq h_{r}}}.
 \end{align*}
  subset of $f(S)\subseteq \F_{q^d}^{n}$. 
 
\begin{proposition}\label{cor:ael_rate}
Let $\cD$ be a CSS code in $\F_{q^k}^n$ of dimension $k_{\out}$, and let $\cC$ be a CSS code in $\F_q^d$ of dimension $k$.
Then, the folded AEL code, $\fold(\cE) = \fold(\cD\circ_\phi \cC)$ defines a $[[n,k_\out \cdot k, \delta_R]]_{q^d}$ QECC where $\delta_R = \min_v \disR{v}{0}$ where the minimum is over non-trivial codewords, \ie  $v \in \braces[\big]{(\ex\setminus \ez^\perp) \cup (\ez\setminus \ex^\perp)}$.
\end{proposition}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> quantum/covering.tex <==
\section{Covering Lemma}\label{sec:covering}
%
\todo{Add a little text to say what the covering lemma does.}

For any $f\in \F_q^E$, recall that $f_r \in  \F_q^d$ is the restriction of $f$ to the edge-neighborhood of a vertex $r \in R$. 
% We embed any $f\in \F_q^E$ into $\R^{q^d\cdot n}$ as $\embed(f)$ which is defined as the concatenation of $e_{f_r} \in \R^{q^d}$ vectors for all $r\in R$. Here, $e_{f_r}$ denotes the characteristic (indicator) vector of $f_r$ as an element of $\F_q^d$, scaled up by a factor of $\sqrt{q^d}$ to make it a unit vector. Inner products for this embedding capture the $\disR{\cdot}{\cdot}$ distances as
%	\[
%		\disR{f_1}{f_2} = 1 - \ip{\embed(f_1)}{\embed(f_2)}
%	\]
%	\tnote{Can we define this embedding a bit more precisely? Something like below?? Also, we might need to mention folding here and I might need to correct folding notation.}
	
	\begin{definition}[Embedding]
	Let $\R^{q^d}$ be spanned by formal orthonormal basis vectors $\Set{e_w\,\mid \,w\in \F_{q}^d}$. Define an embedding $\embed : \F_q^E \to \parens{\R^{q^d}}^R \cong \R^{q^d\cdot n}$, as $\embed (f)_r = e_{f_r}$ for each $r\in R$. We denote the image of a subspace, $U$ under this map $\embed(U)$. The Euclidean inner product for this embedding captures the $\disR{\cdot}{\cdot}$ distance as,
	\[
		\disR{f_1}{f_2} = 1 - \ip{\embed(f_1)}{\embed(f_2)}.
	\]
	\end{definition}
\begin{lemma}[Covering Lemma]\label{lem:covering}
	Let $g\in \F_q^E$ and $\alpha \in (0,1)$.
	There exists a distribution $\calD$ over $\fx$ with support size at most $q^d \cdot n + 1$ such that for any $h \in \fx$ such that $\distR{g} < 1-\alpha$,
	\[
		\Ex{f\sim \calD}{\distR{f}} < 1-\alpha^2 \mper
	\]
\end{lemma}
%\begin{proof}
%	Let $\calH = \inbraces{h\in F_X \suchthat \distR{g} <1-\alpha} = \inbraces{h\in F_X \suchthat \ip{\embed(g)}{\embed(h)} > \alpha}$.
%	\todo{Shashank: Will probably change $\embed$ to something else as it looks very similar to $X$.}
%	
%	Consider the set $T = \inbraces{v\in \conv{\embed(F_X)} \suchthat \ip{v}{\embed(g)} >\alpha}$. We may assume this set to be non-empty, since otherwise the lemma is trivially true. Let $g_0 = \argmin_{v\in T} \norm{v}^2$.
%
%\begin{claim}\label{claim:covering}
%	For any $h\in \calH$, it holds that $\ip{g_0}{\embed(h)}>\alpha^2$.
%\end{claim}
%
%To finish the proof using this claim, we write $g_0$ as a convex combination of elements in $\embed(F_X)$ and let the corresponding distribution over $F_X$ be $\calD$. By the \Caratheodory theorem, $\calD$ can be chosen with support size at most $q^d \cdot n + 1$. Finally,
%\begin{align*}
%	\Ex{f\sim \calD}{\distR{f}} &= \Ex{f\sim \calD}{1 - \ip{\embed(f)}{\embed(h)}} \\
%	&= 1- \ip{\Ex{f\sim \calD}{\embed(f)}}{\embed(h)} \\
%	&= 1- \ip{g_0}{\embed(h)} \\
%	&< 1-\alpha^2 \qedhere
%\end{align*}
%\end{proof}
%

\begin{lemma}[Alphabet-free Johnson bound]
	Let $F = (\fx,\fz)$ be a CSS code of distance $\delta$. Then for any $g\in \F_q^E$, 
	\begin{equation*}
		\abs{\calL( g, 1-\sqrt{1-\delta} ) } \leq q^d \cdot n +1
	\end{equation*}
\end{lemma}

\begin{proof}
	We use \cref{lem:covering} for $g$ to obtain a distribution $\calD$ over $F_X$ of support size at most $q^d \cdot n + 1$. This distribution has the property that for any $h \in \fx$ such that $\distR{g} < 1-\sqrt{1-\delta}$, it holds that
	\begin{equation}\label{eqn:covering}
		\Ex{f \sim \calD}{\distR{f}} < \delta
	\end{equation}
	Fix a coset in the list $\calL(g , 1-\sqrt{1-\delta} )$ and let $h$ be the codeword from this coset that is nearest to $g$, so that $\distR{g} < 1-\sqrt{1-\delta}$. We claim that the support of $\calD$ must contain a member of the coset $h+\cz^{\perp}$. If not, every $f \in \supp(\calD)$ satisfies $\distR{f} \geq \delta$ due to the distance of the code, and so,
	\[
		\Ex{f\sim \calD}{\distR{f}} \geq \delta
	\]
which contradicts \cref{eqn:covering}.

Since the total support of $\calD$ is bounded by $q^d \cdot n + 1$, the number of cosets in the list is also bounded by $q^d\cdot n +1$.
\end{proof}

\todo{Insert text here to be verbose.}

\begin{lemma}[Algorithmic Covering Lemma]\label{lem:algo_covering}
	Let $g\in \F_q^E$, $\alpha \in (0,1)$ and $\eps \in (0,1-\alpha)$. 
	There exists a pseudocodeword $\tildeEx{\cdot}$ of degree $t\geq d$ such that for every $h \in \fx$ such that $\distR{g} < 1-\alpha - \eps$, it holds that
	\[
		\distR{\tildeEx{\cdot}} < 1-\alpha^2 - 2 \alpha \eps \mper
	\]
	Moreover, such a pseudocodeword can be found in time $n^{\calO(t)}$.
\end{lemma}
%
\begin{proof}
	The required pseudocodeword can be found using the following convex program, where $\Psi \parens*{\tildeEx{\cdot}} = \ip{\tildeEx{\embed(\zee)}}{\tildeEx{\embed(\zee)}}$.
	\begin{center}
	\fbox{
	\begin{minipage}[t]{0.75\linewidth}
		\vspace{-5 pt}
		{\small
		\begin{align*}
    			&\mbox{minimize}\quad ~~ \Psi\left(\tildeEx{\cdot}\right) \label{sos:list_dec} \\
			&\mbox{subject to}\quad \quad ~\\
    			&\qquad \ip{\tildeEx{\chiTan(\zee)}}{\embed(g)} ~>~ \alpha + \eps \\
			&\qquad \tildeEx{\cdot}\ \text{is a pseudocodeword of SoS-degree } t
		\end{align*}}
	\vspace{-14 pt}
	\end{minipage}
	}%
	\end{center}
	If $\tildeEx{\cdot}$ is the optimal pseudocodeword found, we will argue that for every $h \in \fx$ such that $\distR{g} < 1-\alpha - \eps$, it holds that
	\begin{equation}\label{eqn:pexp_agreement}
		\ip{\tildeEx{\embed(\zee)}}{\embed(h)} > \alpha^2 + 2 \alpha \eps \mper
	\end{equation}
	This suffices to prove the lemma as 
	\begin{align*}
		\disR{\tildeEx{\cdot}}{h} &= \Ex{r\in R}{\tildeEx{\indi{\zee_r \neq h_r}}} \\
		&= \Ex{r\in R}{\tildeEx{1 - \indi{\zee_r = h_r}}} \\
		&= 1 - \Ex{r\in R}{\tildeEx{\indi{\zee_r = h_r}}} \\
		&= 1 - \Ex{r\in R}{\tildeEx{\ip{\embed(\zee_r)}{\embed(h_r)}}} \\
		&= 1- \ip{\tildeEx{\embed(\zee)}}{\embed(h)}
	\end{align*}
	
	We also note the following lower bound on $\Psi\parens[\Big]{\tildeEx{\cdot}}$:
	\begin{align}
		& \angles[\big]{\tildeEx{\embed(\zee)}\, , \,\tildeEx{\embed(\zee)}}\cdot \ip{\embed(g)}{\embed(g)} ~\geq~ \angles[\big]{\tildeEx{\embed(\zee)} \, , \, \embed(g)}^2 ~>~ (\alpha + \eps)^2 \\
		\implies \quad & \Psi\parens[\Big]{\tildeEx{\cdot}} ~=~ \angles[\big]{\tildeEx{\embed(\zee)}\, , \,\tildeEx{\embed(\zee)}} ~>~ (\alpha + \eps)^2 ~>~ \alpha^2 + 2\alpha \eps \label{eqn:lower_bound_entropy}
	\end{align}
	Suppose \cref{eqn:pexp_agreement} does not hold. Then there exists an $h\in \fx$ such that $\distR{g} < 1-\alpha - \eps$ (which is equivalent to $\ip{\embed(g)}{\embed(h)} > \alpha + \eps$), but
	\begin{align*}
		\ip{\tildeEx{\embed(\zee)}}{\embed(h)} \leq \alpha^2 + 2 \alpha \eps \mper
	\end{align*}
	For a $\tee \in [0,1]$ to be chosen later, consider the degree-$t$ pseudocodeword $\dupPE{\cdot}$ which can be evaluated for any (vector-valued) $t$-local function $\mu$ as
	\[
		\dupPE{\mu(\zee)} = (1-\tee)\cdot \tildeEx{\mu(\zee)} + \tee \cdot \mu(h) \mper
	\]
	Since every integral codeword like $h$ is in particular a degree-$t$ pseucodeword, this convex combination is also a degree-$t$ pseudocodeword, and it is also easy to see that $\ip{\dupPE{\embed(\zee)}}{\embed(g)} ~>~ \alpha + \eps$.
%	Here, we think of $h$ as an SoS-degree-$t$ pseudocodeword, so that by convexity, $\PExp_{\tee}[\cdot]$ is also an SoS-degree-$t$ pseudocodeword. We will show towards a contradiction that $\Psi(\PExp_{\tee}[\cdot]) < \Psi^*$.

	\begin{align*}
		\Psi\parens*{\dupPE{\cdot}}  &= \ip{\dupPE{\chiTan(\zee)}}{\dupPE{\chiTan(\zee)}} \\
		&= \ip{(1-\tee) \cdot \tildeEx{\chiTan(\zee)} + \tee\cdot \chiTan(h)}{(1-\tee)\cdot \tildeEx{\chiTan(\zee)}+\tee \cdot \chiTan(h)} \\
		&= (1-\tee)^2 \cdot \ip{\tildeEx{\chiTan(\zee)}}{\tildeEx{\chiTan(\zee)}} +2\cdot \tee(1-\tee)\cdot \ip{\tildeEx{\chiTan(\zee)}}{\chiTan(h)} + \tee^2\cdot \ip{\chiTan(h)}{\chiTan(h)}\\
		&\leq (1-\tee)^2\cdot \Psi\parens*{\tildeEx{\cdot}} +2\cdot \tee(1-\tee)\cdot \parens{\alpha^2 + 2\alpha \eps} +\tee^2
	\end{align*}

Optimizing over $\tee$, we choose 
\[
	\tee^* = \frac{\Psi\parens*{\tildeEx{\cdot}} - \parens{\alpha^2 + 2\alpha \eps}}{\Psi\parens*{\tildeEx{\cdot}}-2\parens{\alpha^2 + 2\alpha \eps}+1}
\]

Since $\Psi\parens*{\tildeEx{\cdot}} > \alpha^2 + 2\alpha \eps$ from \cref{eqn:lower_bound_entropy}, we get optimal $\tee^* >0$, which implies $\Psi\parens*{\dupPE{\cdot}} < \Psi\parens*{\tildeEx{\cdot}}$, contradicting the optimality of $\tildeEx{\cdot}$.
\end{proof}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> quantum/decoding_new.tex <==
\section{List Decoding Algorithm}\label{sec:decoding}
In this section, we show how to use the machinery of \cite{JST23} to develop a list decoding algorithm for the quantum codes obtained by AEL amplification. The two main components of this machinery are the (algorithmic) covering lemma and the (SoS) distance proof. The former lets us discover an object "containing" the list, while the latter allows the list elements to be extracted from this object.

We start with a subsection on covering lemmas (\cref{sec:covering}), which we then combine with the SoS distance proof from \cref{sec:sos_distance} in \cref{sec:combine}. We show how to derandomize the algorithm in \cref{sec:derandomization}, followed by the application to QLDPC codes in \cref{sec:near_mds}.

We stress that all the results in this section follow the outline from \cite{JST23}, except with minor changes to accommodate the differences in the quantum setting, such as the change from $\Delta_{L}(\cdot , \cdot)$ to $\Delta_{L,\cz^{\perp}}(\cdot , \cdot)$. We choose to write down the formal details due to these minor changes, but defer some proofs to the appendix if they are exactly same as in the classical case.
%\input{covering.tex}

input covering

\subsection{Putting things together}\label{sec:combine}
Next, we combine the algorithmic covering lemma \cref{lem:algo_covering} and the distance proof \cref{lem:sos_ael_distance} to give a list decoding algorithm. However, note that the distance proof is only applicable to $\eta$-good pseudocodewords, and the pseudocodeword found by \cref{lem:algo_covering} need not have this property.

To remedy this, we start with a lemma that says that the $\eta$-good property can be obtained by random conditioning. This technique is common in algorithmic applications of Sum-of-Squares, and first appeared in \cite{BRS11}. It was adapted for decoding in \cite{JST23}. Since the proof is exactly the same as in \cite{JST23}, we defer the proof to \cref{app:correlation_rounding}.

\begin{lemma}[Correlation Rounding]\label{lem:conditioning_eta_good}
	Let $\eta>0$, and $\tildeEx{\cdot}$ be a pseudocodeword of degree at least $2d\left(\frac{s^{3d}}{\eta^2}+1\right)$. Then there exists an integer $u^* \leq s^{3d}/\eta^2 $ such that 
	\[
		\Ex{r_1,r_2,\cdots,r_{u^*}}{\Ex{\li,\ri}{\tildecov\brackets*{\zee_{\li},\zee_{\ri} \vert \zee_{r_1},\zee_{r_2},\cdots,\zee_{r_{u^*}}}}} \leq \eta \mper
	\]
	where $r_1,r_2,\cdots r_{u^*}$ are independent randomly chosen vertices of $R$.
\end{lemma}
That is, conditioning on the neighborhoods of $u^*$ many randomly chosen vertices in $R$ renders the pseudocodeword $\eta$-good in expectation. This can be seen as a form of "sampling" from the pseudodistribution. Sampling from a true distribution of codewords can be seen as conditioning on all $n$ vertex neighborhoods in $R$, and a sampled codeword is always integral, which implies it is $\eta$-good with $\eta=0$. \cref{lem:conditioning_eta_good} shows that there is some non-convex property we can derive even with just constantly many conditionings, and that this argument is also valid for pseudodistributions that do not have high enough moments to support sampling.

We now get to the main technical theorem of this work that gives an algorithm to list decode codes constructed via quantum AEL amplification of unique decodable base codes. We first present a randomized version that outputs each codeword in the list $\calL$ with some small but constant probability. We can repeat this algorithm to output a list of cosets that contains the true list of cosets with probability arbitrarily close to 1. In the next subsection, we will derandomize this algorithm, but will end up with much bigger list sizes since pruning the list can be hard for quantum codes.

\begin{theorem}[List Decoding AEL amplification]\label{thm:list_decoding_ael}
	Let $(\fx, \fz)$ be the code obtained by applying quantum AEL amplification to the outer code $(\dx,\dz)$ and inner code $(\cx,\cz)$ of distance $\delta_{\inn}$ using an $(n,d,\lambda)$--expander graph. The inner code $(\cx,\cz)$ is over an alphabet $\Sigma$ of size $s$, so that $(\fx,\fz)$ is over alphabet $\Sigma^d$ of size $s^d$.

Suppose the code $(\dx, \dz)$ can be unique-decoded from radius $\delta_{\dec}$ in time $\calT(n)$. Assume that $\lambda < \delta_{\dec}$. 
	
	Then for any $\gamma > 0$, there exists an algorithm based on $s^{\calO(d)}/\eps^4$ levels of the SoS hierarchy that given $g\in \Sigma^E$, runs in time $\ln(1/\gamma) \cdot \brackets*{n^{s^{\calO(d)}/\eps^4} + \calT(n)}$ and produces a list $\calL'$ of cosets that contains the list of cosets $\calL \defeq \calL \parens*{g, \calJ\parens*{\delta_{\inn} - \frac{\lambda}{\delta_{\dec}}} - \eps }$ with probability at least $1-\gamma$. The size of $\calL'$ is at most $\widetilde{\Omega}_{s,d} \parens*{ \frac{\ln(1/\gamma)}{\eps^6} }$.
%The size of $\calL'$ is at most $n^{\calO(q^{3d}/\eps^4)}$.
\end{theorem}

\begin{proof}
	The decoding algorithm is presented as \cref{algo:ael-decoding}. 
	Recall that $\calL = \calL \parens*{g, \calJ\parens*{\delta_{\inn} - \frac{\lambda}{\delta_{\dec}}} - \eps }$ is the list of all cosets in $\ex/\ez^{\perp}$ that intersect the Hamming ball $\calB\parens*{g,\calJ\parens*{\delta_{\inn} - \frac{\lambda}{\delta_{\dec}}} - \eps}$.

%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[!ht]
\begin{algorithm}{List Decoding}{$g \in \Sigma^E$, $\gamma\in (0,1)$}{List of cosets $\calL' \subseteq \ex / \ez^{\perp}$ that contains $\calL = \calL \parens*{g, \calJ\parens*{\delta_{\inn} - \frac{\lambda}{\delta_{\dec}}} - \eps }$}\label{algo:ael-decoding}
%
\begin{itemize}
%
\item Pick $\eta = \frac{\eps^2 \delta_{\dec}}{16\delta_{\inn}}$ and $M = \frac{\ln(1 / \gamma)}{p \ln p}$, where $p = \frac{ \parens*{\delta_{\dec}}^2 \cdot \eps^6}{2^{12} \cdot s^{3d} \cdot \delta_{\inn}^4}$.
\item Use \cref{lem:algo_covering} to obtain a pseudocodeword of degree $t \geq 2d(\frac{s^{3d}}{\eta^2} + 1)$ such that for every $h\in \ex$ which satisfies $\distR{g} < \calJ\parens*{\delta_{\inn} - \frac{\lambda}{\delta_{\dec}}} - \eps$, it holds that
\[
	\distR{\tildeEx{\cdot}} ~<~ \delta_{\inn} - \frac{\lambda}{\delta_{\dec}} - \eps
\]
%
% Take $h = (\nfrac{n}{d})^{k-1} \cdot h'$.
%
%
\item Initialize $\calL' = \emptyset$.
\item Repeat $M$ times:
\begin{enumerate}[(i)]
	\item Choose $u$ uniformly at random from $\{1,2,\cdots , \frac{s^{3d}}{\eta^2}\}$.
	\item Choose a random subset $U \subseteq R$ of size $u$, and let $N(U)$ denote the edge neighborhood of $U$. Sample a random assignment $\sigma$ for $N(U)$ using the local distribution for this set of edges. That is, $\sigma$ is chosen with probability $\tildeEx{\indi{\zee_U = \sigma}}$.
	\item Condition $\tildeEx{\cdot}$ on $\zee_U = \sigma$, and let $\dupPE{\cdot} = \condPE{\cdot}{\zee_U = \sigma}$ be the conditioned pseudocodeword of degree $2d\parens*{\frac{s^{3d}}{\eta^2}+ 1} - 2\cdot d \cdot u \geq 2d$.
	\item Generate $y \in (\F_{q}^{b_{\out}})^L$ by independently sampling $\dupPE{\phi_X^{-1} (\zee_{\li})}$. That is, for $w \in \F_q^{b_{\out}}$, the probability that $y_{\li} = w$ is $\dupPE{\indi{\phi_X^{-1}(\zee_{\li}) = w}}$.
	\item Call the $X$-decoder of $(\dx,\dz)$ on $y$. If a coset $\dxz + \dz^{\perp}$ is found close to $y$,
	% with $\dxz \in \dx$ corresponding to $z\in \ex$, 
	then add to $\calL'$ the coset $\wphix(\dxz) + \ez^{\perp}$.
\end{enumerate}
\item Prune $\calL'$ to only include one representative per coset, via Gaussian elimination.
\item Return $\calL'$.
\end{itemize}
%
\vspace{5pt}
%
\end{algorithm}
\end{figure}
%%%%%%%%%%%%%%%%%

We now argue that the probability of all the cosets in $\calL$ being included in $\calL'$ is at least $1 - \gamma$. Fix such a coset in $\calL$ and let $h \in \Sigma^E$ be the nearest codeword to $g$ from this coset $h+\ez^\perp$, so that $\distR{g} < \calJ\parens*{\delta_{\inn} - \frac{\lambda}{\delta_{\dec}}} - \eps$. \cref{lem:algo_covering} implies that $\tildeEx{\cdot}$ satisfies
\begin{align}\label{eqn:agreement_before_conditioning}
	\distR{\tildeEx{\cdot}} ~<~ \delta_{\inn} - \frac{\lambda}{\delta_{\dec}} - \eps\;.
\end{align}
To be able to use the distance proof of \cref{lem:sos_ael_distance}, we need the pseudocodeword to be $\eta$-good. \cref{lem:conditioning_eta_good} shows that this can be obtained by random conditioning. In particular, there exists a $u^*\in \{1,2,\cdots ,\frac{s^{3d}}{\eta^2} \}$ such that,
\begin{equation}\label{eq:conditioning_eta_good}
		\Ex{r_1,r_2,\cdots,r_{u^*}}{\Ex{\li,\ri}{\tildecov\brackets*{\zee_{\li},\zee_{\ri} \vert \zee_{r_1},\zee_{r_2},\cdots,\zee_{r_{u^*}}}}} ~\leq~ \eta\;.
\end{equation}
Note that we picked $\eta = \frac{\eps^2 \delta_{\dec}}{16\delta_{\inn}}$ in \cref{algo:ael-decoding}, so that $u^*$ is bounded by a constant independent of $n$.

Suppose $u$ is chosen in step (i) of \cref{algo:ael-decoding} to be $u^*$, which happens with probability at least $\frac{\eta^2}{s^{3d}}$. Rewriting \cref{eq:conditioning_eta_good} with $U$ to denote the randomly chosen set $\{r_1,r_2,\cdots ,r_u\}$ and $N(U)\sub E$ to denote the set of all edges incident on $U \sub R$, we get
\begin{align*}
	\Ex{\substack{U\subseteq R \\ |U| = u}}{\Ex{\li,\ri}{\tildecov\brackets*{\zee_{\li},\zee_{\ri} \vert \zee_{N(U)}}}} ~\leq~ \eta, \\
\Ex{\substack{U\subseteq R, |U| = u \\ \sigma \sim \zee_{N(U)}}}{\Ex{\li,\ri}{\tildecov\brackets*{\zee_{\li},\zee_{\ri} \vert \zee_{N(U)} = \sigma}}} ~\leq~ \eta,
\end{align*}
where $\sigma \sim \zee_{N(U)}$ is used to denote that $\sigma \in \Sigma^{N(U)}$ is sampled according to the local distribution induced on $N(U)$ by $\tildeEx{\cdot}$.

That is, on average, we end up with an $\eta$-good pseudocodeword. We actually picked $\eta$ to be much smaller than the bound on average covariance we will be needing, so that the probability (over conditionings) of obtaining a weaker low covariance becomes very close to 1. This is needed to be able to take a union bound with some other low-probability events we will see soon. A simple application of Markov's inequality shows that the probability of obtaining an $\frac{\eps\delta_{\dec}}{4}$-good pseudocodeword is at least $1-\frac{\eps}{4\delta_{\inn}}$.
\begin{align}\label{eqn:eta_good}
\Pr{U,\sigma}{\Ex{\li,\ri}{\tildecov\brackets*{\zee_{\li},\zee_{\ri} \vert \zee_U = \sigma}} > \frac{\eps \delta_{\dec}}{4}} ~\leq~ \frac{4\eta}{\eps \delta_{\dec}} ~\leq~ \frac{\eps}{4\delta_{\inn}}\;.
\end{align}
%

Therefore, we started with a pseudocodeword that is close to $h$ (\cref{eqn:agreement_before_conditioning}), and then condition it to make it $\frac{\eps\delta_{\dec}}{4}$-good. We must also argue that this conditioned pseudocodeword is still close to $h$, at least with some probability. This probability cannot be made too large, and this is why we needed to ensure that the low average correlation property holds with probability close to 1, so that both of these hold simultaneously with some positive probability. To do this, we use the law of total expectation and another application of Markov's inequality,
\begin{align}
	\Ex{U,\sigma}{\distR{\condPE{\cdot}{\zee_U = \sigma}}} ~&=~ \Delta_R(\tildeEx{\cdot},h)\;, \\
	~&<~ \delta_{\inn} - \frac{\lambda}{\delta_{\dec}} - \eps\;, && (\text{Using }\cref{eqn:agreement_before_conditioning}) \\
	\implies \Pr{U,\sigma}{\distR{\condPE{\cdot}{\zee_U = \sigma}} \leq \delta_{\inn} - \frac{\lambda}{\delta_{\dec}} - \frac{\eps}{2}} ~&\geq~ \frac{\eps/2}{\delta_{\inn} - \frac{\lambda}{\delta_{\dec}} - \frac{\eps}{2}} ~\geq~ \frac{\eps}{2\delta_{\inn}}\;.\label{eqn:agreement_after_conditioning}
\end{align}

Using a union bound over \cref{eqn:eta_good} and \cref{eqn:agreement_after_conditioning}, we get
\begin{align}\label{eqn:union_bound}
	\Pr{V,\sigma}{\Ex{\li,\ri}{\tildecov\brackets*{\zee_{\li},\zee_{\ri} \vert \zee_U = \sigma}} ~\leq~ \frac{\eps \delta_{\dec}}{4} \text{ and } \distR{\condPE{\cdot}{\zee_U = \sigma}} \leq \delta_{\inn} - \frac{\lambda}{\delta_{\dec}} - \frac{\eps}{2}} ~\geq~ \frac{\eps}{4\delta_{\inn}}\;.
\end{align}

Suppose such a conditioning pair $(U,\sigma)$ is chosen in \cref{algo:ael-decoding}, and this happens with probability at least $\frac{\eps}{4\delta_{\inn}}$.

We define $\dupPE{\cdot} = \condPE{\cdot}{\zee_U = \sigma}$ as in \cref{algo:ael-decoding}, and let us call the corresponding covariance operator as $\dupCov\brackets*{\cdot}$. Rewriting \cref{eqn:union_bound}, we see that $\dupPE{\cdot}$ satisfies the following two properties:
\begin{gather*}
	\Ex{\li,\ri}{\dupCov\brackets*{\zee_{\li},\zee_{\ri}}} ~\leq~ \frac{\eps \delta_{\dec}}{4} \;, \\
	\distR{\dupPE{\cdot}} ~\leq~ \delta_{\inn} - \frac{\lambda}{\delta_{\dec}} - \frac{\eps}{2}\;.
\end{gather*}

Using the SoS distance proof for AEL from \cref{lem:sos_ael_distance} for $\dupPE{\cdot}$, we can use the above upper bound on $\distR{\dupPE{\cdot}}$ to deduce an upper bound on $\distLperp{\dupPE{\cdot}}$.
\begin{align*}
	&\distR{\dupPE{\cdot}} ~\geq~ \delta_{\inn} - \frac{\lambda + \eps \delta_{\dec} / 4}{\distLperp{\dupPE{\cdot}}} \\
	\implies \quad & \quad \frac{\lambda}{\delta_{\dec}} + \frac{\eps}{2} ~\leq~ \frac{\lambda + \eps \delta_{\dec}/4}{\distLperp{\dupPE{\cdot}}} \\
	\implies \quad & \distLperp{\dupPE{\cdot}} ~\leq~ \delta_{\dec} - \frac{\eps \delta_{\dec}}{4\parens*{\frac{\lambda}{\delta_{\dec}} + \frac{\eps}{2}}} ~\leq~ \delta_{\dec} - \frac{\eps \delta_{\dec}}{4 \delta_{\inn}}\;.
\end{align*}
%%%%%%%%%%%

We next wish to show that $y\in (\F_q^{b_{\out}})^L$ obtained by rounding $\tildeEx{\cdot}$ in step (iv) of \cref{algo:ael-decoding} can be used to find the coset $h+\ez^{\perp}$. Let $\dxh$ be the codeword in $\dx \sub (\F_q^{b_{\out}})^L$ corresponding to $h \in \ex$. In other words, $\dxh_{\li} = \unconx(h_{\li})$. 

Let $\dist{y, \dxh}$ denote the normalized Hamming distance between $y$ and $\dxh$, viewed as strings of length $n$ over the alphabet $\F_q^{b_{\out}}$. On average, $y$ satisfies
\begin{align*}
	\Ex{y}{ \dist{y, \dxh}} &= \Ex{y}{ \Ex{\li \in L}{\indi{y_{\li} \neq \dxh_{\li}}}} \\
	&= \Ex{\li \in L}{~\Ex{y}{ \indi{y_{\li} \neq \dxh_{\li}}}} \\
	&= \Ex{\li \in L}{~\Ex{y_{\li}}{ \indi{y_{\li} \neq \dxh_{\li}}}} \\
	&= \Ex{\li \in L}{~ \sum_{w}{ \dupPE{\indi{\unconx(\zee_{\li}) = w}} \indi{w \neq \dxh_{\li}}}} \\
	&= \Ex{\li \in L}{~ \dupPE{\indi{\unconx(\zee_{\li}) \neq \dxh_{\li}}}} \\
	&= \Ex{\li \in L}{~ \dupPE{\indi{\unconx(\zee_{\li}) \neq \unconx(h_{\li})}}} \\
	&= \Ex{\li \in L}{~ \dupPE{\indi{\zee_{\li} \not\in h_{\li} + \cz^{\perp}}}}\\
	&= \distLperp{\dupPE{\cdot}} ~\leq~ \delta_{\dec} - \frac{\eps \delta_{\dec}}{4 \delta_{\inn}} \mper
\end{align*}
%

Using Markov's inequality,
\begin{align*}
	\Pr{y}{ \dist{y, \dxh} \leq \delta_{\dec}} \geq \frac{\eps}{4\delta_{\inn}} \mper
\end{align*}
%

Suppose a $y$ is found in \cref{algo:ael-decoding} such that $\dist{y, \dxh} \leq \delta_{\dec}$, which happens with probability at least $\frac{\eps}{4\delta_{\inn}}$. Then the $X$-decoder of the $(\dx,\dz)$ code must return the coset $\dxh+ \dz^{\perp}$. Let $\dxz$ be a coset representative of $\dxh+\dz^\perp$ returned by the $X$-decoder of $(\dx,\dz)$. Using $\ez^{\perp} = \wphix(\dz^{\perp}) + \mathbb{F}_{q}^n \otimes \cz^{\perp}$ from \cref{prop:concat_dual}, 
\begin{align*}
	\dxh - \dxz ~&\in~ \dz^{\perp}\;, \\
	\wphix(\dxh - \dxz) ~&\in~ \ez^\perp\;, \\
	\wphix(\dxh) - \wphix(\dxz) ~&\in~ \ez^\perp\;, \\
	h - \wphix(\dxz) ~&\in~ \ez^\perp + \F_q^n \otimes \cz^\perp = \ez^\perp\;.
\end{align*}

Therefore, \cref{algo:ael-decoding} adds the coset $\wphix(\dxz)+\ez^\perp = h+\ez^\perp$ to $\calL'$. In conclusion, if the following three events happen, the coset $h + \ez^{\perp}$ is added to the list $\calL'$.
%
\begin{enumerate}
\item $u=u^*$ is chosen, which happens with probability at least $\frac{\eta^2}{s^{3d}}$.
\item The pair $(U,\sigma)$ to condition on is chosen such that \cref{eqn:union_bound} holds. Conditioned on previous event, this happens with probability at least $\frac{\eps}{4\delta_{\inn}}$.
\item A $y$ is generated so that $\dist{g,\dxh} \leq \delta_{\dec}$. Conditioned on above two events, this happens with probability at least $\frac{\eps}{4\delta_{\inn}}$.
\end{enumerate}
%

Therefore, in any iteration, the coset $h + \ez^{\perp}$ is added to the list $\calL'$ with probability at least,
\[
	p ~=~ \frac{\eta^2}{s^{3d}} \cdot \frac{\eps}{4\delta_{\inn}} \cdot \frac{\eps}{4\delta_{\inn}} ~=~ \frac{ \parens*{\delta_{\dec}}^2 \cdot \eps^6}{4096 \cdot s^{3d} \cdot \delta_{\inn}^4} ~=~ \Omega_{s,d,\delta_{\dec}} (\eps^6) \mper
\]

Note that this immediately implies an upper bound of $1/p$ on the list size, although we can get better list sizes (combinatorially) by appealing to the covering lemma and approximate \Caratheodory theorem.

Finally, we show that with enough repetitions, $\calL'$ must contain the entire list $\calL$ with high probability. The probability that a coset in $\calL$ does not get added to $\calL'$ in $M$ iterations is
\[
	(1-p)^M ~\leq~ e^{-p \cdot M}
\]

With a union bound over the entire list, which is of size at most $1/p$, the probability that any coset in $\calL$ is not present in $\calL'$ is at most
\[
	\frac{1}{p} \cdot e^{-p \cdot M} ~=~ e^{-p M \ln p} ~\leq~ \gamma \;\text{ if } M = \frac{\ln(1 / \gamma)}{p \ln p}. \qedhere
\]
%which is at most $\gamma$ if $M = \frac{\ln(1 / \gamma)}{p \ln p}$.
\end{proof}

\subsection{Derandomization}\label{sec:derandomization}

In this section, we show how to derandomize the list decoding \cref{algo:ael-decoding}. In this process, the size of the list $\calL'$ output by the algorithm may be significantly larger, and in particular may grow polynomially with $n$. In contrast, the list size for the probabilistic version was bounded by a constant independent of $n$. Once again, this derandomization is very similar to the one used by \cite{JST23}, and we only include it for completeness.

Suppose we have the same setting as in the last section, and we borrow notation from there to avoid defining the same objects twice. We wish to show that \cref{algo:ael-decoding} can be modified to deterministically output a list $\calL'$ of polynomial size that contains the true list $\calL$. There are three steps where \cref{algo:ael-decoding} makes random choices, and we will address each of them separately:
\begin{enumerate}
\item We try out all $\frac{s^{3d}}{\eta^2}$ possible values of $u$ instead of picking one randomly.
\item We try all pairs $(U,\sigma)$ to condition on. These are at most $n^{\frac{s^{3d}}{\eta^2}} \cdot s^{d\frac{s^{3d}}{\eta^2}}$ many in number, which causes a multiplicative overhead of $ (s^dn)^{\frac{s^{3d}}{\eta^2}}$ in running time and list size.
\item Finally, for independently rounded $y$, we use a standard technique called threshold rounding, also used in \cite{JST23}, to try out all possible $y$ that could be generated. This is described in the next \cref{lem:derandomized_decoding_from_distributions}.
\end{enumerate}
%
\begin{lemma}\label{lem:derandomized_decoding_from_distributions}
	Let $(\dx, \dz)$ be the outer code defined over alphabet $\F_q^{b_{\out}}$, which is unique decodable from distance $\delta_{\dec}\leq \delta/2$ in time $\calT(n)$. Given a pseudocodeword $\tildeEx{\cdot}$ with the property
	\[
		\distLperp{\tildeEx{\cdot}} \leq \delta_{\dec} \;\;\text{ for some $h\in \ex$,}
	\]
we can find the coset $h+\ez^{\perp}$ in time $\calO(q^{b_{\out}} n)\cdot\calT(n)$ with a deterministic algorithm.
%	there is at most one coset of $\dz^{\perp}$ that contains such that $\distLperp{\tildeEx{\cdot}}$
%	
%	collection of distributions $\calD = \inbraces{\calD_i}_{i\in [n]}$, each of them supported on $\F_{q^k}$ described as a collection $q^k$ weights that sum to 1, there is a unique codeword $h$ that satisfies
%	\[
%		%\calL(\calD,\delta_{\dec} - \eps) = \inbraces{ h\in \calC \suchthat \Ex{i}{\Ex{j\sim \calD_i}{\indi{h_i \neq j}}}<\delta_{\dec}-\eps}
%		\Ex{i}{\Ex{j\sim \calD_i}{\indi{h_i \neq j}}} \le \delta_{\dec}
%	\]
	\begin{proof}
	We will use $\tildeEx{\cdot}$ to obtain $|L|=n$ distributions over $\F_q^{b_{\out}}$, say $\{ \calW_{\li} ~|~ \li \in L\}$. We will not use the vector space structure of $\F_q^{b_{\out}}$ here and only view it as a set of size $t\defeq q^{b_{\out}}$. We identify elements of $\F_q^{b_{\out}}$ with those of $[t]$ under an arbitrary ordering, and henceforth, we will view each $\calW_{\li}$ as a distribution over $[t]$. If $w_{\li j}$ denotes the weight of distribution $\calW_{\li}$ on the symbol $j\in [t]$,
	\[
		w_{\li j} = \tildeEx{\indi{\phi_X^{-1}(\zee_{\li}) = j}}
	\]
	%This ensures that $\sum_{j\in [t]} w_{\li j} = 1$. We replace the randomized rounding to produce $y$ in step (iv) of \cref{algo:ael-decoding} by the following process:
%		\begin{enumerate}[(a)]
%			\item Define the cumulative sums $c_{\li j} = \sum_{j' \leq j}{ w_{\li j'}}$, so that $c_{ \li t} = 1$. Define $c_{i0} = 0$.
%			\item For each $\li\in L$, embed $\calW_{\li}$ into the interval $[0,1]$ as $q^k+1$ points $(c_{\li 0} = 0, c_{\li 1}, c_{\li 2},\cdots , c_{\li q^k} = 1)$.
%			\item Choose $\theta \in [0,1]$ uniformly at random.
%			\item Build $h'\in [q^k]^L$ coordinate-wise as follows. For $\li \in L$, if 
%			\[	
%				\theta\in \left[c_{\li (j-1)}, c_{\li j}\right),
%			\]
%			then $h'_{\li} = j$. This ensures that $\Pr{\theta}{h'_{\li} = j} = w_{\li j}$.
%		\end{enumerate}
	We round $\{ \calW_{\li} ~|~ \li \in L\}$ to an $h'\in (\F_q^{b_{\out}})^L$ vertex by vertex. Choose a random $\theta \in [0,1]$. For each $\li \in L$, $h'_{\li}$ is defined to be the smallest $j\in [t]$ such that  $\theta < w_{\li 1}+w_{\li 2} + \cdots  + w_{\li j}$. 
	%$\theta \geq w_{\li 1}+w_{\li 2} + \cdots  + w_{\li (j-1)}$ but
	
	As before, let $\dxh \in \dx$ be the codeword corresponding to $h\in \ex$, that is, $\dxh_{\li} = \unconx(h_{\li})$. Therefore, the probability of $h'_{\li} = j$ is precisely $w_{\li j}$, as before. These events across $\li \in L$ are no longer independent however. But linearity of expectation can be used to show that the key claim from the previous section, that the distance of $h'$ from $\dxh$ is at most $\delta_{\dec}$, continues to hold under this modified rounding. If this holds, $h'$ can be used to find $h+\ez^{\perp}$ using the unique decoder of $(\dx,\dz)$.
		\begin{align*}
			\Ex{\theta \in [0,1]}{\Delta(h',\dxh)} ~&=~ \Ex{\theta \in [0,1]}{\Ex{\li}{\indi{h'_\li \neq \dxh_\li}}} \\
			%&= \Ex{\theta \in [0,1]}{\Ex{\li}{ \indi{\theta \not\in [c_{\li(h_{\li}-1)}, c_{\li \dxh_{\li}}) }}} \\
			%&= \Ex{\li}{ \Ex{\theta \in [0,1]}{\indi{\theta \not\in [c_{\li(\dxh_{\li}-1)}, c_{\li \dxh_\li}) }}} \\
			~&=~\Ex{\li}{1 - w_{\li \dxh_\li}} \\
			~&=~ \Ex{\li}{\tildeEx{\indi{\unconx(\zee_{\li}) \neq \dxh_{\li}}}} \\
			~&=~ \Ex{\li}{\tildeEx{\indi{\unconx(\zee_{\li}) \neq \unconx(h_{\li})}}} \\
			~&=~ \Ex{\li}{\tildeEx{\indi{\zee_{\li} \not\in h_{\li} + \cz^{\perp} }}} \\
			~&=~ \distLperp{\tildeEx{\cdot}} ~\leq~ \delta_{\dec}\;.
		\end{align*}
		
		The fact that a common threshold $\theta$ shared by all $\li \in L$ is used to generate this rounding allows us to make a single random choice for $\theta$ instead of different random choices for each $\li \in L$. Moreover, the rounded $h'$ is exactly same if the threshold $\theta$ is perturbed without crossing any of the $|L| \cdot t = q^{b_{\out}}\cdot n$ values $\{ w_{\li 1}+w_{\li 2} + \cdots w_{\li j} \}_{\li\in L, j \in [t]}$. Therefore, we only need to try out roundings for $q^{b_{\out}}\cdot n$ many distinct thresholds, which proves the lemma.
	\end{proof}
\end{lemma}

\subsection{Near-MDS Quantum LDPC Codes list decodable up to Johnson bound}\label{sec:near_mds}

In this section, we show how instantiating the AEL amplification with unique decodable asymptotically good QLDPC codes leads to QLDPC codes near the (quantum) Singleton bound that can be list decoded up to the Johnson bound. 

\begin{theorem}[Near-MDS Codes decodable upto Johnson bound]\label{thm:near_mds_main}
	For any $0<\rho<1$, and for any $\nfrac{1}{2} >\eps_1, \eps_2>0$, there is an infinite family of quantum LDPC codes $(\fx,\fz)$ with the following properties:
	\begin{enumerate}[(i)]
		\item The rate of the code is at least $\rho$ and distance is at least $\frac{1-\rho-\eps_1}{2}$.
		\item The code is over an alphabet of size $2^{\calO(\eps_1^{-6}\log(1/\eps_1))}$.
		\item The code of blocklength $n$ can be list decoded from radius $\calJ(\frac{1-\rho - \eps_1}{2})-\eps_2$ in time $n^{\calO_{\eps_1}(1/\eps_2^4)}$.
	\end{enumerate}
\end{theorem}

\begin{proof}
We show how to instantiate \cref{thm:list_decoding_ael} to obtain such codes. 
We will use the AEL distance amplification based on a family of $(n,d,\lambda)$-expanders, with $d$ and $\lambda$ to be chosen later.

The inner code $\cC = (\cx,\cz)$ is chosen to be a quantum Reed-Solomon code of rate $\rho_0 \defeq \frac{\rho}{1-\eps_1}$ and distance $\frac{1-\rho_0}{2}$. Since the inner code has blocklength $d$, the alphabet size of $\cC$ must be at least $d$, and we choose $\cC$ to be defined over a finite field $\F_{2^{b_{\inn}}}$, where $b_{\inn} \leq 1+\log_2 d$. Using \cref{lem:field_downgrade}, we will view $\cC$ as a vector space CSS code with alphabet $\F_2^{b_{\inn}}$.
%We focus on the asymptotics and ignore issues such as the codes being defined over fields that are a power of $2$.

For the outer code $\cD = (\dx,\dz)$, we fold the binary QLDPC codes of \cite{LZ23:decodable} into blocks of size $b_{\out}$, with $b_{\out} = b_{\inn}\cdot \rho_0 d$ so that concatenation is well defined. The starting binary code from \cite{LZ23:decodable} is chosen to have rate $1-\eps_1$ that can be unique decoded from radius $\delta_{\dec}=\Omega(\eps_1^2)$, and these properties are preserved after folding.

Let $\lambda = \eps_1 \delta_{\dec},\;$ so that $\lambda \leq \Omega(\eps_1^3)$ and $d=\calO(1/\eps_1^6)$. The rate of the AEL-amplified code $(\fx,\fz)$ is $(1-\eps_1) \rho_0 = \rho$, and the distance is at least
\begin{align*}
	\frac{1-\rho_0}{2} - \frac{\lambda}{\delta_1} &~\geq~ \frac{1}{2} \parens*{1-\frac{\rho}{1-\eps_1}} - \frac{\lambda}{\delta_{\dec}} \\
	&~\geq~ \frac{1}{2} \parens*{1-\rho -2\eps_1 \rho} -\eps_1 \\
	&~\geq~ \frac{1-\rho}{2} - 2\eps_1
\end{align*}

The final code is defined over alphabet $\F_2^{b_{\inn}\cdot d}$, which is of size at most $ 2^{(1+\log d))d}  = 2^{ \calO\inparen{\eps_1^{-6}\log(1/\eps_1)}}$. Since AEL amplification preserves the LDPC property of the outer code, our final code $(\fx,\fz)$ is also LDPC. For list decodability, we use \cref{thm:list_decoding_ael} to claim that the above code can be list decoded from $\calJ(\frac{1-\rho}{2}-2\eps_1)-\eps_2$ in time $n^{\calO_{q,d,\delta_{\dec}}(1/\eps_2^4)} = n^{\calO_{\eps_1}(1/\eps_2^4)}$. The claimed parameters can be obtained by replacing $\eps_1$ by $\eps_1/4$. We note that the decoder above can be made deterministic as described in \cref{sec:derandomization}.
\end{proof}


==> quantum/distance.tex <==
\section{Distance Proofs}\label{sec:distance}

In this section, we prove that the folded AEL code, $\fold(\cD \circ_\varphi \cC)$ has large (fractional) distance, $\delta_R$, that can be made arbitrarily close to that of the inner code $\delta_\inn$ by picking a good enough expander.

\subsection{Partial Minimizer}
As mentioned before, one of the key objects we will use in the distance proof is a partial minimizer, which does not change the coset, but gets closer to the codeword we are measuring distance from.
For a fixed codeword $h \in \ex$, and any vector $z \in \F_q^E$ we define a new vector $\partmin(z,h)$    
\[	\partmin(z,h)_{\li} = \begin{cases}
		z_{\li} \;\; \text { if } \;\;  z_{\li} \not\in\,  h_{\li} + \cz^\perp \\[6pt]
		h_{\li} \;\; \text { if } \;\; z_{\li} \in\,  h_{\li} + \cz^\perp 
	\end{cases}
		\]
We observe that it satisfies two key properties,
\begin{align} 
&\text{ (\small{Coset-preserving}) } \;\;\; &&\partmin(z,h)_{\li} \in\, z_{\li} + \cz^\perp \;\; \forall\, \li \in L  \label{eqn:coset}\\[4pt]
	&\text{ (\small{Monotone}) } \;\;\;	&&\Delta(\partmin(z,h)_\ri, h_\ri) \leq \Delta(z_\ri, h_\ri) \;\; \forall \, \ri \in\, R \label{eqn:monotone}
\end{align}
 
\subsection{Distance proof}
                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                            
\begin{lemma}[Distance proof of AEL]\label{lem:zfc_dist}
Let $z,h \in \ex$ be non-equivalent codewords, \ie $z \not\in h + \ez^\perp$. Then,
\[\Delta_{R}(z,h) \geq \delta := \delta_\inn - \frac{\lambda}{\Delta_{L, \cz^\perp}(z,h)}  \] 	
 where $\Delta_{L,\cz^\perp} (z,h) = \Ex{\li \in L}{\one \braces[\big]{z_{\li} \not\in  h_{\li} + \cz^\perp}} $. Thus, the distance of the folded code $\fold(\cE)$ satisfies $\delta_R \geq \delta$.
\end{lemma}
\begin{proof}
	We will lower bound and upper bound the same quantity $\Delta_E(\partmin(z,h), h)$. Note that by \cref{eqn:coset}, we have $\Delta_{L,\cz^\perp} (z,h) = \Delta_{L,\cz^\perp} (\partmin(z,h),h)$.
	
	\begin{align*}
			\Ex{e\in E}{\partmin(z,h)_e \neq h_e} ~&=~ \Ex{\li\in L}{{\dist{\partmin(z,h)_{\li} , h_{\li} }}} \\
			~&\geq~ \Ex{\li\in L}{\indi{\partmin(z,h)_{\li} \not\in  h_{\li} + \cz^\perp} \cdot \dist{\partmin(z,h)_{\li},h_{\li} }} \\
			~&\geq~ \Ex{\li\in L}{\indi{\partmin(z,h)_{\li} \not\in  h_{\li} + \cz^\perp} \cdot \delta_\inn} \\
			~&=~ \delta_\inn \cdot \Delta_{L,\cz^\perp} (\partmin(z,h),h) \\
			~&=~ \delta_\inn \cdot \Delta_{L,\cz^\perp} (z,h)&& (\text{Using \cref{eqn:coset}}) .
	\end{align*}

	For the upper bound, we will use the expander mixing lemma~(\cref{lem:eml_bipartite}).
	\begin{align*}
		\Ex{e\in E}{{\indi{\partmin(z,h)_e \neq h_e}}} ~&\leq~ \Ex{(\li, \ri)\, \in\, E}{{ \indi{\partmin(z,h)_{\li} \neq h_{\li} } \cdot \indi{\partmin(z,h)_{\ri} \neq h_{\ri} }}} \\[4pt]
		~&\leq~ \Ex{\li, \ri}{{ \indi{\partmin(z,h)_{\li} \neq h_{\li} } \cdot \indi{\partmin(z,h)_{\ri} \neq h_{\ri} }}} + \lambda &&\text{( \cref{lem:eml_bipartite} )}\\[4pt]
		~&=~\Delta_{L} (\partmin(z,h),h)\cdot \Delta_R(\partmin(z,h),h) + \lambda  \\[4pt]
		~&=~ \Delta_{L,\cz^\perp} (\partmin(z,h),h)\cdot \Delta_R(\partmin(z,h),h) + \lambda &&\text{ (Definition of $\partmin$)} \\[4pt]
		~&=~ \Delta_{L,\cz^\perp} (z,h)\cdot \Delta_R(\partmin(z,h),h) + \lambda &&\text{( \cref{eqn:coset} )} \\[4pt]
		~&\leq~ \Delta_{L,\cz^\perp} (z,h)\cdot \Delta_R(z,h) + \lambda &&\text{( \cref{eqn:monotone} )}
%		~&=~ \Ex{\li \in L}{{ \indi{z_{\li} \not\in  h_{\li} + \cz^\perp} }} \cdot \Ex{\ri \in R}{{\indi{\partmin(z,h)_{\ri} \neq h_{\ri} }}} + \lambda && \text{By \cref{eqn:coset}}\\[4pt]
%		~&\leq~ \Ex{\li \in L}{{ \indi{z_{\li} \not\in  h_{\li} + \cz^\perp} }} \cdot \Ex{\ri \in R}{{\indi{z_{\ri} \neq h_{\ri} }}} + \lambda && \text{By \cref{eqn:monotone}}
\end{align*}
%	The last inequality is obtained by applying~\cref{eqn:monotone} for each $r$, by setting $S = N_R(r)$.
	 Comparing the two sides, we get  
	\begin{align*}
		\Delta_{R}(z,h)\cdot \Delta_{L, \cz^\perp}(z,h) + \lambda ~\geq~ \delta_\inn \cdot \Delta_{L, \cz^\perp}(z,h)
	\end{align*}
	Since $z\not\in h+ \ez^\perp$, there exists at least one vertex $\li \in L$ such that $z_\li \not \in h_\li + \cz^\perp$ and thus, $\Delta_{L,\cz^\perp} (z,h) > 0$.  Dividing by it gives the result.	
\end{proof}
%

By combining~\cref{cor:ael_rate} with the above distance bound~\cref{lem:zfc_dist}, we can deduce that using AEL machinery amplifies the distance of the base outer code. 
%\textit{good LDPC CSS codes} with inner codes yields codes that are near-MDS.\todo{Correct/prune. check theorem statement, esp the $\delta_{\out}$ part.}

\begin{theorem}\label{thm:ael_final}
Let $\cD$ be a $[[ n,k_{\out}, \delta_{\out}n]]_{q^k}$ CSS code and let $\cC$ be a $[[ d,k, \delta_{\inn}d]]_q$ CSS code.
Then, the folded AEL code, $\fold(\cE) = \fold(\cD\circ_\phi \cC)$ defines a $[[n,k_\out \cdot k, \delta_R \cdot n]]_{q^d}$ QECC where $\delta_R \geq \delta_{\inn} - \frac{\lambda}{\delta_{\out}}$.
\end{theorem}

%\begin{theorem}
%	Let $\cD$ be good quantum LDPC codes, and let $\cC$ be random CSS codes such that .. Then, $\fold(\cD\circ_\varphi \cC)$ defines a near-MDS
%\end{theorem}
%\todo{Say something about code distance amplification. How about "here is a near-MDS QLDPC code using AEL machinery"?}


==> quantum/prelims.tex <==
\section{Preliminaries}
\label{sec:prelims}

Throughout the paper, we will assume that $\F_q$-vector spaces are equipped with the Hamming metric and the usual bilinear form $\angles{u,v} = \sum_i u_iv_i$ and $V^\perp = \Set{w\mid \ip{v}{w} = 0,\, \forall\, v \in V}$. We will also work with $\R$-vector spaces equipped with the expectation inner product and norm.

\subsection{Quantum CSS codes and list decoding}
% 
% In this section, we define the notions of \textit{quantum (vector space) CSS codes} and \textit{list decodable (vector space) CSS codes}. 
%
\paragraph{Vector space CSS codes}
Calderbank--Shor, and Steane (independently) showed that a pair of subspaces over $\F_q$ define a
quantum code, if they satisfy a certain orthogonality condition. This construction is known as the CSS construction. The work~\cite{BGG22} shows that this construction can be generalized to the setup where the $\F_q$-linear subspaces have coefficients in a vector space $\F_q^d$.  This generalization is useful in formalizing the notion of \textit{folded CSS codes}, which is an extension of the classical coding theoretic operation of folding to the quantum setup. We will work with this general definition throughout the paper.   
 
%his construction can be slightly generalized to the setup when the linear codes are

\begin{definition}[Vector space CSS Codes] Let $d$ be a positive integer and let $\cx,\cz \subseteq \parens{\F_q^d}^n$ be $\F_q$-linear subspaces such that\footnote{The dual spaces, $\cx^\perp, \cz^\perp$, is with respect to the usual billinear form over $\F_q^{dn}$} $\cz^\perp \subseteq \cx$. Then, $\cC = (\cx, \cz)$ defines a $[[n,k,\delta n]]_{q^d}$ quantum code, where 
\[ 
k =  \dim (\cx) - \dim(\cz^\perp), \;\; \delta = \frac{1}{n} \min \braces[\big]{ \abs{v}\;\Big\lvert\; v \in (\cx\setminus \cz^\perp) \cup (\cz\setminus \cx^\perp)}.
\]
The weight $\abs{c}$, is the Hamming weight over the alphabet $q^d$.  When $d=1$, this is the usual CSS construction. The CSS code is \textit{low-density parity check} (LDPC) if there exist (row and column)-sparse parity check matrices, $\hx, \hz$, over $\F_q$ such that $\cx = \ker \hx$ and $\cz = \ker \hz$.
\end{definition}

\paragraph{Folding} \textit{Folding} is an element-wise syntactic operation in which vectors in $\F_q^{dn}$ are viewed as vectors in $\parens*{\F_q^d}^n$. Formally, let $V \subseteq \F_q^{nd}$ be a vector space over $\F_q$. For a vector $v \in V$, denote \[\fold(v) = (v^{(1)}, \cdots, v^{(n)}) \in \parens*{\F_q^d}^n \text{ where } v^{(i)} = (v_{(i-1)d+1},\cdots, v_{id})\in \F_q^d.\] Using this, one can fold a CSS code to a vector space CSS code since the bilinear form remains unchanged.
% This  transformation of the vectors of a subspace wherein we divide the coordinate into blocks of length $d$, and view these blocks as vectors in $\F_q^d$ rather than $\F_q$. We now formalize this.

%map each block into an element of $\F_{q^d}$. 

 %\[v = (v_1,\cdots, v_d, \cdots, v_{(n-1)d+1}, \cdots, v_{nd}) \mapsto \parens{\fold(v_1,\cdots, v_d), \cdots, \fold\parens{v_{(n-1)d+1}, \cdots, v_{nd}}} \]     

%\todo{Do we really need the definition of quantum code??}
%Let $\cC$ be a CSS code over $\F_q^n$. We say that two vectors are equivalent $u-v \in \cx^\perp$... \todo{Clash of notation, need a consistent one. Also, formalize this equivalence properly.}
%\begin{definition}[List of codewords]
%	For any $g\in [q]^n$, the list of codewords in $\calC$ that are at a distance less than
%        $\delta$ from $g$ is denoted by $\calL(g,\delta)$. That is $\calL(g,\delta) = \inbraces{h\in \calC \suchthat \dist{h,g} < \delta }$.
%\end{definition}
 
% \begin{definition}[vector space CSS codes and folding]
% A vector space CSS code is a CSS code,
% 	$. 
% \end{definition}
 
% \begin{definition}[Folded CSS code]
% Let $\cE$ be a CSS code over $\F_q^{nd}$ and let $\fold:\F_q^d \to \F_{q^d}$ be any $\F_q$-linear isomorphism. The folded code $\fold(\cE) =  (\fold(\ex), \fold(\ez))$ is defined as,
% \begin{align*}
% 	\fold(\ex) ~&=~ \Set*{\parens*{\fold(x^{(1)}), \cdots , \fold(x^{(n)})} \mid (x^{(1)}, \cdots, x^{(n)}) \in \ex} \subseteq \F_{q^d}^n , \\
% 	\fold(\ez) ~&=~ \Set*{\parens*{\fold(z^{(1)}), \cdots , \fold(z^{(n)})} \mid (z^{(1)}, \cdots, z^{(n)}) \in \ez} \subseteq \F_{q^d}^n .
% 	\end{align*} 
% \end{definition}
\begin{lemma}[Folded CSS Codes~{{\cite[Thm. 2.2]{BGG22}, \cite[Prop. 31]{GG23}}}]
 	 Let $\cE = (\ex, \ez)$ be a $[[nd, k, \delta]]_{q}$ CSS code. Denote by $\fold(\cE) = (\fold(\ex), \fold(\ez))$ a vector space CSS code where,
 \begin{align*}
 	\fold(\ex) ~=~ \Set*{\fold(x) \mid x \in \ex}, \qquad  \fold(\ez) ~=~ \Set*{\fold(z) \mid z \in \ez}.
% 	\fold(\ez) ~&=~ \Set*{\parens*{\fold(z^{(1)}), \cdots , \fold(z^{(n)})} \mid (z^{(1)}, \cdots, z^{(n)}) \in \ez} \subseteq \F_{q^d}^n .
\end{align*}
Then, $\fold(\cE)$ defines a $[[n,k, \delta_R\, n]]_{q^d}$ QECC, where,
\[ 
\delta_R = \frac{1}{n} \min \braces[\Big]{ \, \abs{v}\, \;\Big\lvert\; v \in \braces{\fold(\ex)\setminus \fold(\ez^\perp)} \cup \braces{\fold(\ez)\setminus \fold(\ex^\perp)}}.
\]
 \end{lemma}
% \todo{Theorem 2.2 does a simpler distance computation where each code already has distance $d$. Perhaps add a note.}
%\begin{remark}
%Note that $\fold(\ex)$ (or $\fold(\ez)x$) is $\F_q$-linear but not necessarily $\F_{q^d}$-linear, and therefore not a subspace. Thus, $\fold(\cE)$ does not define a CSS code. However, one can generalize the CSS construction to folded CSS codes and use them to define quantum codes over $\F_{q^d}$. 
%\end{remark}
%However, one can view the quantum code defined by $\cE$ as a quantum code over the larger alphabet $q^d$. The distance of this code then relates to the Hamming distance of the folded code $\cF$. 
%  they can still be used to define a quantum error correction code.  
%  Then, any subset of $S\subseteq \F_q^{nd}$ can be mapped to a subset of $f(S)\subseteq \F_{q^d}^{n}$. 
% over $\F_q^n$. The folded code is defined as $\cF = (\fx, \fz) :=  (f(\ex), f(\ez))$.

\paragraph{List decoding} We now formalize the notion of list decoding for quantum CSS codes and the folded codes. This is inspired by the classical definition but there are a couple of crucial changes in the quantum setup, (i) the input is no longer a corrupted codeword but a \textit{syndrome}, and (ii) the output is required to be a list \textit{containing} the list of possible errors. The first constraint is necessitated by the no-cloning theorem whereas the second relaxation is required as pruning the list can be difficult unlike in the classical case.

\begin{definition}[List of codewords]
Let $\cC = (\cx,\cz)$ be a vector space CSS code over $\parens*{\F_q^d}^n$. Let $B(g,\tau)$ denote a ball of fractional radius $\tau$, in the Hamming metric over $q^d$, around a vector $g$. For any pair of vectors $\subs{g}{X}, \subs{g}{Z} \in \parens*{\F_q^d}^n$, we define the following lists as lists of cosets of codewords, 
\begin{align*}
\calL_X (\subs{g}{X}, \tau) ~&=~ \braces[\Big]{\subs{h}{X} + \cz^\perp\, \mid \,\subs{h}{X} \in \cx,\,\; B(\subs{g}{X},\tau) \cap \inparen{\subs{h}{X} + \cz^\perp} \neq \emptyset},\\
\calL_Z (\subs{g}{Z}, \tau) ~&=~ \braces[\Big]{\subs{h}{Z} + \cx^\perp\, \mid \,\subs{h}{Z} \in \cx,\,\; B(\subs{g}{Z},\tau) \cap \inparen{\subs{h}{Z} + \cx^\perp} \neq \emptyset},\\
\calL (\subs{g}{X}, \subs{g}{Z},\tau) ~&=~ \calL_X (\subs{g}{X},\tau)\, \times\, \calL_Z (\subs{g}{Z},\tau).
\end{align*}
\end{definition}

%The notion of a list is identical for a folded code, except that the definition of a ball, $B(g,r)$, changes as now the distance is measured via the Hamming metric over $\F_{q^d}$ (instead of $\F_q$). 

We also define $\calL_e (\subs{g}{X}, \subs{g}{Z},\tau)$ as a list of cosets of errors, which is just the codeword list $\calL_e (\subs{g}{X}, \subs{g}{Z},\tau)$ shifted by $\subs{g}{X}$ and $\subs{g}{Z}$ respectively. When decoding from syndromes, all information about the original codeword is lost since the syndrome only depends on the error pattern. Therefore, one can only hope to output a list of errors rather than a list of codewords. In other words, since syndrome is invariant to translation by codewords, so should the output of a list decoding algorithm, and $\calL_e (\subs{g}{X}, \subs{g}{Z},\tau)$ is the translation-invariant version of $\calL (\subs{g}{X}, \subs{g}{Z},\tau)$.
%However, $\calL_e$ is invariant under translation by codewords which is necessary to decode from syndromes as all information about codewords is lost. Thus, one can only hope to output a list of errors rather than codewords 
\begin{align*}
\calL_e (\subs{g}{X}, \subs{g}{Z},\tau) ~&=~ \braces[\Big]{\parens[\big]{\subs{h}{X} -\subs{g}{X}  + \cz^\perp, \subs{h}{Z} - \subs{g}{Z}+ \cx^\perp}\, \mid \, \parens[\big]{\subs{h}{X} + \cz^\perp, \subs{h}{Z} +\cx^\perp} \in \calL (\subs{g}{X}, \subs{g}{Z},\tau)}\\[3pt]
~&=~ \parens*{\calL_X (\subs{g}{X},\tau) -\subs{g}{X}} \times \parens*{\calL_Z (\subs{g}{Z},\tau)-\subs{g}{Z}}\\[4pt]
~&=~\calL_e (\subs{g}{X}', \subs{g}{Z}',\tau) \qquad \text{for any}\qquad  \subs{g}{X}- \subs{g}{X}' \in \cx, \, \subs{g}{Z}- \subs{g}{Z}' \in \cz.
\end{align*} 
The last equality follows as the codes $\cx, \cz$ are linear and the Hamming metric is translation-invariant.
%Denote by $\calL_X(\cdot)$ and respectively $\calL_Z(\cdot)$ , the projection of this set to the first part (respectively, the second part). 



%Using the definition from~\cite{BGG22}, 

\begin{definition}[List Decodable vector space CSS codes, also in~\cite{BGG22}]
A quantum CSS code $\cC$ is $(\tau,L)$-\textit{list decodable} if for every $(\subs{g}{X}, \subs{g}{Z})$, the list size is bounded, \ie $\abs{\calL (\subs{g}{X}, \subs{g}{Z},\tau)} \leq L$.

 Fix a pair of parity check matrices $(\hx,\hz)$. We say that a code is \textit{efficiently list decodable} upto fractional radius $\tau$ if given $(\hx\subs{g}{X}, \hz\subs{g}{Z})$ such that $\subs{g}{X},\subs{g}{Z} \in B(0,\tau)$, there exists a $\poly(n)$-time algorithm that outputs a list that contains $\calL_e(\subs{g}{X}, \subs{g}{Z},\tau)$.  
% We say that a folded code, $\fold(\cC)$, is (efficiently) list decodable up to a radius $r$ (with respect to the Hamming metric over the larger alphabet) if the cosets $\cE$ is (efficiently) list decodable upto radius $r$.
\end{definition}
 
 
 \begin{observation} Assume that for any $(\subs{g}{X}, \subs{g}{Z})$, one can output the lists $\calL_X (\subs{g}{X}, \tau)$ and $\calL_Z (\subs{g}{Z}, \tau)$ in $\poly(n)$-time.  Then, the quantum CSS code is efficiently list decodable. 
% Let $\cC$ be a linear code with a translation-invariant  $d$. Then, the syndrome decoding task of an error $|e| < r$, is polynomial-time equivalent to the task of finding the nearest codeword in a ball of radius $r$.  	
 \end{observation}
 \begin{proof}
Given, $(\hx\subs{g}{X}, \hz\subs{g}{Z})$ one use Gaussian elimination to compute $(\subs{g}{X}', \subs{g}{Z}')$ such that $\subs{g}{X} - \subs{g}{X}' \in \cx$ and $\subs{g}{Z} - \subs{g}{Z}' \in \cz$. By the assumption we can compute $\calL_X (\subs{g}{X}',\tau)$ and $\calL_Z (\subs{g}{Z}',\tau)$, and therefore output, 
$\calL_e (\subs{g}{X}, \subs{g}{Z},\tau) = \parens[Bigg]{\calL_X (\subs{g}{X}',\tau) -\subs{g}{X}'} \times \parens[Bigg]{\calL_Z (\subs{g}{Z}',\tau)-\subs{g}{Z}'}$.
 \end{proof} 
 
 In summary, we can reduce the task of list decoding the classical codes $\fold(\ex)$ and $\fold(\ez)$ but \textit{upto cosets}. Moreover, our decoder will be symmetric and henceforth we will focus on the task of $X$-decoding. 
  
  
 \begin{summary}[List decoding folded codes]
 Let $\fold(\cE)$ be a folded CSS code over $\parens*{\F_q^d}^n$ with given parity-check matrices $(\hx,\hz)$. The task of efficient list decoding $\fold(\cE)$ upto radius $\tau$ reduces to the following two tasks,
 \begin{itemize}
 	\item \textup{\textbf{X-decoding}}: Given as input $\subs{g}{X} \in \parens*{\F_q^d}^n$, output a list, $\calL_X$ of cosets of codewords such that, 
 	\[ \calL_X (\subs{g}{X}, \tau)~\subseteq~ \calL_X' ~\subseteq~ \fold(\ex)/\fold(\ez^\perp).\]   
 	\item \textup{\textbf{Z-decoding}}: Given as input $\subs{g}{Z} \in \parens*{\F_q^d}^n$, output a list, $\calL_Z$ of cosets of codewords such that,
 	\[ \calL_Z (\subs{g}{Z}, \tau)~\subseteq~ \calL_Z' ~\subseteq~ \fold(\ez)/\fold(\ex^\perp).\] 
 \end{itemize}
 	
 \end{summary}

% Firstly, observe that from the definition of the lists, it suffices to compute $\calL_X(\subs{g}{X}) - \subs{g}{X} $ and $\calL_Z(\subs{g}{Z}) - \subs{g}{Z}$. This is because $\calL_e (\subs{g}{X}, \subs{g}{Z},r) \subseteq \parens*{\calL_X (\subs{g}{X},r) -\subs{g}{X}} \times \parens*{\calL_Z (\subs{g}{Z},r)-\subs{g}{Z}}$.
%
% Since the code $\cx$ is linear and the Hamming metric is translation-invariant, for any $\subs{g}{X}, \subs{g}{X}'$ such that $\subs{g}{X}- \subs{g}{X}' \in \cx$, we have $\calL_X (\subs{g}{X},r) -\subs{g}{X} = \calL_X (\subs{g}{X}',r) -\subs{g}{X}'$. Similarly, for $\calL_Z$.
%
%
%Therefore, one can output $\calL_e (\subs{g}{X}, \subs{g}{Z},r) \subseteq \parens[Bigg]{\calL_X (\subs{g}{X}',r) -\subs{g}{X}'} \times \parens[Bigg]{\calL_Z (\subs{g}{Z}',r)-\subs{g}{Z}'}$.

 
 
 %   \problemdef{Quantum list decoding}{For a CSS $\cE = (\cx, \cz)$, $\,\ker \hx = \cx, \, \ker \hz = \cz $, the quantum list decoding task is as follows}{$\subs{s}{X} := \hx(\subs{e}{X}), \; \subs{s}{Z} := \hz(\subs{e}{Z}) $ such that $\abs*{\subs{e}{X}}, \abs*{\subs{e}{Z}} \leq \delta_J n$.}{A list $L$ that contains $\calL (\subs{e}{X}, \subs{e}{Z})$.
%   }

%
%These notions can be directly extended to folded CSS codes. Let $\fold(\cE)$ be a folded code. Then, we say that it is list decodable up to a radius $r$ (with respect to the Hamming metric over the larger alphabet) if the CSS code $\cE$ is. Thus, list decoding $\fold(\cE)$ amounts to list decoding each of the classical linear codes $\ex$ and $\ez$ \textit{upto coset elements}. 
%\todo{Make decoding task more explicit}


% 
%Given $g$ such that $g \in B_d(h,\delta_J)$ for some codeword $h$, one can compute $s := Hg$ and then perform syndrome decoding.
%
%In the other direction, given $s$, one can use Gaussian elimination to compute $g$ such that $Hg = s$. Let $e$ be the small-weight error such that $He = s$. Then, $g-e \in C$ as $H(g-e) = s - s = 0$. Thus, $g \in B_d(h,\delta_J)$ for the codeword $h = g-e$.  	

 
 
% \begin{observation} If $\cx/\cz^\perp$ and $\cz/\cx^\perp$ are each efficiently $(r,L)$-list--decodable (respectively efficiently list decodable), then $\cC$ is $(r,L^2)$-list--decodable.   	
% \end{observation}
% \begin{proof}
% 	The list $\calL (\subs{g}{X}, \subs{g}{Z},r) \subseteq \calL_X (\subs{g}{X},r) \times \calL_Z (\subs{g}{Z},r)$.
% \end{proof}
 
 
% We say that a code is \textit{efficiently list decodable} if given $(\subs{g}{X}, \subs{g}{Z})$, one can output a list that contains $\calL(\subs{g}{X}, \subs{g}{Z})$ in $\poly(r,n)$-time. 


 
 
%\snote{Should the definition of $\calL(\cdot)$ already take into account that we only count non-equivalent codewords? This would make Johnson bound etc appear cleaner.}

%\paragraph{Decoding} Let $\cC = (\cx, \cz)$ be a CSS code with parity check matrices $(\hx, \hz)$ such that $\ker \hx = \cx$, $\ker \hz = \cz$. The task of quantum decoding for CSS codes is to compute 


%  
 
% \tnote{Should we just get rid of X,Z subscripts?}
% 
% \begin{observation} If $\cx, \cz$ are each $(r,L)$-list--decodable, then $\cC$ is $(r,L^2)$-list--decodable. 	
% \end{observation}
% \begin{proof}
% 	The list $\calL (\subs{e}{X}, \subs{e}{Z},r) \subseteq \calL (\subs{e}{Z},r) \times \calL (\subs{e}{Z},r)$.
% \end{proof}
% 
% \snote{$\cx \backslash \cz^{\perp}$ needs to be list decodable.}
% 
%<<<<<<< HEAD
%% \snote{$\cx \backslash \cz^{\perp}$ needs to be list decodable.}
%% 
%
%=======
% The above observation lets us focus on a single type of error which is the problem of list decoding for a classical linear code but \textit{upto coset elements}. 
%>>>>>>> 3bfa94cdd973c8dbe80852f205130da4aa19200f
% 
% \begin{observation} Let $\cC$ be a linear code with with a metric $d$. Then the syndrome decoding task of an error $|e| < r$, is polynomial-time equivalent to the task of finding the nearest codeword in a ball of radius $r$.  	
% \end{observation}
% \begin{proof}
%Given $g$ such that $g \in B_d(h,\delta_J)$ for some codeword $h$, one can compute $s := Hg$ and then perform syndrome decoding.
%
%<<<<<<< HEAD

%  the pair of classical codes over $\F_{q^d}^{n/d}$. Then, $\cF$ defines a 
% 
%   Denote by $N_\cE = \Set{dd}$, the normalizer group defining the quantum code.  
%=======
%In the other direction, given $s$, one can use Gaussian elimination to compute $g$ such that $Hg = s$. Let $e$ be the small-weight error such that $He = s$. Then, $g-e \in C$ as $H(g-e) = s - s = 0$. Thus, $g \in B_d(h,\delta_J)$ for the codeword $h = g-e$.  	
% \end{proof}
% 
%\snote{Add list decoding variant of reduction.}
%>>>>>>> 3bfa94cdd973c8dbe80852f205130da4aa19200f

%\snote{Write "task of nearest codeword" a bit more formally.}
% 
\subsection{Duality preserving maps} 

To generalize the notion of concatenation to quantum CSS codes, we will need the notion of duality-preserving maps. These are needed to properly define the concatenated code such that the orthogonality constraint, $\cz^\perp\subseteq \cx$, is satisfied, thereby defining a quantum CSS code. This has also been used in earlier works, for example, see~\cite{Ham08}. 

\begin{definition}[Dual Systems and Basis]\label{def:dual}
	Let $V,W$ be $\F_q$-vector spaces of equal dimension. Let $\ip{\cdot}{\cdot}$ be a non-degenerate bilinear map $V \times W \to \F_q$. Then, $(V,W,\ip{\cdot}{\cdot})$ defines a \textit{dual system}. A basis $\{v_1,\cdots, v_k\}$ of $V$, and $\{w_1,\cdots, w_k\}$ of $W$ is said to be \textit{dual} if $\ip{v_i}{w_j} = 
	\delta_{ij}$ for all $i,j \in [k]$.\end{definition}
The spaces $V,W$ are called \textit{dual spaces} as the bilinear map gives an isomorphism $W \to V^*$ defined as $w \mapsto \ip{w}{\cdot}$, which also proves the existence of such basis. This map is injective as the bilinear map is non-degenerate. Now, one can use the canonical dual basis of $V^*$. Using a dual basis, one can construct \textit{duality-preserving maps} which are what we will need. 
%
%Such a dual basis always exists for finite-dimensional vector spaces as the bilinear map can be used to construct an isomorphism $W \to V^*$ defined as $w \mapsto \ip{w}{\cdot}$. 
\begin{definition}[Duality preserving map]\label{def:dual_maps}
	Let $(V_1,V_2, \ip{\cdot}{\cdot}_V)$ and $(W_1,W_2, \ip{\cdot}{\cdot}_W)$ be two dual systems. A pair of linear maps $(\phi_1,\phi_2)$ where $\phi_i: V_i \to W_i $ are \textit{duality preserving} if,
	\begin{equation}
   \ip{u}{v}_V = \ip{\phi_1(u)}{\phi_2(v)}_{W}  \; \; \forall\, u,v \in V.
   \end{equation}
\end{definition}

\begin{claim}\label{claim:dual_map}
	Let $(V_1, V_2)$ and be $(W_1, W_2)$ dual systems along with their pairs of dual bases. Then, $\phi_i: V_i \mapsto W_i$ that acts as identity with respect to these dual bases is a duality-preserving map.  
\end{claim}
\begin{proof}
Since the condition is bilinear, it suffices to prove it for any pair of basis vectors of $V_1, V_2$. 
\begin{equation*}
   \ip{u_i}{v_j}_V = \delta_{ij} =    \ip{x_i}{y_j}_V = \ip{\phi_1(u_i)}{\phi_2(y_j)}_{W}.\qedhere
   \end{equation*} 
\end{proof}

%Such a map can be constructed by mapping the  elements of a dual basis for $(V_1, V_2)$ to a dual basis of $(W_1, W_2)$.


 We now define two different dual systems we work with. The first is $\F_{q^k}$, equipped with the \textit{trace form}, and the other comes from the CSS code equipped with the canonical bilinear form.
 
\begin{definition}[Trace Map]
	Let $\F_{q^k}$ be a degree $k$-extension of $\F_q$. The \textit{trace map}\footnote{We will drop the subscript as we will not work with multiple extensions.} is defined as 
	\[\mathsf{Tr}_{\,\F_{q^k}/\F_q} :\F_{q^k} \to \F_q, \;\;  x \mapsto x + x^q + x^{q^2} + \cdots + x^{q^k}.\]
	Note that $\mathsf{Tr}()$ is $\F_q$-linear as for any $a \in F_q$, $a^q = a$. Therefore it defines a non-degenerate $\F_q$-bilinear map over $\F_{q^k} \times \F_{q^k}$ defined as $\ip{x}{y}_\mathsf{Tr} = \mathsf{Tr} (xy)$.
\end{definition} 
 
 \begin{lemma}\label{lem:compl}Let $\cC = (\cx, \cz)$ be a CSS code over $\F_q^d$ of dimension $k$, and let $\cx = \subs{W}{X} \oplus \cz^{\perp}$ and $\cz = \subs{W}{Z}  \oplus \cx^{\perp}$ respectively. Then, the canonical bilinear form over $\F_q$ is non-degenerate over $\subs{W}{X} \,\times \,\subs{W}{Z}$. 
 Therefore, there exists a pair of $\F_q$--linear isomorphisms $\phix: \F_{q^{k}} \to W_X$, $\phiz: \F_{q^{k}} \to W_Z$ such that, 
\[
\mathsf{Tr}\, (xy) = \ip{\phix(x)}{\phiz(y)}_{\F_q^d}  \; \; \forall\, x,y \in \F_{q^k} \mper
\]
\end{lemma}
\begin{proof} If $(\subs{W}{X}, \subs{W}{Z} )$ equipped with the canonical bilinear form is a dual system, then~\cref{claim:dual_map} yields a duality-preserving isomorphism as needed. To show this, we only need to prove the non-degeneracy of the canonical form, and we will do so for one component as the argument is symmetric.

Assume that there exists $v \in \subs{W}{Z}$ such that $\ip{u}{v} = 0$ for all $u \in \subs{W}{X} $. Since, $v \in  \subs{W}{Z} \subseteq \cz$, we have $\ip{w}{v} = 0$ for all $w \in \cz^\perp$. But, $\cx = \subs{W}{X} \oplus \cz^\perp$ and therefore, $v \in \cx^\perp$. Since, $\subs{W}{Z} \cap \cx^\perp = \{0\}$, $v$ must be $0$. 
\end{proof}

%We encapsulate this discussion as a lemma we will use later.  
%
%\begin{lemma}Let $\cC = (\cx, \cz)$ be a CSS code over $\F_q^d$ of dimension $k$, and let $\cx = W_X \oplus \cz^{\perp}$ and $\cz = W_Z \oplus \cx^{\perp}$ respectively. \end{lemma}


%Let $\{\alpha_i\}, \{\beta_j\}$ be a pair of dual bases of $\F_{q^k}$ with respect to the trace map. $\{x_1,\cdots, x_k\}$ be a basis of $\subs{W}{X}$ and let $\{z_1,\cdots, z_k\}$ be a basis of $\subs{W}{X}$.
%
%Note that $\dim (\subs{W}{X}) = \dim (\subs{W}{X}) =  k = \dim(\F_{q^k})$. Now, 
%
%
%
%
%\begin{definition}[Duality preserving map]\label{def:dual_maps}
%	Let $(V_1,V_2, \ip{}{}_V)$ and  A pair of maps $\phix: \F_{q^{k}} \to \subs{W}{X}$, and $\phiz: \F_{q^{k}} \to \subs{W}{Z}$ be $\F_q$-linear isomorphisms such that,
%	\begin{equation}
%   \mathsf{Tr}\, (xy) = \ip{\phix(x)}{\phiz(y)}_{\F_q^d}  \; \; \forall\, x,y \in \F_{q^k}
%%    \end{equation}
%\end{definition}

%\begin{definition}[Dual Basis]\label{def:dual}
%	Let $\{\alpha_1,\cdots, \alpha_k\}$, $\{\beta_1,\cdots, \beta_k\}$ be a pair of bases of $\F_q^k$ as a vector space over $\F_q$. They are said to be \textit{dual} if 	$\mathsf{Tr}\, (\alpha_i\beta_j) = 
%	\delta_{ij}$ for all $i,j \in [k]$.
%\end{definition}
%
%\begin{fact}[{\cite[Theorem 19]{MS77}}]\label{fact:dual}
%	For any $q,k$ there exist dual basis for $\F_{q^k}$ over $\F_q$.
%\end{fact}



% Moreover, $\dim(W_X) = \dim(W_Z) = k$.
%
%Let $\phix$  be a linear isomorphism of $\F_q$-vector spaces  $\phix: \F_{q^{k}} \to W_X$. Analogously, let $\phiz$ be an isomorphism to $W_Z$. We call them \textit{complementary} if, 
%    \begin{equation}
%    \mathsf{Tr}\, (xy) = \ip{\phix(x)}{\phiz(y)}_{\F_q^d}  \; \; \forall\, x,y \in \F_{q^k}
%    \end{equation}

%\begin{definition}[Biorthogonal system]
%Let $V$ be a vector space with a bilinear form $\ip{\cdot}{\cdot}$. A pair of sequence of vectors, $\Set{x_1,\cdots, x_k}$ and $\Set{z_1,\cdots, z_k}$ is said to form a biorthogonal system if $\ip{x_i}{z_j} = \delta_{ij}$.
%\end{definition}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> quantum/sos_distance.tex <==
\section{SoS Proof of Distance}

In this section, we extend the distance proof of last section to pseudocodewords. We use the same definition of pseudocodewords as defined for classical AEL codes, and refer the reader to \cref{sec:sos_and_codes} for details.

We recall the following non-convex property from \cref{def:eta_good} that allows us to prove a distance property similar to \cref{lem:zfc_dist} for pseudocodewords.

\begin{definition}[Restatement of \cref{def:eta_good}]\label{def:eta_good_duplicate}
	A pseudocodeword is $\eta$-good if,
	\[
		\Ex{\li,\ri}{ \tildeCov{ \zee_{\li}}{\zee_{\ri} } } \leq \eta
	\]
\end{definition}
%\begin{definition}[Pseudocodeword]
%    A pseudoexpectation operator $\tildeEx{\cdot}$ of degree $t\geq d$ is called a pseudocodeword if it \emph{respects} the following constraint for all $\li \in L$,
%    \[
%        \one\inbraces{\zee_{\li}\not\in \cx} = 0
%    \]
%\end{definition}
%\snote{Need to set up $\tildeEx{\cdot}$ properly.}\tnote{in the above shouldn't it be $\one\inbraces{\zee_{\li}\in \cx}$?}


%\paragraph{SoS version} Since these definitions are local, we can also define it for pseudocodewords, which we will use later. The only changes are that we now ... \tnote{fill it up here?} There is no any significant change.  	Note that $\partmin(\zee, h)$ depends on $h$, but we only use it in analysis, and the algorithm does not need to compute (pseudoexpectations of) $\partmin(\zee)$. 

We extend the definition of partial minimizer to be a vector-valued local function that can be used inside pseudoexpectations. For a fixed codeword $h$, we define
\[
	\partmin(\zee,h)_{\li} = \begin{cases}
		\zee_{\li} \;\; \text { if } \;\;  \zee_{\li} \not\in\,  h_{\li} + \cz^\perp \\[6pt]
		h_{\li} \;\; \text { if } \;\; \zee_{\li} \in\,  h_{\li} + \cz^\perp 
	\end{cases}
\]
More explicitly, $\partmin(\zee,h)_{\li}$ is shorthand for $\indi{\zee_{\li} \not\in h_{\li} + \cz^{\perp}} \cdot \zee_{\li} + \indi{\zee_{\li} \in h_{\li} + \cz^{\perp}} \cdot h_{\li}$. Again, the partial minimizer $\partmin(\zee,h)$ satisfies the following two properties by definition.
%\todo{Rearrange these. Also, recall $\unconx$ }
%
\begin{align} 
	&\text{ (\small{Coset-preserving}) } \;\;\; &&\partmin(\zee,h)_{\li} \in\, \zee_{\li} + \cz^\perp \iff \phix^{-1}(\partmin(\zee,h)_{\li}) = \phix^{-1}(\zee_{\li}) \;\; \forall\, l \in L  \label{eqn:coset_sos}\\[4pt]
	&\text{ (\small{Monotone}) } \;\;\;	&&\indi{ \partmin(\zee, h)_r \neq h_r} \leq \indi{\zee_r \neq h_r} \;\; \forall \, r \in\, R \label{eqn:monotone_sos}
\end{align}
%
Recall that $\unconx$ is the local inversion map defined in \cref{def:concat}.
%\todo{Figure out $\phix^{-1}$}
%\begin{proof}
%	For any $\li$ and $\ri$,
%{\small
%	\begin{align*}
%		&\tildeEx{X_{\li}(\zee) \cdot Y_{\ri}(\zee)} - \tildeEx{X_{\li}(\zee)} \cdot \tildeEx{Y_{\ri}(\zee)} \\
%		&~=~ \sum_{\alpha \in [q]^{N_L(\li)} \atop \beta\in[q]^{N_R(\ri)}}
%                     \tildeEx{X_{\li}(\alpha) \prod_{s\in N_L(\li)} \zee_{s,\alpha_s} \cdot Y_{\ri}(\beta) \prod_{t\in N_R(\ri)} \zee_{t,\beta_t}} - 
%		 \sum_{\alpha \in [q]^{N_L(\li)} \atop \beta\in[q]^{N_R(\ri)}} \cdot \tildeEx{X_{\li}(\alpha) \prod_{s\in N_L(\li)} \zee_{s,\alpha_s}} \tildeEx{Y_{\ri}(\beta) \prod_{t\in N_R(\ri)} \zee_{t,\beta_t}} \\
%		&~=~ \sum_{\alpha,\beta} X_{\li}(\alpha) Y_{\ri}(\beta) \cdot \inparen{~\tildeEx{
%           \prod_{s\in N_L(\li)} \zee_{s,\alpha_s} \cdot \prod_{t\in N_R(\ri)} \zee_{t,\beta_t}} -
%           \tildeEx{\prod_{s\in N_L(\li)} \zee_{s,\alpha_s}} \cdot \tildeEx{\prod_{t\in N_R(\ri)} \zee_{t,\beta_t}}~} \\
%		&~\leq~  \norm{X_{\li}}_{\infty} \norm{Y_{\ri}}_{\infty} \cdot {\sum}_{\alpha,\beta}
%           \abs*{~\tildeEx{\prod_{s\in N_L(\li)} \zee_{s,\alpha_s} \prod_{t\in N_R(\ri)}
%           \zee_{t,\beta_t}} - \tildeEx{\prod_{s\in N_L(\li)} \zee_{s,\alpha_s}} \cdot \tildeEx{\prod_{t\in N_R(\ri)} \zee_{t,\beta_t}}~} \\
%		&~=~  \norm{X_{\li}}_{\infty} \norm{Y_{\ri}}_{\infty} \cdot \tildecov[\zee_{N_L(\li)},\zee_{N_R(\ri)}]
%	\end{align*}		
%}	
%	Averaging over $\li$ and $\ri$, we get
%%
%\begin{align*}
%\Ex{\li,\ri}{\tildeEx{X_{\li}(\zee) \cdot Y_{\ri}(\zee)} - \tildeEx{X_{\li}(\zee)} \cdot \tildeEx{Y_{\ri}(\zee)}} 
%	&~\leq~  \Ex{\li,\ri}{\norm{X_{\li}}_{\infty} \norm{Y_{\ri}}_{\infty} \cdot \tildecov[\zee_{N_L(\li)},\zee_{N_R(\ri)}]} \\
%	&~\leq~ \max_{\li}\norm{X_{\li}}_{\infty} \cdot \max_{\ri} \norm{Y_{\ri}}_{\infty} \cdot \Ex{\li,\ri}{\tildecov[\zee_{N_L(\li)},\zee_{N_R(\ri)}]} \\
%	&~\leq~ \eta \cdot \max_{\li}\norm{X_{\li}}_{\infty} \cdot \max_{\ri}
%   \norm{Y_{\ri}}_{\infty}
%\qquad \qquad \qquad \qquad  \qedhere
%\end{align*}
%%
%\end{proof}

Using this partial minimizer, we now prove an analog of distance for quantum codes based on AEL amplification. This is the main new contribution of our work, as the remaining parts of the proof can be adapted in a straightforward manner from \cref{chap:framework}.
\begin{lemma}[Distance proof]\label{lem:sos_ael_distance_quantum}
Let $\tildeEx{\cdot}$ be an $\eta$-good pseudocodeword and $h \in \F_q^E$ be such that $\fold(h)$ is a codeword in $ \fold(\ex)$ and $\distLperp{\tildeEx{\cdot}} > 0$. Then,
\[\distR{\tildeEx{\cdot}} \geq \delta_\inn - \frac{\lambda + 
\eta}{\distLperp{\tildeEx{\cdot}}}  \mper\] 	
\end{lemma}
\begin{proof}
	We will closely follow the proof of~\cref{lem:zfc_dist} and similarly, will lower bound and upper bound the quantity $\Ex{e\in E}{~\tildeEx{~\indi{\partmin(\zee, h)_e \neq h_e}}}$. 
%Note that by \cref{eqn:coset}, we have $\distLperp{\tildeEx{\cdot}} = \distLperp{\tildemin}$.	
\begin{align*}
			& \qquad \Ex{e\in E}{~\tildeEx{~\indi{\partmin(\zee, h)_e \neq h_e}}}\\
			~&=~ \Ex{\li\in L}{\tildeEx{\dist{\partmin(\zee, h)_{\li} , h_{\li} }}} \\
			~&\geq~ \Ex{\li\in L}{\tildeEx{\indi{\partmin(\zee, h)_{\li} \not\in h_{\li} + \cz^\perp} \cdot \dist{\partmin(\zee, h)_{\li} , h_{\li} }}} \\
			~&\geq~ \Ex{\li\in L}{\tildeEx{\indi{\partmin(\zee, h)_{\li} \not\in h_{\li} + \cz^\perp} \cdot \delta_{\inn} }} \\
			~&=~ \delta_{\inn} \cdot \Ex{\li\in L}{\tildeEx{\indi{\partmin(\zee, h)_{\li} \not\in h_{\li} + \cz^\perp} }} \\
			~&=~ \delta_{\inn} \cdot \Ex{\li\in L}{\tildeEx{\indi{\zee_{\li} \not\in h_{\li} + \cz^\perp} }} && (\text{Using \cref{eqn:coset_sos}}) \\
			~&=~ \delta_{\inn} \cdot \distLperp{\tildeEx{{\cdot}}}
	\end{align*}

For the upper bound, we will use the SoS version of expander mixing lemma, proved as \cref{lem:eml_for_pexp} in \cref{chap:framework}.
	\begin{align*}
		&\qquad \Ex{e\in E}{~\tildeEx{~\indi{\partmin(\zee, h)_e \neq h_e}}} \\
		~&\leq~ \Ex{\li \sim \ri}{~\tildeEx{~\indi{\partmin(\zee,h)_{\li} \neq h_{\li} } \cdot \indi{\partmin(\zee,h)_{\ri} \neq h_{\ri} }}} \\[4pt]
		~&\leq~ \Ex{\li, \ri}{\tildeEx{ \indi{\partmin(\zee, h)_{\li} \neq h_{\li} } \cdot \indi{\partmin(\zee, h)_{\ri} \neq h_{\ri} }}} + \lambda &&\text{( \cref{lem:eml_for_pexp} )}\\[4pt]
		~&\leq~ \Ex{\li, \ri}{\tildeEx{ \indi{\partmin(\zee, h)_{\li} \neq h_{\li} }} \cdot \tildeEx{\indi{\partmin(\zee, h)_{\ri} \neq h_{\ri} }}} + \lambda +\eta &&\text{( \cref{def:eta_good_duplicate} )}\\[4pt]
		~&=~ \Ex{\li}{\tildeEx{ \indi{\partmin(\zee, h)_{\li} \neq h_{\li} }}} \cdot \Ex{\ri}{\tildeEx{\indi{\partmin(\zee, h)_{\ri} \neq h_{\ri} }}} + \lambda +\eta \\[4pt]
		~&=~ \Ex{\li}{\tildeEx{ \indi{\zee_{\li} \not\in h_{\li} + \cz^{\perp}}}} \cdot \Ex{\ri}{\tildeEx{\indi{\partmin(\zee, h)_{\ri} \neq h_{\ri} }}} + \lambda +\eta &&\text{ (Definition of $\partmin$)} \\[4pt]
		~&\leq~ \Ex{\li}{\tildeEx{ \indi{\zee_{\li} \not\in h_{\li} + \cz^{\perp}}}} \cdot \Ex{\ri}{\tildeEx{\indi{\zee_{\ri} \neq h_{\ri} }}} + \lambda +\eta &&\text{( \cref{eqn:monotone_sos} )} \\[4pt]
		~&=~\distLperp{\tildeEx{\cdot}} \cdot \distR{\tildeEx{\cdot}}  + \lambda + \eta
%		~&=~ \distLperp{\tildemin} \cdot \distR{\tildemin}  + \lambda + \eta &&\text{ (Definition of $\partmin$)} \\[4pt]
%		~&=~ \distLperp{\tildeEx{\cdot}} \cdot \distR{\tildemin} + \lambda + \eta &&\text{( \cref{eqn:coset_sos} )} \\[4pt]
%		~&\leq~ \distLperp{\tildeEx{\cdot}} \cdot \distR{\tildeEx{\cdot}} + \lambda + \eta &&\text{( \cref{eqn:monotone_sos} )}
\end{align*}

Comparing the two sides, we get  
	\begin{align*}
		\distLperp{\tildeEx{\cdot}} \cdot \distR{\tildeEx{\cdot}} + \lambda + \eta  ~\geq~ \delta_{\inn} \cdot \distLperp{\tildeEx{{\cdot}}}
	\end{align*}
	Dividing by $\distLperp{\tildeEx{{\cdot}}}$ gives us the result.
	\end{proof}


%	 and dividing by $\Delta_{L,\cz^\perp} (z,h)$, we get
%	\begin{align*}
%		\Ex{\ri \in R}{\tildeEx{\indi{\zee_{\ri} \neq h_{\ri} }}} \geq \delta_1 - \frac{\lambda }{\Ex{\li\in L}{\tildeEx{\indi{\pi_1(\zee_{\li}) \neq \pi_1(h_{\li}) }}}}
%	\end{align*}
%\end{proof}

%\subsection{SoS distance proof}

%We let the maps $\pi_1, \pi_2$ be the projection maps from $\cx$ to $W_X$ and $\cz^{\perp}$ respectively. That is, any $y\in \cx$ can be uniquely written as a pair $(\pi_1(y), \pi_2(y))$ such that $y=y_1 + y_2$ and $\pi_1(y) \in W_X, \pi_2(y)\in \cz^{\perp}$.




% \begin{lemma}[Distance with wishful thinking]
%     Fix some $h\in E_X$. Let $\tildeEx{\cdot}$ be such that for all $\li \in L$, the following constraint is \emph{respected}:
%     \[
%         \indi{\pi_1(\zee_{\li}) = \pi_1(h_{\li})} \cdot \indi{\pi_2(\zee_{\li}) \neq \pi_2(h_{\li})} = 0
%     \]
%     Then,
%     \[
%         \Ex{e \in E}{\tildeEx{\one\inbraces{\zee_{e} \neq h_{e}}}} \geq \delta_1 \cdot \Ex{\li \in L}{\tildeEx{\one\inbraces{\pi_1(\zee_{\li}) \neq \pi_1(h_{\li})}}}
%     \]
% \end{lemma}

% \begin{proof}
%     \begin{align*}
%         \Ex{e \in E}{\tildeEx{\one\inbraces{\zee_{e} \neq h_{e}}}} =~ &\Ex{\li \in L}{\tildeEx{\Delta\left( \zee_{\li}, h_{\li} \right) }}\\
%         =~ &\Ex{\li \in L}{  \tildeEx{\indi{\pi_1(\zee_{\li}) = \pi_1(h_{\li})} \cdot \Delta \left( \zee_{\li}, h_{\li} \right)}} + \\ 
%         & \Ex{\li \in L}{\tildeEx{\indi{\pi_1(\zee_{\li}) \neq \pi_1(h_{\li})} \cdot \Delta \left( \zee_{\li}, h_{\li} \right)} } \\
%         =~ &\Ex{\li \in L}{  \tildeEx{\indi{\pi_1(\zee_{\li}) = \pi_1(h_{\li})} \cdot \indi{\pi_2(\zee_{\li}) = \pi_2(h_{\li})} \cdot \Delta \left( \zee_{\li}, h_{\li} \right)}} + \\ 
%         & \Ex{\li \in L}{\tildeEx{\indi{\pi_1(\zee_{\li}) = \pi_1(h_{\li})} \cdot \indi{\pi_2(\zee_{\li}) \neq \pi_2(h_{\li})} \cdot \Delta \left( \zee_{\li}, h_{\li} \right)} } + \\
%         & \Ex{\li \in L}{\tildeEx{\indi{\pi_1(\zee_{\li}) \neq \pi_1(h_{\li})} \cdot \Delta \left( \zee_{\li}, h_{\li} \right)} } \\
%         =~ & 0 ~+ \\ 
%         & 0 ~+ \\
%         & \Ex{\li \in L}{\tildeEx{\indi{\pi_1(\zee_{\li}) \neq \pi_1(h_{\li})} \cdot \Delta \left( \zee_{\li}, h_{\li} \right)} } \\
%         \geq~ & \Ex{\li \in L}{\tildeEx{\indi{\pi_1(\zee_{\li}) \neq \pi_1(h_{\li})} \cdot \delta_1} } \\
%         =~ & \delta_1 \cdot \Ex{\li \in L}{\tildeEx{\indi{\pi_1(\zee_{\li}) \neq \pi_1(h_{\li})}} }
%     \end{align*}
% \end{proof}

% \begin{lemma}[Wishful thinking is valid]
%     Fix $h \in E_X$. Let $\tildeEx{\cdot}$ be a pseudocodeword of degree $t \geq d$. Then there exists a pseudocodeword $\PExp^{h} \insquare{\cdot}$ of degree $t$ such that
%     \[
%         \Delta(\PExp^h \insquare{\cdot},h) \leq \Delta(\tildeEx{\cdot},h)
%     \]
%     and $\PExp^h \insquare{\cdot}$ \emph{respects}
%     \[
%         \one\inbraces{\pi_1(\zee_{\li}) = \pi_1(h_{\li})} \cdot \one\inbraces{\pi_2(\zee_{\li}) \neq \pi_2(h_{\li})} = 0.
%     \]
%     Moreover, for any $w\in W_X$,
%     \[
%         \tildeEx{\indi{\pi_1(\zee_{\li}) = w }} = \PExp^h \insquare{\indi{\pi_1(\zee_{\li}) = w }} 
%     \]
% \end{lemma}

% \begin{proof}
    
% \end{proof}
%\tnote{Do we need this concatenation lemma?}
%\begin{lemma}
%    Suppose $\dx$ can be (unique)-decoded up to the radius $\delta_2^{\dec}$. Given a pseudocodeword $\tildeEx{\cdot}$, we can find all $h\in E_X$ such that $\Delta(\tildeEx{\cdot},h) < \delta_1 \cdot \delta_2^{\dec}$.
%\end{lemma}
%
%\begin{proof}
%    \begin{align*}
%        \Delta(\tildeEx{\cdot}, h) = \Ex{e \in E}{\tildeEx{\one\inbraces{\zee_{e} \neq h_{e}}}} =~ &\Ex{\li \in L}{\tildeEx{\Delta\left( \zee_{\li}, h_{\li} \right) }}\\
%        \geq~ &\Ex{\li \in L}{\tildeEx{\indi{\pi_1(\zee_{\li}) \neq \pi_1(h_{\li})} \cdot \Delta \left( \zee_{\li}, h_{\li} \right)} } \\
%        \geq~ & \Ex{\li \in L}{\tildeEx{\indi{\pi_1(\zee_{\li}) \neq \pi_1(h_{\li})} \cdot \delta_1} } \\
%        =~ & \delta_1 \cdot \Ex{\li \in L}{\tildeEx{\indi{\pi_1(\zee_{\li}) \neq \pi_1(h_{\li})}} }\qedhere
%    \end{align*}
%\end{proof}


%% Commenting this part out
%We now define the SoS variant of our partial minimizer. $\phi$ denote the vector-valued local function defined as
%	\[
%		\partmin(\zee)_{\li} = \indi{\pi_1(\zee_{\li}) \neq \pi_1 (h_{\li})} \cdot \zee_{\li} + \indi{\pi_1(\zee_{\li}) = \pi_1 (h_{\li})} \cdot h_{\li}
%	\]
%	\tnote{How about writing it case-wise? Like this? }
%\[	\partmin(\zee)_{\li} = \begin{cases}
%		\zee_{\li} \;\; \text { if } \;\;  \zee_{\li} \not\in\,  h_{\li} + \cz^\perp \\[6pt]
%		h_{\li} \;\; \text { if } \;\; \zee_{\li} \in\,  h_{\li} + \cz^\perp 
%	\end{cases}
%		\]%	
%		
%	Note that $\partmin$ depends on $h$, but we only use it in analysis, and the algorithm does not need to compute (pseudoexpectations of) $\phi(\zee)$. It again satisfies the properties
%%	\begin{align*}
%%		\indi{\pi(Z)_{N(l)} \neq \pi(h_{N(l)})} &= \indi{\partmin(z,h)_{N(l)} \neq h_{N(l)}} \; \forall\, l \in L\\
%%		\phi(Z)_e &\leq Z_e\\
%%	\end{align*} 
%	
%	
%\begin{lemma}
%    Fix some $h\in E_X$. Let $\tildeEx{\cdot}$ be an $\eta$-good pseudocodeword.	
%%    such that for all $\li \in L$, the following constraint is \emph{respected}:
%%    \[
%%        \indi{\pi_1(\zee_{\li}) = \pi_1(h_{\li})} \cdot \indi{\pi_2(\zee_{\li}) \neq \pi_2(h_{\li})} = 0
%%    \]
%    Then,
%    \[
%        \Ex{\ri \in R}{ \tildeEx{\indi{\zee_{\ri} \neq h_{\ri}}}} \geq \delta_1 - \frac{\lambda + \eta}{\Ex{\li \in L}{\tildeEx{\indi{\pi_1(\zee_{\li}) \neq \pi_1(h_{\li})}}}}
%    \]
%\end{lemma}
%
%\begin{proof}
%
%	
%	We will lower bound and upper bound the same quantity $\dist{\phi(\zee), h} = \Ex{e\in E}{\tildeEx{\indi{\phi(\zee)_e \neq h_e}}}$.
%	
%	\begin{align*}
%			\Ex{e\in E}{\tildeEx{\indi{\phi(\zee)_e \neq h_e}}} &= \Ex{\li\in L}{\tildeEx{\dist{\partmin(\zee)_{\li} , h_{\li} }}} \\
%			&\geq \Ex{\li\in L}{\tildeEx{\indi{\partmin(\zee)_{\li} \neq h_{\li}} \cdot \dist{\partmin(\zee)_{\li} , h_{\li} }}} \\
%			&= \Ex{\li\in L}{\tildeEx{\indi{\pi_1(\zee_{\li}) \neq \pi_1(h_{\li}) } \cdot \dist{\partmin(\zee)_{\li} , h_{\li} }}} \\
%			&\geq \Ex{\li\in L}{\tildeEx{\indi{\pi_1(\zee_{\li}) \neq \pi_1(h_{\li}) } \cdot \delta_1}} \\
%			&= \delta_1 \cdot \Ex{\li\in L}{\tildeEx{\indi{\pi_1(\zee_{\li}) \neq \pi_1(h_{\li}) }}}
%	\end{align*}
%
%	For the upper bound, we will use the expander mixing lemma.
%	\begin{align*}
%		\Ex{e\in E}{\tildeEx{\indi{\partmin(\zee)_e \neq h_e}}} &\leq \Ex{\li \sim \ri}{\tildeEx{ \indi{\partmin(\zee)_{\li} \neq h_{\li} } \cdot \indi{\partmin(\zee)_{\ri} \neq h_{\ri} }}} \\
%		&\leq \Ex{\li, \ri}{\tildeEx{ \indi{\partmin(\zee)_{\li} \neq h_{\li} } \cdot \indi{\partmin(\zee)_{\ri} \neq h_{\ri} }}} + \lambda \\
%		&\leq \Ex{\li, \ri}{\tildeEx{ \indi{\partmin(\zee)_{\li} \neq h_{\li} }} \cdot \tildeEx{\indi{\partmin(\zee)_{\ri} \neq h_{\ri} }}} + \lambda + \eta \\
%		&=\Ex{\li}{\tildeEx{ \indi{\partmin(\zee)_{\li} \neq h_{\li} }}} \cdot \Ex{\ri \in R}{\tildeEx{\indi{\partmin(\zee)_{\ri} \neq h_{\ri} }}} + \lambda + \eta \\
%		&=\Ex{\li}{\tildeEx{ \indi{\pi_1(\zee_{\li}) \neq \pi_1(h_{\li}) }}} \cdot \Ex{\ri \in R}{\tildeEx{\indi{\partmin(\zee)_{\ri} \neq h_{\ri} }}} + \lambda + \eta \\
%		&\leq \Ex{\li}{\tildeEx{ \indi{\pi_1(\zee_{\li}) \neq \pi_1(h_{\li}) }}} \cdot \Ex{\ri \in R}{\tildeEx{\indi{\zee_{\ri} \neq h_{\ri} }}} + \lambda + \eta
%	\end{align*}
%	
%	Comparing the two sides and dividing by $\Ex{\li\in L}{\tildeEx{\indi{\pi_1(\zee_{\li}) \neq \pi_1(h_{\li}) }}}$, we get
%	\begin{align*}
%		\Ex{\ri \in R}{\tildeEx{\indi{\zee_{\ri} \neq h_{\ri} }}} \geq \delta_1 - \frac{\lambda + \eta}{\Ex{\li\in L}{\tildeEx{\indi{\pi_1(\zee_{\li}) \neq \pi_1(h_{\li}) }}}}
%	\end{align*}
%\end{proof}
%\fi

==> quantum/sos_prelims.tex <==
\section{Additional Preliminaries: Sum-of-Squares Hierarchy}

The sum-of-squares hierarchy of semidefinite programs (SDPs) provides a family of increasingly
powerful convex relaxations for several optimization problems. 
%
Each ``level" $t$ of the hierarchy is parametrized by a set of constraints corresponding to
polynomials of degree at most $t$ in the optimization variables. While the relaxations in the
hierarchy can be viewed as  semidefinite programs of size $n^{O(t)}$ \cite{BS14, FKP19}, 
it is often convenient to view the solution as a linear operator, called the ``pseudoexpectation" operator.
%
% It is well-known that such constrained pseudoexpectation operators of SoS-degree $t$ can be described as solutions to semidefinite programs of size $n^{O(t)}$ \cite{BS14, Laurent09}. This hierarchy of semidefinite programs for increasing $t$ is known as the SoS hierarchy.


%
%
\vspace{-5 pt}
%
\paragraph{Pseudoexpectations}
%
Let $t$ be a positive even integer and fix an alphabet $[q]$. Let $\zee = \{Z_{i,j}\}_{i\in[m],j\in[q]}$ be a collection of variables and $\R[\zee]^{\leq t}$ be the vector space of polynomials of degree at most $t$ in the variables $\zee$ (including the constants). 





\begin{definition}[Constrained Pseudoexpectations]\label{def:constraints_on_sos}
%	 
Let $\calS = \inbraces{f_1 = 0, \ldots, f_m = 0, g_1 \geq 0, \ldots, g_r \geq 0}$ be a system of
polynomial constraints in $\zee$, with each polynomial in $\calS$ of degree at most $t$. We say $\tildeEx{\cdot}$ is a pseudoexpectation operator of SoS-degree $t$, over the variables $\zee$  respecting $\calS$, if it is a linear operator $ \tildeEx{\cdot}: \R[\zee]^{\leq t} \rightarrow \R$ such that:
	%
	\begin{enumerate}
	\item $\tildeEx{1} = 1$.
    \item $\tildeEx{p^2} \geq 0$ if $p$ is a polynomial in $\zee = \{Z_{i,j}\}_{i\in [m],j\in [q]}$ of degree $\leq t/2$.
	\item $\tildeEx{p \cdot f_i} = 0$,  $\forall\, i \in [m]$ and $\forall p$ such that $\deg(p \cdot f_i) \leq t$.
	\item $\tildeEx{p^2 \cdot \prod_{i \in S} g_i} \geq 0$, $\forall\, S \subseteq [r]$ and $\forall\, p$ such that $\deg(p^2\cdot \prod_{i \in S} g_i) \leq t$.
	\end{enumerate}
\end{definition}

%\tnote{Suggestion -- directly define the constrained version. Attempting to make the connection with assignments a bit more explicit below.}

% An SoS solution of degree $t$, or a pseudoexpectation of SoS-degree $t$, over the variables $\zee$ is represented by a linear operator $ \tildeEx{\cdot}: \R[\zee]^{\leq t} \rightarrow \R$ such that:
%%
%\vspace{-5 pt}
%%
%\begin{enumerate}[(i)]
%    \item $\tildeEx{1} = 1$.
%    \item $\tildeEx{p^2} \geq 0$ if $p$ is a polynomial in $\zee = \{Z_{i,j}\}_{i\in [m],j\in [q]}$ of degree $\leq t/2$.
%\end{enumerate}
%%
%\vspace{-5 pt}
%%
%\tnote{Is the note needed? It is reiterating that it is a linear operator}
% Note that linearity implies $\tildeEx{p_1} + \tildeEx{p_2} = \tildeEx{p_1+p_2}$ and $\tildeEx{c\cdot
%  p_1} = c \cdot \tildeEx{p_1}$ for $c\in \R$, for $p_1, p_2 \in \R[\zee]^{\leq t}$.
%%
%This also allows for a succinct representation of $\tildeEx{\cdot}$ using any basis for $\R[\zee]^{\leq t}$.
%
%\tnote{ }

% to $m$ variables in alphabet $[q]$.

Let $\mu$ be a distribution over the set of assignments, $[q]^m$.  Let $\zee = \{Z_{i,j}  = \indi{ i \mapsto j} \}_{i\in[m],j\in[q]}$ be a collection of random variables. Then, setting $\tildeEx{p(\zee)} = \Ex{\mu}{p(\zee)} $ for any polynomial $p(\cdot)$ defines an (unconstrained) pseudoexpectation operator. 

However, the reverse is not true when $t < m$, and there can be degree-$t$ pseudoexpectations that do
not correspond to any genuine distribution, $\mu$. Therefore, the set of all pseudoexpectations should be seen as a relaxation for the set of all possible distributions over such assignments. The upshot of this relaxation is that it is possible to optimize over the set. 

Under certain conditions on the bit-complexity of solutions~\cite{OD16, RW17:sos}, one can optimize over the set of degree-$t$ pseudoexpectations in time $m^{O(t)}$ via SDPs.

%   setting the true expectation operator under this distribution is also a . 
%
%
%Given an assignment $f: [m] \rightarrow [q]$, the operator $\tildeEx{Z_{i_1,j_1}\cdots Z_{i_k,j_k}} = \indi{ j_t = f(i_t) \; \forall\, t }$
%\[
%f: [m] \rightarrow [q] ~\mapsto~  \tildeEx{Z_{i_1,j_1}\cdots Z_{i_k,j_k}} = \indi{ j_t = f(i_t) \; \forall\, t }
%\]
%can be seen as a pseudoexpectation that assigns the value $1$ to a monomial consistent with $f$ and $0$ otherwise. 

%
%This can be extended via linearity to all
%polynomials, and then by convexity of the constraints to all distributions over assignments.
%


 
%
%We next define what it means for pseudoexpectations to satisfy some problem-specific constraints.
%\[
% \left\{ \substack{\text{ True expectations} \\
%\text{ \ie for an assignment } f: [m] \rightarrow [q] \\\tildeEx{Z_{} \cdots Z_{}} =  } \right\} \subset  \{ \text{ SoS Pseudoexpectations }  \}
%\]

% Indeed, any assignment $f: [m] \rightarrow [q]$ has a corresponding pseudoexpectation described below.

% Let $z^{(f)}_{i,j} = \indi{f(i) = j}$, where $\indi{\cdot}$ is the $0/1$ indicator function. Then the pseudoexpectation corresponding to assignment $f$ is given by
% \begin{align*}
% 	\PExp^{(f)}[{p(\zee)}] = p\inparen{\inbraces{z^f_{i,j}}_{i\in[m],j\in[q]}}
% \end{align*}

% for every polynomial $p$ of degree at most $t$.

% As can be verified easily, the set of pseudoexpectations is convex, and so we can also extend this correspondence to distributions over assignments in a natural way. If $\PExp^{(\calD)}[{\cdot}]$ is the pseudoexpectation corresponding to a distribution $\calD$ over assignments, it holds that
% \[
% 	\PExp^{(\calD)}[{p(\zee)}] = \Ex{f\sim \calD}{p\inparen{\inbraces{z^f_{i,j}}_{i\in[m],j\in[q]}}}
% \]
% which explains the term pseudo-expectation.

% However, pseudoexpectations only exist for low-degree polynomials, and there can be pseudoexpectation operators that do not correspond to any genuine distribution over assignments. The main reason for working with pseudoexpectations instead of genuine distributions is that the set of SoS-degree $t$ can be optimized over in time $m^{O(t)}$ via SDPs.

% As a relaxation, pseudoexpectations are used in efficient algorithm design when coupled with
% suitable rounding algorithms. 
% %
% For such applications (including ours), it is important to look at relaxations that satisfy certain problem-specific constraints. We define next what it means for pseudoexpectations to satisfy constraints.

% \paragraph{Constrained Pseudoexpectations}
% 

%
%
\paragraph{Local constraints and local functions.}
%
Any constraint that involves at most $k$ variables from $\zee$, with $k\leq t$, can be written as a degree-$k$ polynomial, and such constraints may be enforced into the SoS solution.
%
% \paragraph{Canonical usage}
%
In particular, we will always consider the following canonical constraints on the variables $\zee$.
\ifnum\confversion=1
\begin{align*}
&Z_{i,j}^2 = Z_{i,j},\ \forall i\in[m],j\in[q] \\
\text{and} \quad &\sum_j Z_{i,j} = 1,\ \forall i\in[m] \mper
\end{align*}
\else
\[
Z_{i,j}^2 = Z_{i,j},\ \forall i\in[m],j\in[q] 
\quad \text{and} \quad 
\sum_j Z_{i,j} = 1,\ \forall i\in[m] \mper
\]
\fi
% As shown in the previous section, an assignment $f:[m]\rightarrow [q]$ is encoded using $m$ characteristic vectors, and so we wish to impose the following local constraints on the variables $\zee$:
%
% \begin{enumerate}[(i)]
% 	\item $Z_{i,j}^2 = Z_{i,j},\ \forall i\in[m],j\in[q]$.
% 	\item $\sum_j Z_{i,j} = 1,\ \forall i\in[m]$.
% \end{enumerate}
%
% These constraints are enforced as described in \cref{def:constraints_on_sos}, and we will henceforth not explicitly mention it. \snote{See Madhur's comment.}
%
We will also consider additional constraints and corresponding polynomials, defined by ``local" functions. For any $f\in [q]^m$ and $M\sub [m]$, we use $f_M$ to denote the restriction $f|_M$, and $f_i$ to denote $f_{\{i\}}$ for convenience.
%
\begin{definition}[$k$-local function]
	A function $\mu: [q]^m \rightarrow \R$ is called $k$-local if there is a set $M\subseteq [m]$ of size $k$ such that $\mu(f)$ only depends on $\inbraces{f(i)}_{i\in M}$, or equivalently, $\mu(f)$ only depends on $f|_M$.
	
	If $\mu$ is $k$-local, we abuse notation to also use $\mu: [q]^M \rightarrow \R$ with $\mu(\alpha) = \mu(f)$ for any $f$ such that $f|_M=\alpha$. It will be clear from the input to the function $\mu$ whether we are using $\mu$ as a function on $[q]^m$ or $[q]^M$.
\end{definition}

Let $\mu:[q]^m\rightarrow \R$ be a $k$-local function that depends on coordinates $M\subseteq [m]$ with $|M|=k$. Then $\mu$ can be written as a degree-$k$ polynomial $p_{\mu}$ in $\zee$:
\[
	p_{\mu}(\zee) = \sum_{\alpha \in [q]^M} \inparen{\mu(\alpha) \cdot\prod_{i\in M} Z_{i,\alpha_i}}
\]

% To see how $p_{\mu}$ is related to the $k$-local function $\mu$, observe that $p_{\mu}\inparen{\zee = \inbraces{z^{(f)}_{i,j}}} = \mu(f)$.

With some abuse of notation, we let $\mu(\zee)$ denote $p_{\mu}(\zee)$. We will use such $k$-local
functions inside $\tildeEx{\cdot}$ freely without worrying about their polynomial
representation. For example, $\tildeEx{ \indi{\zee_{i} \neq j}}$ denotes $\tildeEx{ 1- Z_{i,j}}$. 
%
% $\tildeEx{\cdot}$ operator applied to the polynomial corresponding to the $1$-local function $\mu: [q]^m \rightarrow \R$ which is defined as: $\mu(f)$ is $1$ if $f_i = 0$ and $\mu(f) = 0$ otherwise.
% %
The notion of $k$-local functions can also be extended from real valued functions to vector valued functions in a straightforward way.

\begin{definition}[vector-valued local functions]
A function $\mu: [q]^m \rightarrow \R^N$ is $k$-local if the $N$ real valued functions corresponding to the $N$ coordinates are all $k$-local. Note that these different coordinate functions may depend on different sets of variables, as long as the number is at most $k$ for each of the functions.
\end{definition}
%
\vspace{-5 pt}
%
\paragraph{Local distribution view of SoS}

It will be convenient to use a shorthand for the function $\indi{\zee_S = \alpha}$, and we will use $\zee_{S,\alpha}$. Likewise, we use $\zee_{i,j}$ as a shorthand for the function $\indi{\zee_i = j}$. That is, henceforth,
\ifnum\confversion=1
\begin{align*}
	&\tildeEx{\zee_{S,\alpha}} = \tildeEx{\indi{\zee_S = \alpha}} = \tildeEx{ \prod_{s\in S}
                             Z_{s,\alpha_s}}
                             \\
	\text{and } \quad & \tildeEx{\zee_{i,j}} = \tildeEx{\indi{\zee_i = j}} = \tildeEx{ Z_{i,j}}.
\end{align*}
\else
\begin{align*}
	\tildeEx{\zee_{S,\alpha}} ~=~ \tildeEx{\indi{\zee_S = \alpha}} ~=~ \tildeE\brackets[\Big]{\prod_{s\in S}
                      Z_{s,\alpha_s}
                                    }
\qquad \text{and} \qquad
	\tildeEx{\zee_{i,j}} ~=~ \tildeEx{\indi{\zee_i = j}} = \tildeEx{ Z_{i,j}}
\end{align*}
\fi

% Note that for any degree-$t$ pseudoexpectation operator $\tildeEx{\cdot}$ with $t\geq 2$,
% \[
% 	\sum_{j\in [q]} \tildeEx{\zee_{i,j}} = \sum_{j} \tildeEx{Z_{i,j}} = \tildeEx{\sum_j Z_{i,j}}= 1
% \qquad \text{and} \qquad
% 	\tildeEx{\zee_{i,j}} = \tildeEx{Z_{i,j}} = \tildeEx{Z_{i,j}^2} \geq 0
% \]
% Thus, the real values $\inbraces{\tildeEx{\zee_{i,j}}}_{j\in [q]}$ define a distribution over $[q]$
% , which we will sometimes call local distribution for $\zee_i$. 

% In fact, this argument can be extended to define local distributions for $\zee_S$ for $|S|\leq
% t/2$. Let $S \subseteq [m]$ be such that $|S|=k\leq t/2$,
Note that for any $S \subseteq [m]$ with $\abs*{S} = k \leq t/2$,
\ifnum\confversion=1
\begin{gather*}
	\sum_{ \alpha \in [q]^{k}} \tildeEx{\zee_{S,\alpha}} = 
% \sum_{ \alpha \in [q]^{k}} \tildeEx{ \prod_{s\in S} Z_{s,\alpha_s}} 
 \tildeEx{ \prod_{s\in S} \inparen{ \sum_{j\in [q]} Z_{s,j}} } = 1
\\
	\tildeEx{\zee_{S,\alpha}} = \tildeEx{ \prod_{s\in S} Z_{s,\alpha_s}} = \tildeEx{ \prod_{s\in
            S} Z^2_{s,\alpha_s}} \geq 0 \mper
\end{gather*}
\else
\[
	\sum_{ \alpha \in [q]^{k}} \tildeEx{\zee_{S,\alpha}} = 
% \sum_{ \alpha \in [q]^{k}} \tildeEx{ \prod_{s\in S} Z_{s,\alpha_s}} 
 \tildeE\brackets[\bigg]{ \prod_{s\in S} \parens[\bigg]{\sum_{j\in [q]} Z_{s,j} } } = 1
\qquad \text{and} \qquad
	\tildeEx{\zee_{S,\alpha}} = \tildeE\brackets[\bigg]{ \prod_{s\in S} Z_{s,\alpha_s}} = \tildeE\brackets[\bigg]{ \prod_{s\in
            S} Z^2_{s,\alpha_s}} \geq 0 \mper
\]
\fi
Thus, the values $\inbraces{\tildeEx{\zee_{S, \alpha}}}_{\alpha\in [q]^S}$ define a distribution
over $[q]^k$, referred to as the local  distribution for $\zee_S$.

% which we think of as the local distribution for $\zee_S$.
%
% Given a distribution $\calD$ over assignments in $[q]^m$, the local distribution induced by $\PExp^{(\calD)}[\cdot]$ on $\zee_S$ is precisely the marginal distribution induced by $\calD$ for the set $S$. In this view, degree-$t$ pseudoexpectations give us consistent marginal distributions over sets of size at most $t/2$ that may not correspond to any global distribution, and allow us to optimize over this set in time $m^{\calO(t)}$.
%
Let $\mu: [q]^m \rightarrow\R$ be a $k$-local function for $k\leq t/2$, depending on $M \subseteq
[m]$. Then,
%
\ifnum\confversion=1
\begin{align*}
	\tildeEx{\mu(\zee)} 
~=~& \tildeEx{\sum_{\alpha\in [q]^M} \inparen{\mu(\alpha) \cdot\prod_{i\in M} Z_{i,\alpha_i}}}\\
~=~& \sum_{\alpha\in [q]^M} \mu(\alpha) \cdot \tildeEx{\prod_{i\in M} Z_{i,\alpha_i}}\\
~=~& \sum_{\alpha\in [q]^M} \mu(\alpha) \cdot \tildeEx{\zee_{M,\alpha}}
\end{align*}
\else
\begin{align*}
	\tildeEx{\mu(\zee)} 
~=~ \tildeE\brackets[\bigg]{\sum_{\alpha\in [q]^M} \parens[\bigg]{\mu(\alpha) \cdot\prod_{i\in M} Z_{i,\alpha_i}}}
~=~ \sum_{\alpha\in [q]^M} \mu(\alpha) \cdot \tildeE\brackets[\Big]{\prod_{i\in M} Z_{i,\alpha_i}}
~=~ \sum_{\alpha\in [q]^M} \mu(\alpha) \cdot \tildeEx{\zee_{M,\alpha}}
\end{align*}
\fi
%
That is, $\tildeEx{\mu(\zee)}$ can be seen as the expected value of the function $\mu$ under the local distribution for $M$.

\begin{claim}
	Let $\tildeEx{\cdot}$ be a degree-$t$ pseudoexpectation. For $k \leq t/2$, let $\mu_1,\mu_2$
        be two $k$-local functions on $[q]^m$, depending on the same set of coordinates $M$, and
        $\mu_1(\alpha) \leq \mu_2(\alpha) ~~\forall \alpha \in [q]^M$. Then $\tildeEx{\mu_1(\zee)} \leq \tildeEx{\mu_2(\zee)}$.
%
 % Suppose that for any $\alpha\in [q]^M$, $\mu_1(\alpha) \leq \mu_2(\alpha)$. Then
 %        \[
 %        	\tildeEx{\mu_1(\zee)} \leq \tildeEx{\mu_2(\zee)}
 %        \]
\end{claim}

\begin{proof}
Let $\calD_M$ be the local distribution induced by $\tildeEx{\cdot}$ for $\zee_M$. Then
$\tildeEx{\mu_1(\zee)} = \Ex{\alpha \sim \calD_M}{\mu_1(\alpha)}$, and $\tildeEx{\mu_2(\zee)} =
\Ex{\alpha\sim \calD_M}{\mu_2(\alpha)}$, which implies $\tildeEx{\mu_1(\zee)} \leq \tildeEx{\mu_2(\zee)}$.
%
% Since $\mu_1(\alpha) \leq \mu_2(\alpha)$ for every $\alpha\in [q]^M$, 
% \[
% 	\Ex{\alpha \sim \calD_M}{\mu_1(\alpha)} \leq \Ex{\alpha\sim \calD_M}{\mu_2(\alpha)}
% \]
% and so,
% \[
% 	\tildeEx{\mu_1(\zee)} \leq \tildeEx{\mu_2(\zee)}
% \]
\end{proof}
%
The previous claim allows us to replace any local function inside $\tildeEx{\cdot}$ by another local function that dominates it. We will make extensive use of this fact.
%
%
\vspace{-5 pt}
%\tnote{Move covariance, conditioning stuff to appendix 1? It seems to disrupt the flow and we only need to cite it in section 6 for Lemma 6.1?}
\paragraph{Covariance for SoS solutions}
Given two sets $S,T \sub [m]$ with $|S|,|T|\leq k/4$, we can define the covariance between indicator random variables of $\zee_S$ and $\zee_T$ taking values $\alpha$ and $\beta$ respectively, according to the local distribution over $S \cup T$. This is formalized in the next definition.
\begin{definition}
Let $\tildeEx{\cdot}$ be a pseudodistribution operator of SoS-degree-$t$, and $S,T$ are two sets of
size at most $t/4$, and $\alpha\in [q]^S$, $\beta\in [q]^T$, we define the pseudo-covariance and
pseudo-variance,
%
\ifnum\confversion=1
\small
\begin{gather*}
\tildecov(\zee_{S,\alpha},\zee_{T,\beta}) 
= \tildeEx{ \zee_{S,\alpha} \cdot \zee_{T,\beta} } - \tildeEx{\zee_{S,\alpha}} \tildeEx{\zee_{T,\beta}} \\	
\tildeVar{\zee_{S,\alpha}} ~=~ \tildecov(\zee_{S,\alpha},\zee_{S,\alpha})
\end{gather*}
\normalsize
\else
\begin{align*}
\tildecov(\zee_{S,\alpha},\zee_{T,\beta}) 
~&=~ \tildeEx{ \zee_{S,\alpha} \cdot \zee_{T,\beta} } - \tildeEx{\zee_{S,\alpha}} \,\tildeEx{\zee_{T,\beta}}\\ 		
\tildeVar{\zee_{S,\alpha}} ~&=~ \tildecov(\zee_{S,\alpha},\zee_{S,\alpha})
\end{align*}
\fi
%
The above definition is extended to pseudo-covariance and pseudo-variance for pairs of sets $S,T$, 
as the sum of absolute value of pseudo-covariance for all pairs $\alpha,\beta$ :
%
\ifnum\confversion=1
\begin{gather*}
\tildecov(\zee_S,\zee_T) 
~=~ \sum_{\alpha\in [q]^S \atop \beta\in [q]^T} \abs*{ \tildecov(\zee_{S,\alpha},\zee_{T,\beta}) } \\
\tildeVar{\zee_S} ~=~ \sum_{\alpha\in [q]^S} \abs*{ \tildeVar{\zee_{S,\alpha} } }
\end{gather*}
\else
\begin{align*}
\tildecov(\zee_S,\zee_T) 
~&=~ \sum_{\alpha\in [q]^S, \beta\in [q]^T} \abs*{ \tildecov(\zee_{S,\alpha},\zee_{T,\beta}) }\\[3pt]
\tildeVar{\zee_S} ~&=~ \sum_{\alpha\in [q]^S} \abs*{ \tildeVar{\zee_{S,\alpha} } }
\end{align*}
\fi
%
\end{definition}

% These definitions can be extended to pseudocovariances and pseudo-variances for pairs of sets $S,T$ with $|S|,|T|\leq t/4$ as the sum of absolute value of pseudocovariance for all pairs $\alpha,\beta$.
% \begin{definition}
% Let $\tildeEx{\cdot}$ be a pseudodistribution operator of SoS-degree-$t$, and $S,T$ are two sets of size at most $t/4$, we define the pseudo-covariance between $\zee_S$ and $\zee_T$ as,
% 	\begin{align*}
% 		\tildecov(\zee_S,\zee_T) = \sum_{\alpha\in [q]^S,\beta\in [q]^T} \abs*{ \tildecov(\zee_{S,\alpha},\zee_{T,\beta}) }
% 	\end{align*}
% We also define the analogous pseudovariance as,
% 	\begin{align*}
% 		\tildeVar{\zee_S} = \sum_{\alpha\in [q]^S} \abs*{ \tildeVar{\zee_{S,\alpha} } }
% 	\end{align*}
% \end{definition}
%
We will need the fact that $\tildeVar{\zee_S}$ is bounded above by 1, since,
%
\ifnum\confversion=1
\begin{align*}
\tildeVar{\zee_S} 
&~=~ \sum_{\alpha} \abs*{\tildeVar{\zee_{S,\alpha}}} \\
&~=~ \sum_{\alpha}\inparen{
          \tildeEx{\zee_{S,\alpha}^2} - \tildeEx{\zee_{S,\alpha}}^2} \\
&~\leq~ \sum_{\alpha} \tildeEx{\zee_{S,\alpha}^2} \\
&~=~ \sum_{\alpha} \tildeEx{\zee_{S,\alpha}} 
~=~ 1
\end{align*}
\else
\[
\tildeVar{\zee_S} 
~=~ \sum_{\alpha} \abs*{\tildeVar{\zee_{S,\alpha}}} 
~=~ \sum_{\alpha}\inparen{
          \tildeEx{\zee_{S,\alpha}^2} - \tildeEx{\zee_{S,\alpha}}^2} 
~\leq~ \sum_{\alpha} \tildeEx{\zee_{S,\alpha}^2} 
~=~ \sum_{\alpha} \tildeEx{\zee_{S,\alpha}} 
~=~ 1
\]
\fi

% \begin{claim}\quad	$\tildeVar{\zee_S} \leq 1$.
% \end{claim}
% %
% \begin{proof}
% \begin{align*}
% 	\tildeVar{\zee_S} &= \sum_{\alpha} \abs*{\tildeVar{\zee_{S,\alpha}}} = \sum_{\alpha}\inparen{ \tildeEx{\zee_{S,\alpha}^2} - \tildeEx{\zee_{S,\alpha}}^2} \leq \sum_{\alpha} \tildeEx{\zee_{S,\alpha}^2} = \sum_{\alpha} \tildeEx{\zee_{S,\alpha}} = 1
% \end{align*}
% \end{proof}
%
\vspace{-5 pt}
\paragraph{Conditioning SoS solutions.}
%
We will also make use of conditioned pseudoexpectation operators, which may be defined in a way
similar to usual conditioning for true expectation operators, as long as the event we condition on
is local. 
%
The conditioned SoS solution is of a smaller degree, but continues to respect the constraints that original solution respects.

\begin{definition} Let $F \subseteq [q]^m$ be subset (to be thought of as an event) such that $\one_F:[q]^m \rightarrow \{0,1\}$ is a $k$-local function. Then for every $t>2k$, we can condition a pseudoexpectation operator of SoS-degree $t$ on $F$ to obtain a new conditioned pseudoexpectation operator $\condPE{\cdot}{F}$ of SoS-degree $t-2k$, as long as $\tildeEx{\one^2_F(\zee)}>0$. The conditioned SoS solution is given by
\[
	\condPE{ p(\zee)}{F(\zee) } \defeq \frac{\tildeEx{p(\zee) \cdot \one^2_{F}(\zee)}}{\tildeEx{\one^2_{F}(\zee)}}
\]
where $p$ is any polynomial of degree at most $t-2k$.
\end{definition}

We can also define pseudocovariances and pseudo-variances for the conditioned SoS solutions.
\begin{definition}
	Let $F\sub [q]^m$ be an event such that $\one_F$ is $k$-local, and let $\tildeEx{\cdot}$ be a pseudoexpectation operator of degree $t$, with $t>2k$. Let $S,T$ be two sets of size at most $\frac{t-2k}{2}$ each. Then the pseudocovariance between $\zee_{S,\alpha}$ and $\zee_{T,\beta}$ for the solution conditioned on event $F$ is defined as,
\ifnum\confversion=1
\begin{multline*}
\tildecov(\zee_{S,\alpha},\zee_{T,\beta} \vert F) = \\
\tildeEx{ \zee_{S,\alpha} \zee_{T,\beta} \vert F} - \tildeEx{\zee_{S,\alpha} \vert F} \tildeEx{\zee_{T,\beta} \vert F}
\end{multline*}
\else
\begin{align*}
\tildecov(\zee_{S,\alpha},\zee_{T,\beta} \vert F) 
~=~ \tildeEx{ \zee_{S,\alpha} \zee_{T,\beta} \vert F} - \tildeEx{\zee_{S,\alpha} \vert F} \tildeEx{\zee_{T,\beta} \vert F}
\end{align*}
\fi
\end{definition}

We also define the pseudocovariance between $\zee_{S,\alpha}$ and $\zee_{T,\beta}$ after
conditioning on a random assignment for some $\zee_V$ with $V\sub [m]$. 
%
Note that here the random assignment for $\zee_V$ is chosen according to the local distribution for
the set $V$.

\begin{definition}[Pseudocovariance for conditioned pseudoexpectation operators]
\ifnum\confversion=1
\begin{multline*}
\tildecov(\zee_{S,\alpha},\zee_{T,\beta} \vert \zee_V) 
= \\ \sum_{\gamma \in [q]^V}   \tildecov(\zee_{S,\alpha},\zee_{T,\beta} \vert \zee_V = \gamma) \cdot \tildeEx{\zee_{V,\gamma}}
	\end{multline*}
\else
\begin{align*}
\tildecov(\zee_{S,\alpha},\zee_{T,\beta} \vert \zee_V) 
~=~ \sum_{\gamma \in [q]^V}   \tildecov(\zee_{S,\alpha},\zee_{T,\beta} \vert \zee_V = \gamma) \cdot \tildeEx{\zee_{V,\gamma}}
\end{align*}
\fi
\end{definition}

And we likewise define $\tildeVar{\zee_{S,\alpha} \vert \zee_V}$, $\tildecov(\zee_S, \zee_T \vert \zee_V)$ and $\tildeVar{\zee_S \vert \zee_V}$.

\subsection{SoS relaxations for codes}
%
%For both Tanner codes and AEL codes, we will identify $[m]$ with $E$ so that the SoS solutions will be relaxations to the assignments to edges of a bipartite $(n,d,\lambda)$-expander.

%\paragraph{Pseudocodewords for Tanner Codes}
%
%Let $G(L,R,E)$ be the bipartite $(n,d,\lambda)$-expander on which the Tanner code is defined, and let $\calC_0\subseteq [q]^d$ be the inner code. The SoS variables will be $\zee = \{Z_{e,j}\}_{e\in E,j\in [q]}$. 
%
%\begin{definition}[Tanner Pseudocodewords]
%For $t\geq 2d$, we define a degree-$t$ Tanner pseuocodeword to be a degree-$t$ pseudoexpectation operator $\tildeEx{\cdot}$ on $\zee$ respecting the following constraints:
%%
%\ifnum\confversion=1
%\begin{align*}
%&\forall \li \in L, \quad \zee_{N_L(\li)} \in \calC_0 \\
%\text{and } \quad &\forall \ri \in R,\quad \zee_{N_R(\ri)} \in\calC_0
%\end{align*}
%\else
%\begin{align*}
%\forall \li \in L, \quad \zee_{N_L(\li)} \in \calC_0 
%\qquad \text{and} \qquad          
%\forall \ri \in R,\quad \zee_{N_R(\ri)} \in\calC_0
%\end{align*}
%\fi
%%
%Again, since these constraints are $d$-local, it is sufficient to enforce that certain degree-$d$ polynomials are zero (respected by pseudoexpectation) to enforce these constraints. 
%%
%In particular, each parity check in the parity check matrix of $\calC_0$ will correspond to a monomial of size at most $d$ that we can enforce to be equal to 1.
%\end{definition}
%
%We can also define a generalization of distance between two codewords to include pseudocodewords.
%%
%\begin{definition}[Distance from a pseudocodeword]
%%
%The distance between a pseudocodeword $\tildeEx{\cdot}$ of SoS-degree $t\geq 2d$ and a codeword $h$ of $\TanC$ is defined as
%\ifnum\confversion=1
%\begin{align*}
%\dis(\tildeEx{\cdot},h) 
%~\defeq~& \Ex{e\in E}{\tildeEx{\indi{\zee_e \neq h_e}}} \\
%~=~& \Ex{\li\in L}{\tildeEx{\dis(\zee_{N_L(\li)},  h_{N_L(\li)})}}
%\end{align*}
%\else
%\[
%\dis(\tildeEx{\cdot},h) 
%~\defeq~ \Ex{e\in E}{\tildeEx{\indi{\zee_e \neq h_e}}} 
%~=~ \Ex{\li\in L}{\tildeEx{\dis(\zee_{N_L(\li)},  h_{N_L(\li)})}}
%\]
%\fi
%\end{definition}

\paragraph{Pseudocodewords for AEL}

Let $G(L,R,E)$ be the bipartite $(n,d,\lambda)$-expander on which the AEL code is defined, and let $\cC = (\cx,\cz)$ be the inner code. The SoS variables will be $\zee = \{Z_{e,j}\}_{e\in E,j\in \F_q}$. 

The subsets of $E$ we consider will all be vertex neighborhoods from the left or right. To simplify notation, we use the convention that if $\li \in L$, then $\zee_{\li}$ denotes $\zee_{N(\li)}$, where $N(\li)$ is the set of all edges incident on the left vertex $\li$. Likewise, if $\ri \in R$, $\zee_{\ri}$ denotes $\zee_{N(\ri)}$, where $N(\ri)$ denotes the set of all edges incident on the right vertex $\ri$.

We also extend this shorthand to include subsets of $L$ and $R$ so that if $S \sub L$ ($R$ respectively), then $\zee_S$ denotes $\zee_{N(S)}$ where $N(S)$ is the set of all edges in $E$ incident on left (right respectively) vertices in $S$.

\begin{definition}[$X$-Pseudocodewords]
	For $t\geq 2d$, we define a degree-$t$ AEL pseuocodeword to be a degree-$t$ pseudoexpectation operator $\tildeEx{\cdot}$ on $\zee$ respecting the following constraints:
	\begin{align*}
		\forall \li \in L,\quad \zee_{\li} \in \cx
	\end{align*}
\end{definition}
%
We now define a generalized version of the notion of distance between a pseudocodeword $\tildeEx{\cdot}$, and a true codeword $h$.  

\begin{definition}[Distance from a pseudocodeword]
We define three types of distances between a pseudocodeword $\tildeEx{\cdot}$ of SoS-degree $t\geq 2d$ and a (unfolded) codeword $h \in \F_q^E$ are defined as
\begin{align*}
 	\distL{\tildeEx{\cdot}} ~&=~ \Ex{\li\sim L}{\tildeEx{\indi{ \zee_\li \neq h_{\li}}}}\\
\distLperp{\tildeEx{\cdot}} ~&=~ \Ex{\li \sim L}{\tildeEx{\indi{ \zee_\li \not\in h_{\li} + \cz^\perp }}}\\
 \distR{\tildeEx{\cdot}} ~&=~\Ex{r\sim R}{\tildeEx{\indi{ \zee_{r} \neq h_{r}}}}
 \end{align*}
 \end{definition}
 
Next, we define a non-convex property for a pseudocodeword that allows us to prove a distance property similar to \cref{lem:zfc_dist} for pseudocodewords.

\begin{definition}
	A pseudocodeword is $\eta$-good if,
	\[
		\Ex{\li,\ri}{ \tildeCov{ \zee_{\li}}{\zee_{\ri} } } \leq \eta
	\]
\end{definition}
%
\todo{Change names of functions in lemma 5.12 and 5.13 to something other than X and Y}
%
The following lemma captures the main property of $\eta$-good pseudocodoewords that we will be using. The proof of this lemma can be found in \cref{app:correlation_rounding} where it is restated as \cref{lem:using_eta_good}.
%
\begin{lemma}\label{lem:eta_good}
	Let $\{X_{\li}\}_{\li\in L}$ and $\{Y_{\ri}\}_{\ri\in R}$ be two collections of $d$-local functions on $[q]^E$ such that for every $\li\in L$, $X_{\li}(f)$ only depends on $f_{\li}$ and for every $\ri\in R$, $Y_{\ri}(f)$ only depends on $f_{\ri}$. Then, for an $\eta$-good pseudocodeword $\tildeEx{\cdot}$,
	\[
		\Ex{\li,\ri}{\tildeEx{X_{\li}(\zee) \cdot Y_{\ri}(\zee)}} ~\leq~ \Ex{\li,\ri}{\tildeEx{X_{\li}(\zee)} \cdot \tildeEx{Y_{\ri}(\zee)}} + \eta \left( \max_{\li} \norm{X_{\li}}_{\infty} \right) \left( \max_{\ri} \norm{Y_{\ri}}_{\infty}\right)
	\]
\end{lemma}

Next, we show that a variant of the expander mixing lemma can be adapted to work inside the SoS proof system by exploiting the non-negativity of sum-of-squares of low-degree polynomials. The proof for the next lemma is deferred to \cref{app:eml_sos}.

\begin{lemma}[EML for pseudoexpectations]\label{lem:eml_pseudoexpectation}
	Let $\{X_{\li}\}_{\li\in L}$ and $\{Y_{\ri}\}_{\ri\in R}$ be two collections of $d$-local functions on $[q]^E$ such that for every $\li\in L$, $X_{\li}(f)$ only depends on $f_\li$ and for every $\ri\in R$, $Y_{\ri}(f)$ only depends on $f_\ri$.
%
Then for a $\lambda$-spectral expander, we have
	\[
		\abs*{\Ex{\li\sim \ri}{\tildeEx{X_{\li}(\zee) \cdot Y_{\ri}(\zee) }} -
                  \Ex{\li,\ri}{\tildeEx{X_{\li}(\zee) \cdot Y_{\ri}(\zee)}}} \leq \lambda
                \sqrt{\Ex{\li}{\tildeEx{X_{\li}(\zee)^2}}} \cdot \sqrt{\Ex{\ri}
                  {\tildeEx{Y_{\ri}(\zee)^2}}} \mper
	\]
\end{lemma}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> regularity/abbrev.tex <==
% filled card suits
\DeclareSymbolFont{extraup}{U}{zavm}{m}{n}
\DeclareMathSymbol{\varheart}{\mathalpha}{extraup}{86}
\DeclareMathSymbol{\vardiamond}{\mathalpha}{extraup}{87}

\def\RR{\mathbb R}
\def\totw{\text{ otherwise }}
\def\tif{\text{ if }}
\def\wio{\backslash}
\def\tand{\quad\text{and}\quad}
\def\tor{\text{ or }}
\def\tst{\text{ s.t. }}
\def\matr#1{\mathsf{#1}}
\def\vecc#1{\boldsymbol{#1}}
\def\rand#1{\mathbf{#1}}
\def\rv#1{\rand #1}
\def\conj{\overline}
\def\SymG{\mathfrak S}
\def\Sep{\mathcal S}
\def\Lap{\mathcal L}
\def\Ray{\mathcal R}
\def\Adj{\mathcal A}
\def\Ker{\mathcal K}
\def\Wal{\mathcal W}
\def\One{\mathbb 1}
\def\one{\mathbf 1}
\def\Sp{\mathbb S}
\def\Ba{\mathbb B}
\def\Aa{\mathcal A}
\def\Pred{\mathcal P}
\def\Cc{\mathcal C}
\def\Xx{\mathcal X}
\def\Tt{\mathcal T}
\def\Ff{\mathcal F}
\def\Ee{\mathcal E}
\def\Di{\mathcal D}
\def\tensor{\otimes}
\def\ALG{\mathsf{ALG}}
\def\OPT{\mathsf{OPT}}
\def\SAT{\mathsf{SAT}}
\def\AVG{\mathsf{AVG}}
\def\SDP{\mathsf{SDP}}
\def\LP{\mathsf{LP}}
\def\vph{\varphi}
\def\ee{\varepsilon}
\def\pmu{\widetilde \mu}
\def\dif{\textrm{d}}
\def\Ins{\mathfrak I}
\def\assn{\sigma}
\def\tree{\mathcal T}
%% matrices
\def\Up{\matr U}
\def\Dee{\matr D}
\def\Aye{\matr A}
\def\Bee{\matr B}
\def\Why{\matr Y}
\def\Www{\matr W}
\def\Enn{\matr N}
\def\Ess{\matr S}
\def\Ide{\matr I}
\def\Pii{\matr P}
\def\Emm{\matr M}
\def\Jay{\matr J}
\def\Gee{\matr G}
%% functions
\def\eff{\vecc f}
\def\gee{\vecc g}
\def\eee{\vecc e}
\def\etch{\vecc h}
\def\pii{\vecc p}
\def\cee{\vecc c}
\def\wii{\vecc w}
%% faces
\def\aye{\mathfrak a}
\def\ess{\mathfrak s}
\def\tee{\mathfrak t}
\def\bee{\mathfrak b}
\def\teen{\widetilde{\tee}}
% operators
\DeclareMathOperator{\SwapT}{Swap}
\DeclareMathOperator{\Ent}{Ent}
\DeclareMathOperator{\hamw}{wt}
\DeclareMathOperator{\ddeg}{deg}
\DeclareMathOperator{\Det}{det}
\DeclareMathOperator{\sspan}{span}
\DeclareMathOperator{\Sym}{Sym}
\DeclareMathOperator{\Deg}{deg}
\DeclareMathOperator{\Herm}{\mathcal H}
\DeclareMathOperator{\Pos}{\mathcal P}
\DeclareMathOperator{\Dens}{\mathcal D}
\DeclareMathOperator{\OO}{\mathcal O}
\DeclareMathOperator{\OOs}{\widetilde{\mathcal O}}
\DeclareMathOperator{\Oms}{\widetilde{\Omega}}
\DeclareMathOperator{\oo}{o}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\Cay}{Cay}
\DeclareMathOperator{\colp}{cp}
\DeclareMathOperator{\plog}{polylog}
\DeclareMathOperator{\vol}{vol}
\DeclareMathOperator{\ddiag}{diag}
\DeclareMathOperator{\MI}{I}
\DeclareMathOperator{\Stab}{Stab}
\DeclareMathOperator{\NoSe}{NS}
\DeclareMathOperator{\dist}{d}
\DeclareMathOperator{\parikh}{\#}
\DeclareMathOperator{\ddiam}{diam}
\DeclareMathOperator{\Num}{N}
\DeclareMathOperator{\spec}{Spec}
\DeclareMathOperator{\Diff}{\Delta}
\DeclareMathOperator{\Rank}{rank}
\DeclareMathOperator{\PExp}{\widetilde \E}
% parens, braces, brackets, norms, absolute value, and inner products
\DeclarePairedDelimiter\set{\lbrace}{\rbrace}
\DeclarePairedDelimiter\parens{\lparen}{\rparen}
\DeclarePairedDelimiter\sqbr{[ }{]}
\DeclarePairedDelimiter\Abs{|}{|}


\DeclareMathOperator{\bias}{bias}
\DeclareMathOperator{\lift}{dsum}
\DeclareMathOperator{\dsum}{dsum}
\DeclareMathOperator{\dprod}{dprod}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%       Walk Operators
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%        Swap Walks
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Height Specific Rectangular Swap Walk
% Args:
%       #1='k' size of initial face s
%       #2='l' size of final face t
%       #3='j' number of new elements, i.e., |t\s|
%       #4='u' walk height
\newcommand{\hrswap}[4]{\Ess_{#1,#2}^{\left(#3,#4\right)}}

% Rectangular Swap Walk (Height Independent)
% Args:
%       #1='k' size of initial face s
%       #2='l' size of final face t
%       #3='j' number of new elements, i.e., |t\s|
\newcommand{\rswap}[3]{\Ess_{#1,#2}^{\left(#3\right)}}
% Rectangular full swap walk
% Args:
%       #1='k' size of initial face s
%       #2='l' size of final face t
\newcommand{\rfswap}[2]{\Ess_{#1, #2}}
% Height Specific Squared Swap Walk
% Args:
%       #1='k' size of initial face s
%       #2='j' number of new elements, i.e., |t\s|
%       #3='u' walk height
\newcommand{\hswap}[3]{\hrswap{#1}{#1}{#2}{#3}}

% Squared Swap Walk (Height Independent)
% Args:
%       #1='k' size of initial face s
%       #2='j' number of new elements, i.e., |t\s|
%\newcommand{\swap}[2]{\rswap{#1}{#1}{#2}}


\newcommand{\swap}[2]{\Ess_{#1,#2}}

% Walk Swap Operator
% Args:
%      #1='k_1'
%      #2='k_2'
\newcommand{\wswap}[3]{\Ess_{#1,#2}^{#3}}

\newcommand{\tswap}[3]{\Ess_{#1,#2,#3}}

\newcommand{\fswap}[3]{\mathfrak{S}_{#1,#2,#3}}

\newcommand{\sswap}[1]{\Ess_{#1,#1}^{\bigtriangleup}}

\newcommand{\CUT}{\textup{CUT}}

\newcommand{\SCUT}{\textup{CUT}_{\pm}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%        Normal Walks
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Rectangular Normal Walk
% Args:
%       #1='k' size of initial face
%       #2='l' size of final face
%       #3='u' walk height
\newcommand{\rnwalk}[3]{\Enn_{#1,#2}^{\left(#3\right)}}

% Normal Walk
% Args:
%       #1='k' size of initial face
%       #3='u' walk height
\newcommand{\nwalk}[2]{\Enn_{#1,#1}^{\left(#2\right)}}

\newcommand{\lict}[1]{$(1/2-#1)$-\text{close}}

\newcommand{\error}{\delta}

\newcommand{\sset}{\chi}

\newcommand{\AN}{\alpha_{\textup{\textbf{AN}}}}

\newcommand{\tuples}[1]{W(#1)}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Commands from
% pages.cs.wisc.edu/~dieter/Courses/2013s-CS880/Scribes/TEX/lecture.sty
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% circle a character
\usepackage{tikz}
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=1pt] (char) {#1};}}
% replacement product
\DeclareMathOperator{\replacement}{\circled{{\rm r}}}
% zig-zag product
\DeclareMathOperator{\zigzag}{\circled{{\rm z}}}
% derandomized squaring
\DeclareMathOperator{\dersquare}{\circled{{\rm s}}}

%!TEX root=main.tex


==> regularity/abstract.tex <==
The Gilbert--Varshamov bound non-constructively establishes the existence of binary codes of distance $1/2-\epsilon/2$ and rate $\Omega(\epsilon^2)$. 
In a breakthrough result, Ta-Shma [STOC 2017] constructed the first \emph{explicit} family of nearly optimal binary codes with distance $1/2-\epsilon/2$ and rate $\Omega(\epsilon^{2+\alpha})$, where $\alpha \to 0$ as $\epsilon \to 0$. 
%
Moreover, the codes in Ta-Shma's construction are $\eps$-balanced, where the distance between distinct codewords is not only bounded from below by $1/2-\epsilon/2$, but also from above by $1/2+\epsilon/2$.

\medskip
%
Polynomial time decoding algorithms for (a slight modification of) Ta-Shma's codes appeared in [FOCS 2020], and were based on the Sum-of-Squares (SoS) semidefinite programming hierarchy. The running times for these algorithms were of the form $N^{O_{\alpha}(1)}$ for unique decoding, and $N^{O_{\epsilon,\alpha}(1)}$ for the setting of ``gentle list decoding", with large exponents of $N$ even when $\alpha$ is a fixed constant. 
%
We derive new algorithms for both these tasks, running in time $\tilde{O}_{\eps}(N)$. Our algorithms also apply to the general setting of decoding direct-sum codes.

\medskip
%
Our algorithms follow from new structural and algorithmic results for collections of $k$-tuples (ordered hypergraphs) possesing a ``structured expansion" property, which we call \emph{splittability}. 
%
This property was previously identified and used in the analysis of SoS-based decoding and constraint satisfaction algorithms, and is also known to be satisfied by Ta-Shma's code construction.
%
We obtain a new weak regularity decompomposition for (possibly sparse) splittable collections $W \subseteq [n]^k$, similar to the regularity decomposition for dense structures by Frieze and Kannan [FOCS 1996].
%
These decompositions are also computable in near-linear time $\tilde{O}(\abs{W})$, and form a key component of our algorithmic results.

% and it is also known that the rate cannot be
% larger than $O(\epsilon^2 \log(1/\epsilon))$. 

% For a code $\Cc_{\epsilon,\alpha,N} \subseteq \mathbb{F}_2^N$ in Ta-Shma's construction, This property, known as $\epsilon$-balanced, is used in the study of pseudorandomness.

% where the Sum-of-Squares (SOS) semi-definite
% hierarchy was employed. While SOS is a powerful algorithmic tool to
% investigate polynomial time computation, it may not result in the
% fastest polynomial running times and the decoders in [FOCS 2020] were
% no exception. They either run in $N^{O_{\epsilon,\alpha}(1)}$ time or,
% at best, $N^{O_{\alpha}(1)}$ when $\alpha$ is a constant (in both
% cases very far from even $N^2$). The question of whether much faster
% polynomial time decoding algorithms existed was left open.

% Here, we show that much faster decoding algorithms indeed exist.  More
% precisely, we show that (essentially) Ta-Shma's codes can be decoded
% in near linear time in the block length $N$, \ie can be decoded in
% $\widetilde{O}_{\epsilon}(N)$ time. Our near linear time decoding
% algorithms are obtained using a new weak regularity decomposition, in
% the style of the celebrated regularity decomposition for dense
% structures by Frieze and Kannan [FOCS 1996], which we develop here for
% (possibly) sparse \emph{splittable} collection of tuples $W
% \subseteq [n]^k$. This splittable property is a notion of expansion
% for tuples and it is known to hold for a slight modification of tuples
% appearing in Ta-Shma's code construction.


%!TEX root=main.tex

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> regularity/code_param.tex <==

\fnote{With these simple changes in Ta-Shma's parameter of round I, we should be able to handle
       an error as bad as $2^{-2^{k}}$ from efficient weak regularity with unbalanced splits.}

We will need minor adjustments to code parameter used in~\cite{JQST20}
which are similar to Ta-Shma's original analysis~\cite{Ta-Shma17}.

\fnote{The text below is essentially the FOCS text with the required
  modifications.}

\subsection{Round I: Initial Analysis}\label{sec:round_1}

We are given the dimension $D$ of the desired code and $\epsilon \in
(0,1/2)$.  We set a parameter $\alpha \le 1/128$ such that (for
convenience) $1/\alpha$ is a power of $2$ and
\begin{equation}\label{eq:alpha_epsilon}
\frac{\alpha^{4/\alpha^2 + 2}}{4 \log_2(1/\alpha)} \ge \frac{1}{\log_2(1/\epsilon)}.
\end{equation}
We can assume that $\alpha \le 1/128$ satisfy~\cref{eq:alpha_epsilon}
since otherwise $\epsilon$ is a constant and we can use the list
decodable codes from \fnote{Perhaps, Guruswami--Indyk or other
  construction.}. The use of~\cref{eq:alpha_epsilon} will be clear
shortly. It becomes a necessity from round III onward. For rounds I
and II, the parameter $\alpha$ will be a constant, but it will be
useful to establish the analysis in more generality now so that
subsequent rounds can reuse it.

\noindent \textbf{The inner graph $H$.} \enspace The choice of $H$ is
similar to Ta-Shma's choice. More precisely, we set $s=1/\alpha$ and
$d_2 = s^{s^{4s^2}}$ (Ta-Shma took $d_2 = s^{4s}$).
We obtain a Cayley graph $H
= \textup{Cay}(\mathbb{F}_2^{4s\log_2(d_2)}, A)$ such that $H$ is an
$(n_2=d_2^{4s}, d_2, \lambda_2)$ graph where
$\lambda_2 = b_2/\sqrt{d_2}$ and $b_2 = 4 s \log_2(d_2)$.
%$b_2 = 4 \sqrt{2} \log_2(d_2) s$.
(The set of generators, $A$, comes from a small bias code derived from
a construction of Alon et al.~\cite{AGHP92}, but we will rely on
Ta-Shma's analysis embodied in~\cref{lemma:aghp} and not discuss it
further.)

\noindent \textbf{The base code $\Cc_0$.} \enspace
Set $\epsilon_0 = 1/d_2^2 = \lambda_2^4/b_2^4 \le \lambda_2^4/3$ (this
choice differs from Ta-Shma's and it appears because we are
essentially working with $H^2$ rather than $H$). We will choose a base
code $\Cc_0$ such that the desired code will be obtained as a direct
sum lifting of $\Cc_0$, and because this lifting preserves the
dimension, the dimension of $\Cc_0$ should be $D$. We choose $\Cc_0$
to be an $\epsilon_0$-balanced code with dimension $D$ and block
length $n=O_{\epsilon_0}(D)$.  For instance, we take $\Cc_0$ to be any
near linear time (in the parameter $n$) decodable
$\epsilon_0$-balanced code of rate
$\Omega_{\epsilon_0}(1)$. \fnote{Gurswami--Indyk may have such a
code~\cite{GI02}.}

%Similarly to Ta-Shma, we can construct words with block length $2n$
%(if needed) by duplicating each codeword.

\noindent \textbf{The outer graph $G$.} \enspace
Set $d_1 = d_2^4$ so that $n_2 = d_1^s$ as required by the
$s$-wide replacement product. We apply Ta-Shma's explicit Ramanujan
graph~\cref{lemma:explicit_ramanujan} with parameters $n$, $d_1$ and
$\theta$ to obtain an $(n',d_1,\lambda_1)$ Ramanujan graph $G$ with
$\lambda_1 \le 2\sqrt{2}/\sqrt{d_1}$ and $n' \in [(1-\theta)n,n]$ or $n'\in [(1-\theta)2n,2n]$. Here, $\theta$ is an error parameter that we set as $\theta = \lambda_2^4/6$ (this choice of $\theta$ differs from
Ta-Shma). Because we can construct words with block length $2n$
(if needed) by duplicating each codeword, we may assume w.l.o.g. that $n'$ is close to $n$ and
$(n-n') \le \theta n \le 2 \theta n'$. See \cref{app:explicit_structures} for a more formal description of this graph.

Note that
$\lambda_1 \le \lambda_2^4/6$ since $\lambda_1 \le 3/\sqrt{d_1} =
3/d_2^2 = 3 \cdot \lambda_2^4/b_2^4 \le \lambda_2^4/6$. Hence,
$\epsilon_0 + 2\theta + 2\lambda_1 \le \lambda_2^4$.

\noindent \textbf{The walk length.} \enspace
Set the walk length $t-1$ to be the smallest integer such that
$$
(\lambda_2^2)^{(1-5\alpha)(1-\alpha)(t-1)} \le \epsilon.
$$
This will imply using Ta-Shma's analysis that the bias of the final code is at most $\epsilon$ as shown later.

\begin{center}
\fbox{\begin{minipage}{30em}

$s=1/\alpha, \text{ such that } \frac{\alpha^{4/\alpha^2 + 2}}{\log_2(1/\alpha)} \ge \frac{1}{\log_2(1/\epsilon)}$
\vskip 0.3cm
$H: (n_2,d_2,\lambda_2),\quad n_2=d_1^s,\quad d_2=s^{s^{4s^2}},\quad \lambda_2=\frac{b_2}{\sqrt{d_2}},\quad b_2 = 4s\log d_2$
\vskip 0.3cm
$G: (n',d_1,\lambda_1),\quad n' \approx n = O(D/\epsilon_0^c),\quad d_1=d_2^4,\quad \lambda_1\leq \frac{2\sqrt{2}}{d_1}$
\vskip 0.3cm
$t: \text{ smallest integer such that } (\lambda_2^2)^{(1-5\alpha)(1-\alpha)(t-1)} \leq \epsilon$

\end{minipage}}
\end{center}

\begin{claim}\label{claim:t_lower_bound}
  We have $t-1 \ge s/\alpha = s^2$.
\end{claim}

\begin{proof}
  Using $d_2 = s^{s^{4s^2}}$ and~\cref{eq:alpha_epsilon}, we have
  \begin{align*}
  \left(\frac{1}{\lambda_2^2}\right)^{(1-5\alpha)(1-\alpha)s/\alpha} & \le \left(\frac{1}{\lambda_2^2}\right)^{s/\alpha} = \left(\frac{d_2}{b_2^2}\right)^{s/\alpha} \le \left(d_2\right)^{s/\alpha} = s^{s^{4s^2+1}/\alpha}\\
                                                              & = 2^{s^{4s^2+1} \log_2(s)/\alpha} = 2^{4 \log_2(1/\alpha)/\alpha^{4/\alpha^2 +2}} \le  2^{\log_2(1/\epsilon)} = \frac{1}{\epsilon}.
  \end{align*}
  Hence, $\epsilon \le (\lambda_2^2)^{(1-5\alpha)(1-\alpha)s/\alpha}$ and thus
  $t-1$ must be at least $s/\alpha$.
\end{proof}

\begin{remark}\label{remark:choice_of_t}
 By our choice of $t$, we have $(\lambda_2^2)^{(1-5\alpha)(1-\alpha)(t-2)} \ge \epsilon$.
 Since $1/(t-1) \le \alpha$, we get $(\lambda_2^2)^{(1-5\alpha)(1-\alpha)^2 (t-1)} \ge \epsilon$.
\end{remark}

\noindent \textbf{Final Bias.} We denote by $\Cc_{\ell}$ the final code obtained
by $t$ steps of the $s$-wide replacement product. The bias of
$\Cc_{\ell}$ is given by~\cref{cor:tweaked_ta-shma_spectral_analysis}
(which in turn is a simple corollary of
Ta-Shma's~\cref{fact:ta-shma_main}) as shown next.
\begin{corollary}
  The code $\Cc_{\ell}$ is $\epsilon$-balanced.
\end{corollary}

\begin{proof}
  Using~\cref{cor:tweaked_ta-shma_spectral_analysis}, we have that the final bias  
  \begin{align*}
    b \coloneqq \left(\sigma_2(H^2)^{s-1} + (s-1) \cdot \sigma_2(H^2)^{s-2} + (s-1)^2 \cdot \sigma_2(H^2)^{s-4}\right)^{\lfloor (t-1)/s \rfloor}
  \end{align*}
  is bounded by
  \begin{align*}
    b &\le (3(s-1)^2\sigma_2(H^2)^{s-4})^{((t-1)/s)-1} && (\text{Using } \sigma_2(H^2)\leq 1/3s^2) \\
      &\le ((\sigma_2(H^2)^{s-5})^{(t-1-s)/s} \\
      &= \sigma_2(H^2)^{(1-5/s)(1-s/(t-1))(t-1)}\\
      &\le \sigma_2(H^2)^{(1-5\alpha)(1-\alpha)(t-1)}\\
      &= \left(\lambda_2^2\right)^{(1-5\alpha)(1-\alpha)(t-1)} \le \epsilon,                                                                                                                          
  \end{align*}
  where the last inequality follows from $s = 1/\alpha$ and $t-1 \ge s/\alpha$, the latter from~\cref{claim:t_lower_bound}.
\end{proof}

\noindent \textbf{Rate.}
The proof of the rate follows a similar structure of Ta-Shma's
original argument except that we take $s$ to be a constant independent
of $\epsilon$ so that $\epsilon_0$, $\lambda_1$, and $\lambda_2$ are also
constants independent of $\epsilon$. Note that we previously said $\alpha = 1/s$ needs to satisfy \autoref{eq:alpha_epsilon}, but that implies only an upper bound for $s$, and smaller (even constant) values for $s$ are still permissible.
\begin{claim}\label{claim:rate_round_i}
  $\Cc_{\ell}$ has rate $\Omega(\epsilon^{2+ 26 \cdot \alpha})$ provided $\epsilon_0 > 0$ is constant.
\end{claim}

\begin{proof}
  The support size is the number of walks of length $t$ on the
  $s$-wide replacement product of $G$ and $H$ (each step of the walk has $d_2^2$ options),
  which is
  \begin{align*}
    |V(G)| |V(H)| d_2^{2(t-1)} = n' \cdot d_1^s \cdot d_2^{2(t-1)} &= n' \cdot  d_2^{2(t-1)+4s} \le n \cdot  d_2^{2(t-1)+4s}\\
                                                      &= \Theta_{\epsilon_0}\left(D \cdot d_2^{2(t-1)+4s}\right)\\
                                                      &= \Theta\left(D \cdot (d_2^2)^{t-1+2s}\right)\\
                                                      &= O\left(D \cdot (d_2^2)^{(1+2\alpha)(t-1)}\right),                                                      
  \end{align*}
  where the penultimate equality follows from the assumption that $\epsilon_0$ is a constant.

  Note that $d_2^{\alpha} = d_2^{1/s} = s^{s^{4s^2-1}} \ge b_2$ since
  % $b_2 = 4\sqrt{2} \log_2(d_2) s = 16\sqrt{2} s^2 \le s^4$
  $b_2 = 4 s \log_2(d_2) = 4 s^{4s^2}$
  (recall that $s=1/\alpha \ge 128$). Thus,
  $$
  d_2^{1-2\alpha} = \frac{d_2}{d_2^{2\alpha}} \le \frac{d_2}{b_2^2} = \frac{1}{\sigma_2(H^2)}.
  $$
  We obtain
  \begin{align*}
  (d_2^2)^{(t-1)} &\le \left(\frac{1}{\sigma_2(H^2)}\right)^{\frac{2(t-1)}{1-2\alpha}} \\
  &\le \left(\frac{1}{\epsilon}\right)^{\frac{2}{(1-2\alpha)(1-5\alpha)(1-\alpha)^2}} && \text{(Using~\cref{remark:choice_of_t})}\\
  &\le \left(\frac{1}{\epsilon}\right)^{2(1+10\alpha)},
  \end{align*}
  which implies a block length of
  $$
  O\left(D \cdot (d_2^2)^{(1+2\alpha)(t-1)}\right) = O\left(D \left(\frac{1}{\epsilon}\right)^{2(1+10\alpha)(1+2\alpha)}\right) = O\left(D \left(\frac{1}{\epsilon}\right)^{2(1+13\alpha)}\right).
  $$
\end{proof}


\begin{lemma}[Codes Near the GV bound I]\label{lemma:codes_near_gv_i}
  For every constant $\beta > 0$, there exists a sufficiently large constant $s$ in the above
  analysis so that for any dimension value $D \in \mathbb{N}^+$ (sufficiently large) and $\epsilon > 0$
  (sufficiently small) the final code $\Cc_{N,\epsilon,\beta}$, where $N$ is the block length,
  satisfies
  \begin{itemize}
    \item $\Cc_{N,\epsilon,\beta}$ is $\epsilon$-balanced, 
    \item $\Cc_{N,\epsilon,\beta}$ has rate $\Omega(\epsilon^{2+\beta})$, and
    \item $\Cc_{N,\epsilon,\beta}$ is a linear code of dimension $D$.
  \end{itemize}
\end{lemma}


%% \begin{remark}
%%   As a consequence of code cascading, the final attainable walk lengths have the form $s^{\ell}-1$
%%   where $\ell$ is a positive integer. Given $\beta > 0$, we have infinitely many values of $\epsilon$
%%   attainable by such walk lengths which gives infinitely many codes $\Cc_{N,\epsilon,\beta}$. This means
%%   that although the bias $\epsilon$ cannot be arbitrary, we have an infinite sequence of values of $\epsilon$
%%   for which the rates of the codes $\Cc_{N,\epsilon,\beta}$ are near the GV bound. In~\cref{sec:careful_analysis_continum_for_beta}, we show how to bypass this artificial limitation. These codes are used in the proof of~\cref{theo:main_1}.
%% \end{remark}

%% We can view the above analysis as defining a function $\Gamma$ that
%% receives
%% \begin{itemize}
%%   \item the dimension $D \in \mathbb{N}^+$,
%%   \item the final bias $\epsilon > 0$,
%%   \item the approximating error $\alpha \in (0,1/128]$ with $s\coloneqq1/\alpha$ being a power of two, and
%%   \item a multiplying factor $Q \in \mathbb{N}^+$ such that $d_2 = s^{4s^2 \cdot Q}$ (in the above $Q$ was $1$).
%% \end{itemize}
%% and outputs a tuple of parameters $(t,\epsilon_0, \theta,d_1,\lambda_1,
%% n')$, graphs $G$ and $H$ (as above) where, in particular, the number
%% of steps $t \in \mathbb{N}^+$ is such that the final code $\Cc_{\ell}$
%% has bias at most $\epsilon$ and rate $\Omega(\epsilon^{2+
%% 26 \cdot \alpha})$.

%% In future rounds, $\Gamma$ may be called with $Q=s$ instead of $Q=1$. This will cause $d_2$ to increase from $s^{4s^2}$ to $s^{4s^2\cdot Q}$, and so in the proof of \autoref{claim:t_lower_bound}, $2^{4\log_2(1/\alpha) / \alpha^4}$ will be replaced by $2^{4\log_2(1/\alpha) / \alpha^5}$. This explains why \cref{eq:alpha_epsilon} has a stricter requirement than needed in the $Q=1$ case above.

%% \subsection{Round II: A More Careful Analysis}\label{sec:careful_analysis_continum_for_beta}

%% We are given the dimension of the code $D$ and $\epsilon \in (0,1/2)$.
%% As before, we set a parameter $\alpha \le 1/128$ such that (for convenience)
%% $1/\alpha$ is a power of $2$. Set $s = 1/\alpha$ and $Q = s$.

%% Apply $\Gamma$ to $(D,\epsilon,\alpha,Q)$ to obtain all parameters except $t$. Choose $t$ to be the smallest integer satisfying
%% $$
%% (\lambda_2^2)^{(1-5\alpha)(1-2\alpha)(1-\alpha)(t-1)} \le \epsilon,
%% $$
%% where observe that an extra $(1-2\alpha)$ factor appears in the exponent. This change in $t$ will worsen the rate but by losing a factor of $\frac{1}{1-2\alpha}$ in the exponent, we can lower bound the rate. That is, $(d_2^2)^{-(t-1)} = \Omega(\eps^{\frac{2+26\cdot \alpha}{1-2\alpha}})$. 

%% Set $\ell \in \mathbb{N}^+$ to be the smallest value such that
%% $s^{\ell} \ge t$ (here we are implicitly assuming that $t >
%% s$). If $s^{\ell} = t$, we are done since we can use all the
%% parameters returned by $\Gamma$ for the construction of
%% $\Cc_{\ell}$. Now assume $s^{\ell} > t$ and let $\zeta =
%% t/s^{\ell-1}$. Note that $\zeta \in (1,s)$. Choose $P$ to be the
%% integer in the interval $[Q,s\cdot Q]$ such that
%% $$
%% 0 \le \frac{P}{Q} - \zeta \le \frac{1}{Q}.
%% $$

%% Because $s^\ell > t$, and only powers of $s$ may be chosen for walk length, we might overshoot in walk length by a multiplicative factor of $s$. This will cause a corresponding decay in rate computation that we cannot afford. To overcome this, in the last level of the cascade between codes $\Cc_{\ell-1}$ and
%% $\Cc_{\ell}$, perform the direct sum over walks of length $(P-1)$ instead
%% of length $(s-1)$. The new total number of vertices is $t' =
%% P s^{\ell-1}$. Note that $P$ can be as large as $s^2$, so our
%% splittability guarantee of $W(P)$ (the walk collection from the lift
%% between $\Cc_{\ell-1}$ and $\Cc_{\ell}$) has to be strong enough to
%% accommodate this larger arity and not only arity $s$.

%% \begin{claim}\label{claim:approx_walk_length}
%%   We have $t-1 \le \frac{t'-1}{Q} \le (1+2\alpha) (t-1)$.
%% \end{claim}

%% \begin{proof}
%%  By construction, we have the sequence of implications
%%  \begin{align*}
%%     & 0 \le \frac{P}{Q}s^{\ell-1} - \zeta s^{\ell-1} \le \frac{s^{\ell-1}}{Q} \\
%%     \implies & 0 \le \frac{t'}{Q} - t \le \frac{s^{\ell-1}}{Q} \le \frac{t}{Q} \\ 
%%     \implies & t - \frac{1}{Q} \le \frac{t'-1}{Q} \le (t-1)\left(1+\frac{1}{Q} \right)+1,
%%  \end{align*}
%%  from which we obtain
%%  	$$t-1 \le t - \frac{1}{Q} \le \frac{t'-1}{Q}$$
%%  and
%%  	$$\frac{t'-1}{Q} \le (t-1) \left(1+\frac{1}{Q}\right) +1 = (1+\alpha) (t-1) + 1 < (1+2\alpha)(t-1),$$
%%  the latter using $Q = s = 1/\alpha$.
%% \end{proof}
 
%% We apply $\Gamma$ again but this time to $(D,\epsilon,\alpha,1)$ to
%% obtain new parameters $(t'', \epsilon_0'$, $\theta'$, $d_1'$,
%% $\lambda_1'$, $n'')$, and graphs $G'$ and $H'$.

%% \begin{claim}
%%   The code $\Cc_{\ell}'$ obtained by $t'$ walk steps on the
%%   $s$-wide replacement product of $G'$ and $H'$ from the second
%%   application of $\Gamma$ has bias at most $\epsilon$ and rate
%%   $\Omega(\epsilon^{2+40\alpha})$.
%% \end{claim}

%% \begin{proof}
%%   Let $d_2 = s^{4s^2 \cdot Q}$, $b_2 = 4 s \log_2(d_2)$ and $\lambda_2 = b_2/\sqrt{d_2}$ be
%%   the parameters of the first invocation of $\Gamma$. Recall that $t$ was chosen to
%%   be the smallest integer satisfying
%%   $$
%%   (\lambda_2^2)^{(1-5\alpha)^2(1-\alpha)(t-1)} \le \epsilon.
%%   $$
%%   Let $d_2' = s^{4s^2}$, $b_2' = 4 s \log_2(d_2')$ and $\lambda_2' = b_2'/\sqrt{d_2'}$
%%   be the parameters of the second invocation of $\Gamma$. Observe that
%%   \begin{align*}
%%   (\lambda_2')^{Q} &= \frac{(b_2')^Q}{\sqrt{(d_2')^Q}} = \frac{(b_2'^Q)}{\sqrt{d_2}} = \frac{(16 s^3 \log_2(s))^Q}{s^{2s^2 \cdot Q}} \\
%%   &\le \frac{s^{4Q}}{s^{2s^2\cdot Q}} = \frac{1}{s^{2s^2\cdot Q(1 - \frac{2}{s^2})}} = \left( \frac{1}{s^{2s^2\cdot Q}}\right)^{1-2\alpha} \leq \left( \frac{b_2}{\sqrt{d_2}}\right)^{1-2\alpha} = \lambda_2^{1-2\alpha}.
%%   \end{align*}
%%   Then the bias of $\Cc'_{\ell}$ is at most
%%   \begin{align*}
%%   (((\lambda_2')^Q)^2)^{(1-5\alpha)(1-\alpha)(t'-1)/Q} &\le (\lambda_2^2)^{(1-5\alpha)(1-2\alpha) (1-\alpha)(t'-1)/Q}\\
%%                                             &\le (\lambda_2^2)^{(1-5\alpha)(1-2\alpha) (1-\alpha)(t-1)} \le \epsilon.
%%   \end{align*}
%%   For the rate computation of $\Cc'_{\ell}$, we will lower bound the term $((d'_2)^2)^{-(t'-1)}$. Since $d_2 = (d_2')^{Q}$, $(d_2^2)^{-(t-1)} = \Omega(\eps^{\frac{2+26\cdot \alpha}{1-2\alpha}})$ and $\frac{t'-1}{Q} \le (1+2\alpha)(t-1)$
%%   (the latter by~\cref{claim:approx_walk_length}), the rate of $\Cc_{\ell}'$ is
%%   $$
%%   \Omega(((d'_2)^2)^{-(t'-1)}) = \Omega((d_2^2)^{-(t'-1)/Q}) = \Omega((d_2^2)^{-(1+2\alpha)(t-1)}) = \Omega((\epsilon^{2+ 26 \cdot \alpha})^{\frac{1+2\alpha}{1-2\alpha}}) = \Omega(\epsilon^{2+ 40 \cdot \alpha}).
%%   $$
%% \end{proof}


==> regularity/decoding.tex <==
\snote{I am not sure in how much detail we wish to recall the approach we used in previous papers, specifically that we look at the decoding task as a CSP. The first paragraph can be extended to accommodate that. For now, the main parts start from the second paragraph.}

Let $W(k) \subseteq W(1)^k$ be the set of $k$-tuples corresponding to the direct sum lifting we wish to decode, so that $W(k)$ lifts the code $\mathcal{C}_0$ to $\mathcal{C}$. Given a corrupted bit string of size $|W(k)|$, the (unique) decoding task is to find the codeword nearest to it. When the code is a direct sum lifting of some base code $\mathcal{C}_0$, we can instead find the base codeword in $\mathcal{C}_0$ corresponding to the nearest codeword in $\mathcal{C}$.

The constraints can then be categorized into two depending on the RHS being 0 or 1. Let $W_1(k)$ be the set of 1-constraints, which is dense in $W(k)$, and so $W_0(k) = W(k)-W_1(k)$ is the set of 0-constraints. Let a particular assignment be respresented by $S_0$, where $S_0$ is the set of variables assigned value 0, and let $S_1 = W(1)-S_0$. Define $\chi_{S_0} : W(1)\rightarrow \{-1,1\}$,

\begin{align*}
\chi_{S_0}(i) = (-1)^{\mathbb{1}_{i\in S_0}}
\end{align*}

Given a function $g\in \mathbb{R}^{W(1)^k}$, define $f_{0,S_0}$ and $f_{1,S_0}$ as,

%\begin{align*}
%	f_{0,S_0}(g) = \sum_{i \text{ binary string of length } k \text{ and weight even}} \ip{g}{\mathbb{1}_{S_{i_1}} \otimes \mathbb{1}_{S_{i_2}} \otimes \cdots \otimes \mathbb{1}_{S_{i_k}}} \\
%	f_{1,S_0}(g) = \sum_{i \text{ binary string of length } k \text{ and weight odd}} \ip{g}{\mathbb{1}_{S_{i_1}} \otimes \mathbb{1}_{S_{i_2}} \otimes \cdots \otimes \mathbb{1}_{S_{i_k}}}
%\end{align*}

\begin{align*}
	f_{S_0}(g) = \ip{g}{\chi_{S_0} \otimes \chi_{S_0} \otimes \cdots \otimes \chi_{S_0}}
\end{align*}

Then the number of 1-constraints satisfied by $S_0$ can be given by $\frac{|W_1(k)|+f_{S_0}(-\mathbb{1}_{W_1(k)})}{2}$, and the number of 0-constraints can be given by $\frac{|W_0(k)|+f_{S_0}(\mathbb{1}_{W_0(k)})}{2}$. The CSP can then be written as,

\begin{align*}
\frac{|W(k)|}{2}+\max_{S_0\subseteq W(1)} f_{S_0}(\mathbb{1}_{W_0(k)})+f_{S_0}(-\mathbb{1}_{W_1(k)})\\
=\frac{|W(k)|}{2}+\max_{S_0\subseteq W(1)} f_{S_0}(\mathbb{1}_{W_0(k)})-f_{S_0}(\mathbb{1}_{W_1(k)})
\end{align*}

%\begin{align*}
%	f_{1,S_0}(\mathbb{1}_{W'}) = & \ip{\mathbb{1}_{W'}}{\mathbb{1}_{S_0}\otimes \mathbb{1}_{S_0} \otimes \cdots \otimes \mathbb{1}_{S_0}\otimes \mathbb{1}_{S_1}} \\
%	+ & \ip{\mathbb{1}_{W'}}{\mathbb{1}_{S_0}\otimes \mathbb{1}_{S_0} \otimes \cdots \otimes \mathbb{1}_{S_1}\otimes \mathbb{1}_{S_0}}\\
%	& \vdots \\
%	+ & \ip{\mathbb{1}_{W'}}{\mathbb{1}_{S_1}\otimes \mathbb{1}_{S_1} \otimes \cdots \otimes \mathbb{1}_{S_1}\otimes \mathbb{1}_{S_1}}
%\end{align*}

Applying Lemma \ref{lemma:dense_model_lemma} with $W(k)$, $W' = W_1(k)$, $\epsilon = \eta/2$, we get $g_0$ supported on $O(1/\eta^2)$ functions from $\textup{CUT}^{\otimes k}$ such that,

\begin{align*}
|f_{S_0}(\mathbb{1}_{W_0(k)})-f_{S_0}(g_0)|\leq \eta/2 \cdot |W(k)|
\end{align*}

Likewise, we get another function $g_1$ supported on $O(1/\eta^2)$ functions from $\textup{CUT}^{\otimes k}$ such that,

\begin{align*}
|f_{S_0}(\mathbb{1}_{W_1(k)})-f_{S_0}(g_1)|\leq \eta/2 \cdot |W(k)|
\end{align*}

Instead of optimizing (over $S_0$) for $f_{S_0}(\mathbb{1}_{W_0(k)})-f_{S_0}(\mathbb{1}_{W_1(k)})$, we will now use the approximation $f_{S_0}(g_0)-f_{S_0}(g_1)$, with the advantage that we know $g_0$ and $g_1$ are low rank functions. In the process, we incur an error of at most $\eta \cdot |W(k)|$.

\begin{lemma}\label{lemma:obtain_fractions}
Given functions $g_0, g_1 \in \mathbb{R}^{W(1)^k}$ supported on $O(1/\eta^2)$ cut functions, we can find $\max_{S_0\subseteq W(1)} f_{S_0}(g_0)-f_{S_0}(g_1)$ in $O_{\eta,\gamma}(|W(1)|)$ time upto an error of $\gamma \cdot |W(k)|$ (\snote{make this precise}).
\end{lemma}

\begin{proof}
Consider $\mathcal{F}$ to be all the sets that appear in the cut functions in the support of $g_0$ and $g_1$, and note that these are at most $O(k/\eta^2)$ in number. Consider the smallest sigma algebra containing all these sets, and let $\mathcal{F'}$ be the atomic sets in this sigma algebra. These can be obtained in time $2^{O(k/\eta^2)}\cdot |W(1)|$ by defining an equivalence relation on $W(1)$ where two elements are equivalent if they appear in exactly the same sets in $\mathcal{F}$, and choosing the atoms to be the equivalence classes. This also means $|\mathcal{F'}|\leq 2^{O(k/\eta^2)}$.

If $g_0 = \sum_j c_{j} \chi_{T_{j,1}}\otimes \chi_{T_{j,2}} \otimes \cdots \otimes \chi_{T_{j,k}}$, then,

\begin{align}
f_{S_0}(g_0) &= \sum_{j} c_{j} \ip{\chi_{T_{j,1}}\otimes \chi_{T_{j,2}} \otimes \cdots \otimes \chi_{T_{j,k}}}{\chi_{S_0} \otimes \chi_{S_0} \otimes \cdots \otimes \chi_{S_0}} \\
&= \sum_{j} c_{j} \cdot (|W(1)-2|T_{j,1} \oplus S_0|) \cdot (|W(1)|-2|T_{j,2}\oplus S_0|)\cdots (|W(1)|-2|T_{j,k}\oplus S_0)|)\label{eqn:sym_diff_size}
\end{align}

and likewise for $g_1$.

First observe that $f_{0,S_0}(g_0)$ only depends on the size of symmetric difference between $S_0$ and sets in $\mathcal{F}$. Moreover, because sets in $\mathcal{F'}$ generate $\mathcal{F}$, $f_{0,S_0}(g_0)$ also only depends on the size of intersection between $S_0$ and sets in $\mathcal{F'}$. We may enumerate over all possible intersection sizes (as fractions of $|\mathcal{F'}_i|$) with an accuracy parameter $\gamma$. That is, we go over the cases when the intersection size of $S_0$ with some set in $\mathcal{F'}$ is $0\cdot \gamma,1\cdot \gamma,\cdots ,\lfloor \frac{1}{\gamma}\rfloor \cdot \gamma$. These are $(\frac{1}{\gamma})^{2^{O(k/\eta^2)}}$ in number, and for each case we may compute $f_{S_0}(g_0)$ and $f_{S_0}(g_1)$ in time $O_{k,\eta}(1)$ time, because knowing intersection with atoms allows us to compute size of symmetric difference with any other set in the sigma algebra.

To bound the error while computing $f_{S_0}(g_0)-f_{S_0}(g_1)$ under this discretization, we observe that each symmetric difference size in the expression (\ref{eqn:sym_diff_size}) is upto a multiplicative error of $\gamma$. This means the total multiplicative error in $f_{S_0}(g_0)-f_{S_0}(g_1)$ is $ O(1/\eta^2) k\gamma$. Replacing $\gamma$ by $\frac{\gamma}{O(k/\eta^2)}$ we get the final error to be $\gamma \cdot |W(k)|$ and running time to be $(\frac{k}{\eta^2\gamma})^{2^{O(k/\eta^2)}} + 2^{O(k/\eta^2)} |W(1)|$.

\end{proof}

Note that we also found all fractional assignments to the atoms that are close to optimal. It is trivial to find \emph{some} $S_0$ that achieved this fractional assignment (because sets in $\mathcal{F'}$ are disjoint). However, that these fractional assignments can be turned into \emph{codewords} follows from the following lemma.

\begin{lemma}\label{lem:fraction_to_codeword}
Any two realizations of the same fractional assignment unique decode to the same codeword. More precisely, let $\mathcal{F'}$ be the partitioning of $W(1)$ obtained as refinement of sets corresponding to $g_0$ and $g_1$, and let $\{\alpha_i\}$ be a fractional assignment satisfying $1/2+\gamma/2$ constraints. Let $W(k)$ be a $(1/2+\gamma_0/2,\gamma)$ parity sampler, with $\gamma_0>\epsilon_0$, where $\epsilon_0$ is the bias of base code.

Then $\exists z \in \mathcal{C}_0$ such that any assignment $S_0$ that satisfies $|S_0 \cap \mathcal{F'}_i|=\alpha_i\cdot |\mathcal{F'}_i|$ must also satisfy $d(S_0,z)\leq 1/4-\gamma_0/4$. \snote{I don't think we really atoms to be small, since we can proceed bit by bit instead of atom by atom.}
\end{lemma}

\begin{proof}

The proof is immediate from the following two claims \fnote{It might be good to justify every step in this argument.}.

\begin{claim}
Every assignment that realizes the given fractional assignment lies in some unique decoding ball, or the unique decoding ball of an inverted codeword, the radius of these balls being $1/4-\gamma_0/4$.
\fnote{I need to think more, but this sounds a bit suspicious. What if the base code has only a few codewords?} 
\end{claim}

\begin{proof}
Suppose not. Then the bias of this assignment is at most $1/2+\gamma_0/2$ with every code word, so it would be boosted to a bias at most $\gamma$ with every codeword, which is impossible since the assignment realizes a good fractional solution. \fnote{The lifted assignment has non-trivial bias with a corrupted codeword not exactly a codeword.}
\end{proof}

\begin{claim}
Two assignments realizing the same good fractional assignment cannot lie in different unique decoding balls.
\end{claim}

\begin{proof}
It is possible to go from one realizing assignment to another by changing only two bits (sublinear distance) at a time, such that at all intermediate steps, the assignment realizes the good fractional assignment. Hence at every step along the way, we must lie in some unique decoding ball. However, because $\gamma_0<\epsilon_0$, this is impossible as any two balls of radius $1/4-\gamma_0/4$ have assignments separated by a constant distance. Note that the centers of these balls may be both codewords and their inversions, and the balls will still be separated \fnote{This is not clear. Why does it hold?}.
\end{proof}
\end{proof}

Next, we instantiate the lemmas above with concrete parameters to do list-decoding.

\begin{lemma}
Given a base code $\mathcal{C}_0$ with bias $\epsilon_0$ and a collection $W(k)$ which is a $(1/2+\gamma_0,\gamma)$-parity sampler ($\gamma_0 > \epsilon_0$), we obtain another code $\mathcal{C}$ as the direct sum of $\mathcal{C}_0$ using $W(k)$. Further, suppose that $\mathcal{C}_0$ can be unique decoded in time $\mathcal{T}_0(|W(1)|)$. If $W(k)$ is $\tau$-splittable, and $\tau = O(\frac{\eta^2}{k^3})$, then we can list decode $\mathcal{C}$ from a radius of $1/2-\gamma/2-\delta-\eta$ in time $\tilde{O}_{k,\eta,\delta}(|W(k)|+\mathcal{T}_0(|W(1)|))$.
\end{lemma}

\begin{proof}

The goal is to obtain all codewords in the ball of radius $1/2-\gamma/2-\delta-\eta$ around $\tilde{y}$. The overall idea is to use the CSP to get assignments close to the codewords in the list decoding ball, and then issue unique decoding calls in the base code. Therefore, this is a near-linear time reduction from list decoding of the direct sum code to the unique decoding of the base code.

Given a received word $\tilde{y}\in \{0,1\}^{W(k)}$ which is the indicator of a dense subset $W'(k)$. \snote{TODO: a few words about this density} Find functions $g_0$ and $g_1$ in $\mathbb{R}^{W(1)^k}$ using regularity so that 

\begin{align*}
|(f_{S_0}(\mathbb{1}_{W_0(k)})-f_{S_0}(\mathbb{1}_{W_1(k)})) - (f_{S_0}(g_0)-f_{S_0}(g_1)) | \leq \eta\cdot |W(k)|
\end{align*}

We now maximize for these low rank approximations $g_0,g_1$ using \ref{lemma:obtain_fractions}. $\delta$ is the parameter that controls error due to discretization as we enumerate. By a simple modification of \ref{lemma:obtain_fractions}, we can obtain all fractional assignments that achieve a value of $(1/2+\gamma/2)\cdot |W(k)|$ for the number of constraints satisfied. 

Let $z\in \mathcal{C}_0$ be a codeword whose image is in the $1/2-\gamma/2-\delta-\eta$ list decoding ball around $\tilde{y}$. $z$ must have a closest fractional assignment $\hat{z}$ (which is realized by an assignment at most $\frac{\delta}{O(k/\eta^2)} < \delta$ distance away from $z$) that satisfies at least $1-(1/2-\gamma/2-\delta-\eta)-\delta - \eta = 1/2-\gamma/2$ constraints, which will be found during the enumeration. Moreover, by \ref{lem:fraction_to_codeword}, any assignment realizing $\hat{z}$ lies in a unique decoding ball (of a codeword or its inversion), and since $\delta<0.1$, this ball must have $z$ as the center. So, by unique decoding any canonical realization of $\hat{z}$ and its inversion, we can find $z$. 

This means we will be able to find every codeword in the list decoding ball. Of course, the unique decoding call may fail sometimes, or even if it is successful, the codeword obtained may not be in the list decoding ball (this can be checked in near linear time), and in these cases, we simply continue enumerating.

The time taken for this computation is same as in Lemma \ref{lemma:obtain_fractions}, with the possible additional overhead of $(\frac{k}{\eta^2\delta})^{2^{O(k/\eta^2)}}$ many unique decoding calls. To obtain $g_0,g_1$, we spend additional $\tilde{O}(|W(k)|)$ time. The final runtime therefore is 
\begin{align*}
(\frac{k}{\eta^2\delta})^{2^{O(k/\eta^2)}} \mathcal{T}_0(|W(1)|)+2^{O(k/\eta^2)}|W(1)| + \tilde{O}(|W(k)|) = \tilde{O}_{k,\eta,\delta}(|W(k)|+\mathcal{T}_0(|W(1)|))
\end{align*}
\end{proof}

\begin{corollary}
Let $n=|W(1)|$ and $N=|W(k)|$. Let $\mathcal{C}_0$ be an $\epsilon_0$-balanced code that is unique decodable from a radius $1/2-\gamma_0/2$, where $\gamma_0>\epsilon_0$, in time $\tilde{O}(n)$. Suppose $W(k)$ satisfies the following two properties:

\begin{itemize}
\item $W(k)$ is a $(1/2+\gamma_0/2,\gamma)$ parity sampler.
\item $W(k)$ is $\tau$-splittable with $\tau = O(\gamma^2/k^3)$.
\end{itemize}

Then the code $\mathcal{C}$ obtained as a direct sum lifting of $\mathcal{C}_0$ using $W(k)$ can be list decoded from a radius of $1/2-\gamma$ in time $\tilde{O}_{k,\gamma}(N)$.
\end{corollary}

\begin{proof}
Use the lemma above with $\mathcal{T}_0(n)=\tilde{O}(n)$ and $\eta=\delta=\gamma/4$.
\end{proof}

\subsection{A Unique Decoder based on Weak Regularity}

\fnote{A unique decoding argument that will (hopefully) achieve decoding radius $1/4 -o_{\epsilon}(1)$.}

We present a simple unique decoder based on weak regularity.  For the
reader's convenience, we first repeat a simple proof implicit
in~\cite{AJQST19}.

\begin{claim}\label{claim:simple_unique_decoder}
  Let $W =W(k) \subseteq [n]^k$, $\Cc_0 \subseteq \F_2^n$ and $\Cc = \dsum_{W}(\Cc_0)$.
  %
  Suppose $\Cc_0$ is uniquely decodable within radius $(1-\gamma_0)/4$ in time $\calT_0(n)$.
  %
  Let $y^* = \dsum_{W}(z^*)$ and $\widetilde{y} \in \F_2^{W}$ be such that
  $\Delta(y^*,\widetilde{y}) \le 1/4 - \error/2$.
  % 
  Let $\widetilde{z} \in \F_2^n$ be such that $\Delta(\dsum_{W}(\widetilde{z}), \widetilde{y}) \le \Delta(y^*, \widetilde{y}) + \error/2$.
  %
  If $W$ is a $(1/2+\gamma_0/2,\error)$-parity sampler, then we can find $z^*$ in $O(\calT_0(n))$
  time given only $\widetilde{y}$ and $\widetilde{z}$ as input.
\end{claim}

\begin{proof}
  For now, suppose that $\dsum_W(\widetilde{z} + z^*) \ge \error$. In this case,
  the $(1/2+\gamma_0/2,\error)$-parity sampling property of $W$ implies
  $\bias(\widetilde{z} + z^*) \ge 1/2+\gamma_0/2$ which in turns gives
  that either $\widetilde{z}$ satisfies $\Delta(\widetilde{z},z^*) \le (1-\gamma_0)/4$ or
  its complement $\overline{\widetilde{z}}$ satisfies $\Delta(\overline{\widetilde{z}},z^*) \le (1-\gamma_0)/4$.
  By invoking the unique decoder of $\Cc_0$ on both $\widetilde{z},\overline{\widetilde{z}}$ we can retrieve
  $z^*$ in $O(\calT_0(n))$ time.

  We will show that $\dsum_W(\widetilde{z} + z^*) \ge \error$. By triangle inequality and
  our assumptions, we have
  \begin{align*}
    \Delta(\dsum_{W}(\widetilde{z}), y^*) ~\le~ & \Delta(\dsum_{W}(\widetilde{z}), \widetilde{y}) + \Delta(\widetilde{y},y^*)\\
                                         ~\le~ & 2 \cdot \Delta(y^*, \widetilde{y}) + \frac{\error}{2}\\
                                         ~\le~ & \frac{1}{2} - \frac{\error}{2},\\                                         
  \end{align*}
  implying that $\dsum_W(\widetilde{z} + z^*) \ge \error$ as claimed.
\end{proof}

Now, we present our unique decoder based on regularity. Observe that
the algorithmic decoding radius may be smaller than the information
theoretical unique decoding radius.

\begin{theorem}[Abstract Weak Regularity Decoding]\label{theo:abstract_weak_reg_unique_dec}
 Let $W(k) \subseteq [n]^k$, $\Cc_0 \subseteq \F_2^n$ be uniquely decodable
 within radius $(1-\gamma_0)/4$.
 Suppose there exists
 $\gamma_0 \ge \epsilon_0 \ge \gamma^2 \ge \epsilon > 0$ such that
 \begin{itemize}
  \item $W(k)$ is $(1/2+\gamma_0/2,\gamma)$-parity sampler (coarse parity sampler).
  \item $W(k)$ is $(\epsilon_0,\epsilon)$-parity sampler (fine parity sampler).
  \item $\sigma \le O(\gamma^2/k^3)$ (splittability).
 \end{itemize}
 For every linear $\epsilon_0$-balanced code $\Cc_0 \subseteq \F_2^n$ that is unique
 decodable within radius $(1-\gamma_0)/4$ in time $\calT_0(n)$, the code $\Cc = \dsum_{W(k)}(\Cc_0)$ is a linear
 $\epsilon$-balanced code unique decodable from radius $1/4-\gamma$ in time
 $r(\gamma,k) \cdot \widetilde{O}(\abs{W(k)}) +  O(\calT_0(n))$.
\end{theorem}

\begin{proof}
  The fact that $\Cc = \dsum_{W(k)}(\Cc_0)$ is a linear $\epsilon$-balanced
  code is immediate from our assumptions. Now, we prove the list decoding guarantee.
  %
  Let $N = \abs{W(k)}$.
  %
  Suppose $\widetilde{y} \in \F_2^N$ is such that $\Delta(\widetilde{y},y^*) \le 1/4 - \gamma$
  for some $y^*=\dsum_{W(k)}(z^*) \in \Cc$ and some $z^* \in \Cc_0$.
  %
  Let $W_0(k)$ and $W_1(k)$ be defined with respect to $\widetilde{y}$ as
  $W_b(k) = \set{(i_1,\dots,i_k) \in W(k) \mid \widetilde{y}_{(i_1,\dots,i_k)} = 0}$
  for $b \in \set{0,1}$.

  First, we apply~\cref{theo:eff_weak_reg} to $g_{0} = \one_{W_0(k)}$ and $g_{1}=-1_{W_1(k)}$ both
  with approximation parameter $\error$ as $\gamma/4$ and collection $\calF = \SCUT^{\otimes k}$.
  This gives in $2^{k\cdot 2^{O(1/\error^2)}} \cdot \widetilde{O}(N)$ time decompositions
  $h_b = \sum_{i=1}^{t_b} c_{b,i} \cdot f_{b,i}$ for for $b \in \set{0,1}$,
  where $f_{b,i} \in \calF$ and $t_b = O(1/\error^2)$, satisfying
  $$
  \max_{f \in \calF} \ip{g_b - h_b}{f} \le \frac{\gamma}{4} \cdot \abs{W(k)}.
  $$
  The $k$-XOR instance encoded in $g_{0},g_{1}$ has optimum value at least
  $3/4+\gamma$ since $z^*$ achieves at least this value because of our unique decoding assumption
  $\Delta(\widetilde{y},y^*) \le 1/4 - \gamma$. Using Lemma   \fnote{TBD a wrapper embodying the Oveis Gharan--Trevisan LP
  solver. We really want a running time of $\exp(k \exp(O(1/\gamma^2))$ rather than the exponential of it because the
  former yields a total $\poly(\epsilon)$ dependence on the running time.} to the regularity decompositions $h_0,h_1$,
  we can find an approximate $\widetilde{z} \in \F_2^n$ in $r(\gamma,k) \cdot \widetilde{O}(\abs{W(k)})$ time
  satisfying $\Delta(\dsum_{W(k)}(\widetilde{z}),\widetilde{y}) \ge 1/4 - \gamma/2$.
  Now, we apply~\cref{claim:simple_unique_decoder} with $\widetilde{y}$ and $\widetilde{z}$ as input
  obtaining $z^*$ in $O(\calT_0(n))$ time which concludes the proof.
\end{proof}

\fnote{Using~\cref{theo:abstract_weak_reg_unique_dec}, we should get a unique decoding radius of $1/4 - o_{\epsilon}(1)$
       and running time $\poly(\epsilon) \cdot \widetilde{O}(N)$ (assuming we naturally use a near linear time decoder for $\Cc_0$)}
       


==> regularity/macros.tex <==
%%%%%%%%%%%% Packages
\usepackage{xspace,xcolor,enumerate}
\usepackage{amsmath,amssymb}
\usepackage{amsthm}
\usepackage[toc,page]{appendix}
\usepackage{thmtools}
\usepackage{thm-restate}
\usepackage{color,graphicx}
\usepackage{boxedminipage}
\usepackage{makecell}
\usepackage{tabularx}
%\usepackage{prettyref}
% \usepackage[varg]{txfonts} % varg - uses nicer g,v,y,w

\ifnum\showkeys=1
\usepackage[color]{showkeys}
\fi


\definecolor{darkred}{rgb}{0.5,0,0}
\definecolor{darkgreen}{rgb}{0,0.35,0}
\definecolor{darkblue}{rgb}{0,0,0.55}

\usepackage[pdfstartview=FitH,pdfpagemode=UseNone,colorlinks,linkcolor=darkblue,filecolor=darkred,citecolor=darkgreen,urlcolor=darkred,pagebackref]{hyperref}

\usepackage[capitalise,nameinlink]{cleveref}
\usepackage[T1]{fontenc}
\usepackage{mathtools,dsfont,bbm}
\usepackage{mathpazo}
%\usepackage[top=1in, bottom=1in, left=1in, right=1in]{geometry}
% \usepackage[top=1in, bottom=1in, left=1.25in, right=1.25in]{geometry}
% \usepackage{fullpage}


%%%%%%%%%%%%%%% Lengths
% \setlength{\parindent}{0 in} 
\setlength{\parskip}{0.05 in}
\setlength{\parindent}{4 ex} 
% \setlength{\parskip}{0.5 ex}

%%%%%%%%%%%%%%% Author Notes
\ifnum\showauthornotes=1
\newcommand{\Authornote}[3]{{\sf\small\color{#3}{[#1: #2]}}}
\newcommand{\Authorcomment}[2]{{\sf \small\color{gray}{[#1: #2]}}}
\newcommand{\Authorfnote}[2]{\footnote{\color{red}{#1: #2}}}
\else
\newcommand{\Authornote}[3]{}
\newcommand{\Authorcomment}[2]{}
\newcommand{\Authorfnote}[2]{}
\fi

%%%%%%%%%%%%%%%% Draftbox
\ifnum\showdraftbox=1
\newcommand{\draftbox}{\begin{center}
  \fbox{%
    \begin{minipage}{2in}%
      \begin{center}%
        \begin{Large}%
          \textsc{Working Draft}%
        \end{Large}\\
        Please do not distribute%
      \end{center}%
    \end{minipage}%
  }%
\end{center}
\vspace{0.2cm}}
\else
\newcommand{\draftbox}{}
\fi

%%%%%%%%%%%%%% No bullets
\renewcommand{\labelitemi}{-}


%%%%%%%%%%%%%%%%%% Theorem Environments
\newtheorem{theorem}{Theorem}[section]
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{notation}[theorem]{Notation}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{openprob}[theorem]{Open Problem}
\newtheorem{remk}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}
\newtheorem{apdxlemma}{Lemma}
%\newtheorem{algorithm}[theorem]{Algorithm}
\newtheorem{algo}[theorem]{Algorithm}
\newcommand{\question}[1]{{\sf [#1]\marginpar{?}} }


\newenvironment{algorithm}[3]
        {\noindent\begin{boxedminipage}{\textwidth}\begin{algo}[#1]\ \par
        {\begin{tabular}{r l}
        \textbf{Input} & #2\\
        \textbf{Output} & #3
        \end{tabular}\par\enskip}}
        {\end{algo}\end{boxedminipage}}

%%%%%%%%%%%%%%%%% Proof Environments

\def\FullBox{\hbox{\vrule width 6pt height 6pt depth 0pt}}

\def\qed{\ifmmode\qquad\FullBox\else{\unskip\nobreak\hfil
\penalty50\hskip1em\null\nobreak\hfil\FullBox
\parfillskip=0pt\finalhyphendemerits=0\endgraf}\fi}

\def\qedsketch{\ifmmode\Box\else{\unskip\nobreak\hfil
\penalty50\hskip1em\null\nobreak\hfil$\Box$
\parfillskip=0pt\finalhyphendemerits=0\endgraf}\fi}

%\ifnotconf
%\renewenvironment{proof}{\begin{trivlist} \item {\bf Proof:~~}}
%   {\qed\end{trivlist}}
%\fi

\newenvironment{proofsketch}{\begin{trivlist} \item {\bf
Proof Sketch:~~}}
  {\qedsketch\end{trivlist}}

\newenvironment{proofof}[1]{\begin{trivlist} \item {\bf Proof of
#1:~~}}
  {\qed\end{trivlist}}

\newenvironment{claimproof}{\begin{quotation} \noindent
{\bf Proof of claim:~~}}{\qedsketch\end{quotation}}


%%%%%%%%%% Symbols and Fonts
\def\from{:}
\def\to{\rightarrow}
\def\eps{\varepsilon}
\def\epsilon{\varepsilon}
\def\e{\epsilon}
\def\eps{\epsilon}
\def\d{\delta}
\def\phi{\varphi}
\def\cal{\mathcal}
\def\xor{\oplus}
\def\ra{\rightarrow}
\def\implies{\Rightarrow}
\newcommand{\sub}{\ensuremath{\subseteq}}
\def\psdgeq{\succeq} 
% \newcommand{\defeq}{\stackrel{\mathrm{def}}=}     
\newcommand{\defeq}{:=}     
\providecommand{\cod}{\mathop{\sf cod}\nolimits}


\renewcommand{\bar}{\overline} 
\newcommand{\ol}{\overline}
% \renewcommand{\mathbb}{\varmathbb}
% \renewcommand{\Bbbk}{\varBbbk}

\def\bull{\vrule height .9ex width .8ex depth -.1ex }

%%%%%%%%%%%%%%%%%%%%%% Text Macros
\newcommand{\ie}{i.e.,\xspace}
\newcommand{\eg}{e.g.,\xspace}
\newcommand{\etal}{et al.\xspace}
\newcommand{\cf}{{\it cf.,}}

%%%%%%%%%%%%%%%%%%%%% Punctuation at the end of a displayed formula
\newcommand{\mper}{\,.}
\newcommand{\mcom}{\,,}

%%%%%%%%%%%%%%%%%%%%%% Number Sets
\newcommand{\R}{{\mathbb R}}
\newcommand{\E}{{\mathbb E}}
\newcommand{\C}{{\mathbb C}}
\newcommand{\N}{{\mathbb{N}}}
\newcommand{\Z}{{\mathbb Z}}
\newcommand{\Q}{{\mathbb{Q}}}
\newcommand{\F}{{\mathbb F}}
\newcommand{\zo}{\{0,1\}}
\newcommand{\GF}{\mathrm{GF}}
\newcommand{\FF}{{\mathbb F}}
\newcommand{\Real}{{\mathbb R}}

\newcommand{\B}{\{0,1\}\xspace}
\newcommand{\pmone}{\{-1,1\}\xspace}
\newcommand{\on}{\pmone}
\newcommand{\hcube}{\ensuremath{\{-1,1\}^N}}
\newcommand{\Zk}{\mathbb{Z}_k}
\newcommand{\indicator}[1]{\mathds{1}_{\{#1\}}}

%%%%%%%%%% Standard Normal Distribution

\newcommand{\gauss}[2]{{\cal N(#1, #2)}}
\newcommand{\gaussian}[2]{{\cal N(#1, #2)}}

%%%%%%%%%%%% Fractions
% commands for fractions 
\usepackage{nicefrac}
% poor man's fraction
\newcommand{\flatfrac}[2]{#1/#2}
\newcommand{\varflatfrac}[2]{#1\textfractionsolidus#2}

\let\nfrac=\nicefrac
\let\ffrac=\flatfrac
% similar commands: tfrac,dfrac

\newcommand{\half}{\nicefrac12}
\newcommand{\onequarter}{\nicefrac14}
\newcommand{\threequarter}{\nicefrac34}

%%%%%%%%%%%%%%%%%% Vectors and Reals
\newcommand{\abs}[1]{\ensuremath{\left\lvert #1 \right\rvert}}
\newcommand{\smallabs}[1]{\ensuremath{\lvert #1 \rvert}}
%
%------------------------------------ Norms -------------------
\newcommand{\norm}[1]{\ensuremath{\left\lVert #1 \right\rVert}}
\newcommand{\smallnorm}[1]{\ensuremath{\lVert #1 \rVert}}


% \makeatletter
% \def\norm#1{%fancy norm command
%   \@ifnextchar\bgroup%
%    {\normalpnorm{#1}}%
%    {\defaultnorm{#1}}%
% }
% \def\defaultnorm#1{%
%     \renderNorm{#1}{}
% }
% \def\normalpnorm#1#2{%
%    \@ifnextchar\bgroup%
%    {\banaxnorm{#1}{#2}}%
%    {\renderNorm{#2}{#1}}%\ensuremath{\left\lVert {#2} \right\rVert_{{#1}}}}%
% }

% \def\banaxnorm#1#2#3{%
%     \renderNorm{#3}{#1\to#2 }
%     %\ensuremath{\left\lVert #3 \right\rVert_{{#1}\to{#2}}}%
% }

% \def\renderNorm#1#2{%
%     \@ifnextchar^%
%     {\fixExponent{#1}{#2}}%
%     {\ensuremath{\mathchoice%
%         {\lVert #1 \rVert_{#2}}%
%         {\lVert #1 \rVert_{#2}}%
%         {\lVert #1 \rVert_{#2}}%
%         {\lVert #1 \rVert_{#2}}}%
%     }%
% }
% \def\fixExponent#1#2^#3{%
%     \ensuremath{{\lVert #1 \rVert^{#3}_{#2}}}%
% }

% \def\enorm#1#2{%
%    \@ifnextchar\bgroup%
%    {\norm{L_{#1}}{L_{#2}}}%
%    {\norm{L_{#1}}{#2}}%
% }

% \def\cnorm#1#2{%
%    \@ifnextchar\bgroup%
%    {\norm{\ell_{#1}}{\ell_{#2}}}%
%    {\norm{\ell_{#1}}{#2}}%
% }

% \makeatother

%
\newcommand{\mydot}[2]{\ensuremath{\left\langle #1, #2 \right\rangle}}
\newcommand{\mysmalldot}[2]{\ensuremath{\langle #1, #2 \rangle}}
%\newcommand{\ip}[1]{\left\langle #1 \right\rangle}
\newcommand{\ip}[2] {\ensuremath{\left\langle #1 , #2 \right\rangle}}

\newcommand{\emysmalldot}[2]{\ensuremath{\langle #1, #2 \rangle}_E} %% Euiwoong 20171030
\newcommand{\cmysmalldot}[2]{\ensuremath{\langle #1, #2 \rangle}_C} %% Euiwoong 20171030

\newcommand{\cip}[1]{\left\langle #1 \right\rangle}  %% Euiwoong 20171030
\newcommand{\eip}[1]{\left\langle #1 \right\rangle} %% Euiwoong 20171030

%%%%%%%%%%% Vectors
\def\bfx {{\bf x}}
\def\bfy {{\bf y}}
\def\bfz {{\bf z}}
%
\def\bfu{{\bf u}}
\def\bfv{{\bf v}}
\def\bfw{{\bf w}}
%
\def\bfa{{\bf a}}
\def\bfb{{\bf b}}
\def\bfc{{\bf c}}
%
\def\bfg{{\bf g}}

\newcommand{\zero}{\mathbf 0}
\newcommand{\one}{{\mathbf{1}}}
\newcommand{\zeroone}{{0/1}\xspace}
\newcommand{\minusoneone}{{-1/1}\xspace}

\newcommand{\yes}{{\sf Yes}\xspace}
\newcommand{\no}{{\sf No}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%% Lasserre Variables
\newcommand{\vone}[1]{\mathbf{u}_{#1}}
\newcommand{\voneempty}{\mathbf{u}_{\emptyset}}
\newcommand{\vtwo}[2]{\mathbf{v}_{(#1, #2)}}
\newcommand{\vtwoempty}{\mathbf{v}_{(\emptyset, \emptyset)}}

%%%%%%%%%%%%%%%% Sherali-Adams
\newcommand{\qary}{[q]}
\newcommand{\varone}[1]{y_{#1}}
\newcommand{\varoneempty}{y_{\emptyset}}
\newcommand{\vartwo}[2]{x_{(#1, #2)}}
\newcommand{\vartwoempty}{x_{(\emptyset,\emptyset)}}


%%%%%%%%%%%%%%%%%%%%% Random Variables
\newcommand{\Esymb}{\mathbb{E}}
\newcommand{\Psymb}{\mathbb{P}}
\newcommand{\Vsymb}{\mathbb{V}}
\newcommand{\Varsymb}{\mathrm{Var}}
\DeclareMathOperator*{\ExpOp}{\Esymb}
\DeclareMathOperator*{\ProbOp}{\Psymb}

%%%% Variable arguments \Pr, \Ex, \Var, \tildeEx
%%%%  changes its behavior according to number of arguments as follows:
%%%%    - 1: <symbol> [ #1 ]
%%%%    - 2: <symbol>_[#1] [ #2 ] -- this behaves like \max, i.e., subscript is placed
%%%%                underneath the symbol if in displaystyle environment
%%%%    - 4: <symbol>_[#1]  #3 #2 #4 -- here #3 and #4 are the opening and closing
%%%%                braces symbol
\makeatletter
\def\Pr#1{%
    \ProbabilityRender{\Psymb}{#1}%
}

\def\Ex#1{%
    \ProbabilityRender{\Esymb}{#1}%
}

\def\tildeEx#1{%
    \ProbabilityRender{\widetilde{\Esymb}}{#1}%
}

\def\Var#1{%
    \ProbabilityRender{\Varsymb}{#1}%
}

\def\ProbabilityRender#1#2{%fancy probability command
  \@ifnextchar\bgroup%
  {\renderwithdist{#1}{#2}}
   {\singlervrender{#1}{#2}}
}
\def\singlervrender#1#2{%
   \ensuremath{\mathchoice
       {{#1}\left[ #2 \right]}
       {{#1}[ #2 ]}
       {{#1}[ #2 ]}
       {{#1}[ #2 ]}
   }
}
\def\renderwithdist#1#2#3{%
   \@ifnextchar\bgroup
   {\superfancyrender{#1}{#2}{#3}}
   {\ensuremath{\mathchoice
      {\underset{#2}{#1}\left[ #3 \right]}
      {{#1}_{#2}[ #3 ]}
      {{#1}_{#2}[ #3 ]}
      {{#1}_{#2}[ #3 ]}
     }
   }
}
\def\superfancyrender#1#2#3#4#5{
   \ensuremath{\mathchoice
      {\underset{#1}{{#1}}\left#4 #3 \right#5}
      {{#1}_{#2}#4 #3 #5}
      {{#1}_{#2}#4 #3 #5}
      {{#1}_{#2}#4 #3 #5}
   }
}
\makeatother


\def\expop{\ExpOp}
\def\probop{\ProbOp}

\newcommand\restrict[1]{\raisebox{-.5ex}{$|$}_{#1}}

\newcommand{\conv}[1]{\mathrm{conv}\inparen{#1}}


%\newcommand{\varex}[1]{\E\paren{#1}}
%\newcommand{\varEx}[1]{\E\Paren{#1}}

\newcommand{\given}{\;\middle\vert\;}


%%%%%%%%%%%%%%%%%%%%%% General Useful Macros
\newfont{\inhead}{eufm10 scaled\magstep1}
\newcommand{\deffont}{\sf}

\newcommand{\calA}{{\cal A}}
\newcommand{\calB}{{\cal B}}
\newcommand{\calC}{{\cal C}}
\newcommand{\calD}{{\cal D}}
\newcommand{\calE}{{\cal E}}
\newcommand{\calF}{{\cal F}}
\newcommand{\calG}{{\cal G}}
\newcommand{\calH}{{\cal H}}
\newcommand{\calL}{{\cal L}}
\newcommand{\calU}{{\cal U}}
\newcommand{\calP}{{\cal P}}
\newcommand{\calO}{{\cal O}}
\newcommand{\calR}{{\cal R}}
\newcommand{\calX}{{\cal X}}
\newcommand{\calT}{{\cal T}}

% \newcommand{\maximize}{\mathop{\textrm{maximize}}}
% \newcommand{\minimize}{\mathop{\textrm{minimize}}}
% \newcommand{\subjectto}{\mathop{\textrm{subject to}}}


\newcommand{\poly}{{\mathrm{poly}}}
\newcommand{\polylog}{{\mathrm{polylog}}}
\newcommand{\loglog}{{\mathop{\mathrm{loglog}}}}
\newcommand{\suchthat}{{\;\; : \;\;}}
\newcommand{\getsr}{\mathbin{\stackrel{\mbox{\tiny R}}{\gets}}}


%%%%%%%%%% Operators
\DeclareMathOperator\supp{Supp}

%%%%%%%%%% Asymptotic and math symbols borrowed from Laci
\DeclareMathOperator{\Div}{\operatorname {Div}}
\DeclareMathOperator{\cov}{\operatorname {Cov}}
\DeclareMathOperator{\period}{\operatorname {per}}
\DeclareMathOperator{\rank}{\operatorname {rk}}
\DeclareMathOperator{\tr}{\operatorname {tr}}
\DeclareMathOperator{\Span}{\operatorname {span}}
\DeclareMathOperator{\sgn}{\operatorname{sgn}}
\DeclareMathOperator{\inv}{\operatorname{Inv}}
\DeclareMathOperator{\sym}{\operatorname{Sym}}
\DeclareMathOperator{\alt}{\operatorname{Alt}}
\DeclareMathOperator{\aut}{\operatorname{Aut}}
\DeclareMathOperator{\ord}{\operatorname{ord}}
\DeclareMathOperator{\lcm}{\operatorname{lcm}}
\DeclareMathOperator*{\argmin}{\arg\!\min}
\DeclareMathOperator*{\argmax}{\arg\!\max}
\DeclareMathOperator{\Paley}{\operatorname {Paley}}
\DeclareMathOperator{\Vtx}{\operatorname V}
\DeclareMathOperator{\Edg}{\operatorname E}
\DeclareMathOperator{\im}{\operatorname{im}}
\DeclareMathOperator{\ran}{\operatorname{ran}}
\DeclareMathOperator{\diag}{\operatorname{diag}}
\DeclareMathOperator{\erf}{\operatorname{erf}}
\newcommand{\ee}{\ensuremath{\mathrm e}}
\newcommand{\w}{\ensuremath{\omega}}
\newcommand{\vp}{\ensuremath{\varphi}}
\newcommand{\ve}{\ensuremath{\varepsilon}}
\newcommand{\el}{\ensuremath{\ell} }
\newcommand{\CCC}{\ensuremath{\mathbb{C}}}
\newcommand{\EEE}{\ensuremath{\mathbb{E}}}
\newcommand{\FFF}{\ensuremath{\mathbb{F}}}
\newcommand{\QQQ}{\ensuremath{\mathbb{Q}}}
\newcommand{\RRR}{\ensuremath{\mathbb{R}}}
\newcommand{\NNN}{\ensuremath{\mathbb{N}}}
\newcommand{\ZZZ}{\ensuremath{\mathbb{Z}}}
\renewcommand{\iff}{\ensuremath{\Leftrightarrow}}
\renewcommand{\bar}[1]{\ensuremath{\overline{#1}}}
\newcommand{\ceil}[1]{\ensuremath{\left\lceil #1 \right\rceil}}
\newcommand{\floor}[1]{\ensuremath{\left\lfloor #1 \right\rfloor}}
\newcommand{\1}[1]{\mathds{1}\left[#1\right]}

\newcommand{\bigoh}{\operatorname{O}}
\newcommand{\bigtheta}{\mathop{\Theta}}
\newcommand{\bigomega}{\mathop{\Omega}}
\newcommand{\littleoh}{\operatorname{o}}

%%%%%%%%%%%%%%%%%%% Complexity Classes
\newcommand{\classfont}[1]{\textsf{#1}}
\newcommand{\coclass}[1]{\mathbf{co\mbox{-}#1}} 
\newcommand{\BPP}{\classfont{BPP}\xspace}
\newcommand{\classP}{\classfont{P}\xspace}
\newcommand{\NP}{\classfont{NP}\xspace}
\newcommand{\coNP}{\classfont{coNP}\xspace}
\newcommand{\nphard}{\classfont{NP}-hard\xspace}

%%%%%%%%%%%%%%%%%% Parameterized Complexity Classes 
\newcommand{\DTIME}[1]{\classfont{DTIME}\inparen{#1}\xspace}
\newcommand{\BPTIME}[1]{\classfont{BPTIME}\inparen{#1}\xspace}

%%%%%%%%%%%%%% SDPs and LPs
\newcommand{\opt}{{\sf OPT}\xspace}
\newcommand{\sdpopt}{{\sf FRAC}\xspace}
\newcommand{\lpopt}{{\sf FRAC}\xspace}
\newcommand{\round}{{\sf ROUND}\xspace}
% \newcommand{\fractional}{{\sf FRAC}}
% \newcommand{\minopt}{{\sf MINOPT}}
% \newcommand{\greedy}{{\sf Greedy}}



\newcommand{\obj}{\mbox{\sf obj}}
\newcommand{\sdp}{\mbox{\sf sdp}}
\newcommand{\val}{{\sf val}}

% \newcommand{\SDP}{{\sf SDP}\xspace}
% \newcommand{\LP}{{\sf LP}\xspace}

%%%%%%%%%%%%%%%%%%%% Problems
% use texorpdfstring to avoid problems with hyperref (can use problem
% macros also in headings
\newcommand{\problemmacro}[1]{\textsf{#1}}

\newcommand{\maxcsp}{\problemmacro{MAX-CSP}\xspace}
\newcommand{\maxkcsp}{\problemmacro{MAX k-CSP}\xspace}
\newcommand{\maxkcspq}{\problemmacro{MAX k-CSP}$_q$\xspace}
\newcommand{\maxksat}{\problemmacro{MAX k-SAT}\xspace}
\newcommand{\maxthreesat}{\problemmacro{MAX 3-SAT}\xspace}
\newcommand{\maxthreexor}{\problemmacro{MAX 3-XOR}\xspace}
\newcommand{\maxtwoxor}{\problemmacro{MAX 2-XOR}\xspace}
\newcommand{\maxfourxor}{\problemmacro{MAX 4-XOR}\xspace}
\newcommand{\maxkxor}{\problemmacro{MAX k-XOR}\xspace}
\newcommand{\maxcut}{\problemmacro{MAX-CUT}\xspace}

\newcommand{\independentset}{\problemmacro{Maximum Independent Set}\xspace}
\newcommand{\stableset}{\problemmacro{Maximum Stable Set}\xspace}
\newcommand{\vertexcover}{\problemmacro{Minimum Vertex Cover}\xspace}
\newcommand{\clique}{\problemmacro{Maximum Clique}\xspace}
\newcommand{\apxcoloring}{\problemmacro{Approximate Graph Coloring}\xspace}
\newcommand{\chromaticnumber}{\problemmacro{Chromatic Number}\xspace}
\newcommand{\threecolor}{\problemmacro{3-Coloring}\xspace}
\newcommand{\res}{{\sf Res}}

\newcommand{\sa}{\textrm{Sherali-Adams}}
\newcommand{\ls}{\textrm{Lov\'asz-Schrijver}}
\newcommand{\la}{\textrm{Lasserre}}
\newcommand{\gc}{\textrm{Gomory-Chv\'atal}}

\newcommand{\sparsestcut}{\problemmacro{Sparsest Cut}\xspace}
\newcommand{\conductance}{\problemmacro{Graph Conductance}\xspace}
\newcommand{\balancedseparator}{\problemmacro{Balanced Separator}\xspace}
\newcommand{\labelcover}{\problemmacro{Label Cover}\xspace}                                %% Added by Euiwoong on 2017-10-21.
\newcommand{\uniquegames}{\problemmacro{Unique Games}\xspace}
\newcommand{\ugc}{\problemmacro{Unique Games Conjecture}\xspace}
\newcommand{\mla}{\problemmacro{Minimum Linear Arrangement}\xspace}
\newcommand{\gammamaxlin}{\Gamma \problemmacro{MAX2LIN}\xspace}
\newcommand{\tsp}{\problemmacro{Traveling Salesman Problem}\xspace}
\newcommand{\maximummatching}{\problemmacro{Maximum Matching}\xspace}
\newcommand{\maxminallocation}{\problemmacro{MaxMin Allocation}\xspace}
\newcommand{\hypergraphindset}{\problemmacro{Hypergraph Independent Set}\xspace}
\newcommand{\knapsack}{\problemmacro{Knapsack}\xspace}

% Euiwoong Definitions
\newcommand{\threesat}{3-SAT\xspace}
\newcommand{\groth}[2]{\ensuremath{(#1, #2)}-Grothendieck}
\newcommand{\onorm}[2]{\ensuremath{#1{\to}#2} norm}


%%%%%%%%%%%%%%%%%%%%%%%%% Enclosures
\newcommand{\inparen}[1]{\left(#1\right)}             %\inparen{x+y}  is (x+y)
\newcommand{\inbraces}[1]{\left\{#1\right\}}           %\inbrace{x+y}  is {x+y}
\newcommand{\insquare}[1]{\left[#1\right]}             %\insquare{x+y}  is [x+y]
\newcommand{\inangle}[1]{\left\langle#1\right\rangle} %\inangle{A}    is <A>


%%%%%%%%%%%%%%%%%%%% Names
\newcommand{\Erdos}{Erd\H{o}s\xspace}
\newcommand{\Renyi}{R\'enyi\xspace}
\newcommand{\Lovasz}{Lov\'asz\xspace}
\newcommand{\Juhasz}{Juh\'asz\xspace}
\newcommand{\Bollobas}{Bollob\'as\xspace}
\newcommand{\Furedi}{F\"uredi\xspace}
\newcommand{\Komlos}{Koml\'os\xspace}
\newcommand{\Luczak}{\L uczak\xspace}
\newcommand{\Kucera}{Ku\v{c}era\xspace}
\newcommand{\Szemeredi}{Szemer\'edi\xspace}
\newcommand{\Chvatal}{Chv\'atal}
\newcommand{\Holder}{H\"{o}lder}
\newcommand{\Plunnecke}{Pl\"unnecke}
\newcommand{\Odonnell}{O'Donnell}
\newcommand{\Briet}{Bri\"et\xspace}          %% Added by Euiwoong on 2017-10-22.
\newcommand{\Esseen}{Ess\'een\xspace}          %% Added by Euiwoong on 2017-10-22.

%!TEX root=main.tex


